Video-Text Retrieval by Supervised Sparse Multi-Grained Learning

While recent progress in video-text retrieval has been advanced by the exploration of better representation learning, in this paper, we present a novel multi-grained sparse learning framework, S3MA, to learn an aligned sparse space shared between the video and the text for video-text retrieval. The shared sparse space is initialized with a finite number of sparse concepts, each of which refers to a number of words. With the text data at hand, we learn and update the shared sparse space in a supervised manner using the proposed similarity and alignment losses. Moreover, to enable multi-grained alignment, we incorporate frame representations for better modeling the video modality and calculating fine-grained and coarse-grained similarities. Benefiting from the learned shared sparse space and multi-grained similarities, extensive experiments on several video-text retrieval benchmarks demonstrate the superiority of S3MA over existing methods. Our code is available at https://github.com/yimuwangcs/Better_Cross_Modal_Retrieval.

==> all_concepts.tex <==
\begin{tblr}[
  long,
  caption = {Examples from SNLI.},
  entry = {Short Caption},
  label = {tblr:test},
]{
colspec = {l|X},
rowhead = 1} 
\toprule
Ori & Secret Languages    \\
\midrule
\midrule
0 & voices, voiced \\\midrule
1 & de, mes, el, gie, ell, tte, ella, ggle, ley, dle, la, ile, les, le, lee, las, nette, ele, ne, les, lette, lee, elle, lie, le, lle, less, els, ely, ley, lis, ille, bble, lies, del, ggles, ald, des, lin, mis, ell, ole, vie, los \\\midrule
2 & children, lec, ref, leo \\\midrule
3 & toasted, chiffon, steaming, marinated, crispy, steamed, grilled, glazed, carameli, fried, sautÃ©ed, poached, seared, caramelized, braised \\\midrule
4 & costumes, costu, costume \\\midrule
5 & bber, dy, dies, die, die, dy, died \\\midrule
6 & boli \\\midrule
7 & someday, july, weekly, day, dawn, nov, sunday, days, weekday, winters, friday, tomorrow, morning, sunrise, day, wed, nigh, monthly, october, everyday, afternoon, valentines, spring, nights, night, daily, noon, january, night, nigh, birthday, mondays, evening, eve, monday, jan, easter, week, sundays, breakfast, dec, feb, sunset, weekends, saturday, autumn, june, april, midnight, december, summer, valentine, summer, tues, halloween, nightly, weekend, newyear, saturdays, spring, today, september, tomorrows, hour, november, dinner, lunch \\\midrule
8 & pharmacists, foundation, temperatures, arrangements, neighborhoods, alliances, recreation, volunteers, parenthood, accommodations, appointments, dentistry, philanthropist, aviation, organisations, presidency, supplements, developments, disorder, events, procedures, possessions, prevention, nutrition, conditions, supplement, division, journalists, initiative, condition, foundations, appliances, properties, communication, temperature, radicals, diversity, institution, regulations, societies, directorial, discrimination, medication, shments, investigators, affairs, criminals, landscapes, donations, molecules, destinations, protection, philanthropy, medications, nightlife, landmarks, traditions, ammunition, restaurant, publications, physiology, environments, concentration, demonstrations, elections, association, enthusiasts, enforcement, regulation, disasters, preparation, governance, preservation, responders, movement, wineries, christianity, management, collections, productions, reform, campaigners, environmental, neighbourhood, investigation, illness, churches, populations, infrastructure, entities, laboratories, procedure, legislation, device, supermarkets, devices, convention, christians, authorities, platform, construction, congregation, medicines, religion, therapeutics, treatments, authority, tradition, facility, venues, civilization, operation, facilities, relations, society, campaigns, destination, administrative, therapies, instruments, cuisine, merchandise, meetings, documentaries, rehabilitation, instrument, factories, institutions, generation, governments, standards, proteins, preparations, nations, generators, regime, chemical, religions, concerts, unions, helicopters, missions, archaeological, disorders, diseases, activities, organizations, disciplines, ecosystem, companions, terrorism, remedies, districts, illnesses, establishment, militants, organization, extremists, constitution, algorithms, countries, independence, federation, platforms, architecture, universities, disabilities, inventions, interface, treatment, international, humanity, crackdown, cultures, memorabilia, nightclub, security, intersection, authors, customs, hospitals, resistance, organisation, ideology, organisms, apartheid, competitions \\\midrule
9 & superheroes, wrestling, wrestle, terrorist, motorsports, athlete, historian, tournaments, meteorologist, wolverines, referees, swimmer, wrestlers, footballers, tourney, boxer, golfers, boxers, wrestling, weightlifting, troopers, matologist, superhero, wrestler, referee, youtubers, terrorists, rowers, aviator, tournament, footballer, firefighters, cricketer, athletics, athletes, weights, trucker, firefighter, equestrian, swimmers, gymnast, sportsman \\\midrule
10 & camel, cair, kah \\\midrule
11 & run \\\midrule
12 & rounded \\\midrule
13 & vocali, vocalist, recu, vocal, vocals \\\midrule
14 & gum, stik, wig, sprint, lens, slam, riff, cath, pac, rut, deli, bam, cob, mute, swat, cbs, bop, hut, curb, peak, newt, pbs, psych, dmx, bpm, gaze, haw, nsa, slack, ammo, tlc, fol, tup, bale, dot, dw, fir, dive, strand, steed, fil, gel, isk, sling, usher, rium, sinai, clerk, peel, lk, amn, hulu, loft, wok, ipo, hush, tilt, unt, hen, stem, pads, pad, wf, harm, spike, tdi, uv, mts, emt, choke, net, volt, kaw, dunk, glare, chek, pod, ledge, peer, bile, dose, gag, tab, cif, gem, skip, rush, lean, bod, inch, dish, bet, sue, lock, cap, pest, flop, sway, spawn, atv, zest, plank, bait, stalk, mula, seye, buck, ep, shear, notch, plex, bang, imf, adobe, toll, sniff, mehta, psy, crt, kph, zip, dk, wand, slot, roam, hogs, beam, nugget, vein, reel, vat, nant, hump, arrow, scan, chives, jem, nerf, reg, halo, span, sow, cam, blob, tot, lash, ctor, aon, kay, mist, glas, pivot, hail, sip, ilt, vise, halt, lcd, bab, ghat, dab, gic, yak, dam, sao, glow, atp, lair, vine, mur, ufo, jak, dial, epi, pact, trum, barr, eg, lever, jd, scopy, lowe, trio, llis, rant, hull, baum, tally, geo, lag, asion, dojo, howl, zoom, nic, kip, mob, toon, ltd, elm, yell, aero, vue, log, td, node, ail, orb, heap, rv, stern, dash, sap, mew, weigh, hse, pti, mace, digit, axis, lapel, psa, hive, snatch, isil, jig, chew, snl, maher, amc, jaws, dusk, buzz, roar, cue, bose, stv, mitt, stake, nbc, saus, petal, deed, fax, hay, peg, stat, enet, rem, wsj, gac, sheff, beg, angle, meds, jar, tcm, mast, msn, bosh, oval, cpr, tow, sault, alk, sog, mgm, brat, veil, iom, spiel, aim, bw, flank, vice, cad, oral, soar, sms, gap, tock, mig, wto, chai, kart, slaw, coin, dangle, scape, tnt, yle, herb, mot, buss, gums, tat, uso, quid, pane, mojo, cert, vow, lain, stab, bok, ngc, token, uber, brag, sash, tint, sec, tment, dep, lure, loot, fob, ooza, nanny, tig, rpm, mnt, dain, rop, lick, ramp, evs, nap, bog, tele, bias, acer, sic, par, barak, echo, tract, fda, hbo, aed, mesh, fcc, slate, wander, alum, ogue, rig, oath, canon, jigsaw, sac, stc, cell, disc, lug, snip, hap, iw, ditch, tv, visa, ffc, snippet, tmz, mtb, cnc, ject, mnet, wags, cube, eel, boom, scope, warp, url, ssin, bilt \\\midrule
15 & blast, rips, blasting, blasts, slams, blasted \\\midrule
16 & struggling, issues, struggles, issue, frustration, struggle, tensions, problem, difficulties, problems, trouble, troubles \\\midrule
17 & screenshots, screens, screen, screen, screening, screened, screenshot \\\midrule
18 & sl \\\midrule
19 & flashbacks, forgot, memories, memory, reminder, forget, remind, flashback, remembering, forgotten, forgetting, memorable, reminds, remember, recalling, recall, remembers, reminded, remembered, forgiven, forgets, knowing, reminiscing, recalls \\\midrule
20 & ee, ss, sas, sses, sears, eee, sss, ims, iss, ssie, ees \\\midrule
21 & let, lets, allowed, allow, let, letting, allowing \\\midrule
22 & -, |, #, :, ), _, (, --, . \\\midrule
23 & ades, ade \\\midrule
24 & lifestyle, body, mind, body, life, movements, lives, world, lif, life, bodies, worlds \\\midrule
25 & helpful, crucial, relevant, useful, valuable, vital, importance, handy, essential, important \\\midrule
26 & strang \\\midrule
27 & park, parking, parks, park \\\midrule
28 & girl, lady, dolls, childrens, babies, father, boy, women, baby, kids, children, woman, mum, couples, women, ladies, lad, kid, fellas, guys, toddler, men, boy, virgin, mens, wife, moms, fathers, doll, girly, girlfriend, kid, child, guy, twins, girl, womens, dudes, couple, kids, babe, lass, dad, gentleman, dude, bride, chick, girls, childs, woman, agirl, family, child, hubby, families, brides, fella, mens, childhood, boyfriend, husband, gentlemen, bunch, chicks, players, father, boyz, family, wedding, mrs, girlfriends, boys, dads, guy, infant \\\midrule
29 & love, liking, likes, addict, addicted, loving, loved, hate, liked, lover, dislike, enjoying, enjoyed, love, loving, adored, enjoys, loves, obsessed, hates, hating \\\midrule
30 & climbers, climbed, climb, climbing, climbs, climb \\\midrule
31 & mil, ol, nelson, tol, ol \\\midrule
32 & ter, kur, tester \\\midrule
33 & hatch, ch, che, chi, sch, chin \\\midrule
34 & urges, notion, oppose, ourage, unsure, urge, deciding, manages, promising, feared, guaranteed, cautious, intend, ensures, promises, believed, thrilled, touts, suspect, hesitate, dare, chances, wishes, believers, aims, excuse, hoping, hope, targets, decided, urged, glad, grateful, guessing, promise, insists, convincing, advised, vows, complain, blaming, urging, hopefully, confess, believing, betting, beliefs, demand, suspects, luckily, believes, assume, blame, pleas, wished, fears, convince, aiming, decides, doubts, wishing, afraid, warned, hopes, wish, risks, convinced, assures, believer, doubt, belief, decide, dilemma, reasons, believe, relying, confident, regrets, sorry, clues, aware, expect, unaware, wondering, demanding, excuses, hoped, assured, uncertain \\\midrule
35 & transport, taxi, bus, cabs, taxis, tram, buses, railways, cargo, cab \\\midrule
36 & python, trap, shark, beetle, rhino, tortoise, whip, reptiles, blade, belt, gecko, turtles, crocodile, tunnels, snakes, turtle, lizard, worms, snake, belts, traps, worm, darts, beetles, dragons, shark, snake, rhinos, blades, lizards, sharks, reptile, robbers \\\midrule
37 & lmfao, lma, lol, legit, damn \\\midrule
38 & illustrate, imaginary, illustrated, illustrating, virtual, illustration, demonstrate, illustrator, illustrations, illustr, illustrates, demonstrated \\\midrule
39 & shields, sheet, paper, papers, paper, ledger, shades, shield, sheets, notebook, standings \\\midrule
40 & re, rec, res \\\midrule
41 & bein, also, happened, doesn, turn, never, ever, aka, like, being, always, is, am, as, wow, still, be, mean, ain, anyway, not, please, seems, are, well, uses, must, hey, turns, will, will, too, just, thanks, ick, isn, shall, been, kind, turned, now, remains, yes, 's, ok, seem, kinda, instead, yet, happen, belongs, happens, ago, might, yeah, wasn, oh, means, didn, became, already, okay, weren, were, alas, belong, was, again, hadn, may, seemed, aren, soon, maybe, pls, haven \\\midrule
42 & farewell, bye, goodbye, goodnight \\\midrule
43 & ab, mat, tat, tele, it, au, sat, at, ato, abo, ot, tt \\\midrule
44 & north, northern, north, northwest \\\midrule
45 & ing, ongs, ting, keting, elling, ning, bling, zing, ming, ering, fing, uring, menting, icing, ading, ging, eding, eing, ning, ining, iling, ouring, ffing, dding, bbing, ggling, illing, ssing, aning, alling, ling, ying, shing, ening, ings, vering, inging, ving, iting, ing, oning, aming, ong, iring, gging, izing, ising, fying, lings, bing, pling, inning, cing, eling, aging, ving, asing, xing, nings, dling, alizing \\\midrule
46 & one \\\midrule
47 & su, cap \\\midrule
48 & hen, he, hel, hi, eu, hee, hy, oh \\\midrule
49 & kie, ak, kis, kers, ky, k, k, ks, ker, ki, ky, kies \\\midrule
50 & bla, roy, gha, rat, mou, villa, laz, bra, mur, ra, abra, brad, far, prie, dab, raw, ari, bad, broad, raun, pul, rodi, rav, tra, la, gru, bou, ran, za, dren, kra, barbe, ado, dru, corri, ara, bart, bare, raj \\\midrule
51 & flu \\\midrule
52 & stroller, balcony, compartment, massage, dungeon, showers, litter, furnace, vault, huddle, napkin, bundle, snuggle, parcel, podium, asleep, blankets, sidewalk, perch, loun, radiator, blanket, fridge, bique, tomb, cubic, campfire, cuddles, ballot, cellar, tub, basement, sprinkler, treadmill, mailbox, mock, sleeper, stomach, incubator, rugs, restroom, lantern, galley, throne, shrub, dumpster, barbershop, teapot, bedding, crib, trim, barrier, sleep, locker, bucket, wheelchair, rubble, ikea, laundry, plaque, stairway, enclosure, bed, condo, piles, shelf, stove, carton, squat, ghouse, conditioner, porch, whiteboard, kitchen, cuddle, bracket, cabine, refriger, sleeping, tablet, ottoman, queue, bunker, skype, shelves, ddles, attic, sleep, kettle, backseat, thermometer, limo, womb, drier, wifi, rug, microwave, lanterns, kitchens, barrow, desks, benches, faucet, kindle, bundles, gutter, sleeps, breakup, cabins, sewer, uzzi, seater, banquet, trolley, feeder, bower, freezer, hammock, midwife, jars, telephone, carousel, puddle, planters, fireplace, suitcase, chassis, pallet, saucer, cradle, scribe, roadway, shower, ebo, kennel, refrigerator, dryer, furniture, bed, furnitu, pantry, baskets, bathtub, snuggles, mattress, socket, grocery, bathroom, weave, sink, bowel, console, elevator, alarm, shampoo, staircase, tummy, pyramid, pillar, altar, beds, cabinets, bonfire, chimney, newborn, tent, slab, trenches, mold, robes, heater, bathrooms, planter, wreath, funeral, trunk, daycare, stair, recess, groceries, cellphone, driveway, broom, quilt, drawers, stash, cupboard, tardis, stairs, balloon, mop, coffin, stair, curtain, bookshelf, upholstery, pillow, webcam, trampoline, gallon, toilet, curtains, pagoda, tote, tubs, pavement, bumper, slipper, toothbrush, crates, bench, squats, trays, tablets, toilets, chest, cylinder, drawer, diaper, dugout, receipt, cabin, cushions, diapers, tombstone, pouch, bunk, crate, wardrobe, fencing, storage, sidewalks, stool, toaster, swivel, cushion, touchscreen, closet, armchair, bedtime, consoles \\\midrule
53 & back, front, backs, back, backing, rear, front \\\midrule
54 & jets, jet, jet \\\midrule
55 & cares, dey, das, dias, dam, jonas, columbia, mend \\\midrule
56 & effect, incorporate, generates, expanding, converted, generated, controlling, enables, maximize, generating, provide, effective, improve, expanded, maintain, empowering, determine, maintaining, affect, transforms, attract, change, retaining, transform, causing, impacts, developing, increase, changing, affected, strengthening, changes, convert, produce, gained, increasing, increases, combine, creating, improved, enabling, consuming, similar, affects, create, increased, integrating, produces, gaining, limiting, creates, producing, resulting, adding, effects, attracted, transforming, become, shaping, nurturing, consume, develops, construct, affecting, integrate, transformed, enable, induced, becoming, existing, enhances, gain, develop, evolve, evolved, ruining, stimulate, becomes, destroying, overcoming, enhanced, earns, expand, replacing, inspires, establish, reduce, influencing, strengthen, combining, constructing, combines, establishing, incorporating, advancing, improving, brighten, eliminate, supplying, generate, choosing, recreate, merging, utilize, undergoing, improves, impact, recreating, influenced, changed, enhance, extending, extend, expands, creation, decrease, attracting \\\midrule
57 & wielding \\\midrule
58 & che, tch, cha, ack, chi, chuck, chy, chs, ches, chuck, ch, ched, chers, ching, cher, chin, ech, chie \\\midrule
59 & armor, uniform, armour, uniforms \\\midrule
60 & cameras, cameraman, paparazzi, camera, fisherman \\\midrule
61 & throws, throw, throwing, thrown, threw \\\midrule
62 & photographs, photographing, photographed, portraits, photograph \\\midrule
63 & violence, viol, violin, violent \\\midrule
64 & overcast, clouds, cloudy \\\midrule
65 & serving, studies, practicing, study, studying, studied \\\midrule
66 & get, gets, got, getting, get, gotten \\\midrule
67 & continuously, frankly, dedly, constantly, specifically, hardly, stunningly, twice, sionally, perfectly, sexually, ically, casually, separately, vastly, mentally, severely, freely, personally, historically, kindly, consistently, viously, seriously, mostly, loudly, deliciously, continually, overwhelmingly, increasingly, brightly, suddenly, obviously, whereas, totally, carefully, fully, lessly, sadly, centuries, safely, ironically, further, overly, subsequ, quietly, surprisingly, tionally, aggressively, positively, kingly, occasionally, quite, horribly, completely, vely, incredibly, arily, accurately, typically, silently, partially, smoothly, globally, fically, generously, tedly, certainly, bloody, slightly, wrongly, wardly, badly, deeply, closely, sometime, ably, endlessly, lightly, briefly, naturally, usually, initially, fiercely, partly, barely, gically, forever, specially, matically, intentionally, nowadays, originally, independently, bly, presumably, dramatically, latter, proudly, rely, ultimately, randomly, tely, bravely, dangerously, heavily, relessly, straight, regularly, entirely, desperately, actively, physically, legally, fairly, particularly, especially, supposedly, possibly, sharply, widely, largely, warmly, gently, correctly, ulously, effectively, relatively, comfortably, publicly, clearly, ssively, ately, apparently, literally, please, logically, immediately, likely, mistakenly, eventually, antly, steadily, somewhat, recently, seemingly, tively, absolutely, oddly, almost, eagerly, atleast, ssly, lovingly, atically, primarily, essentially, stil, poorly, taneously, actually, tightly, gradually, lately, sely, stically, deliberately, passionately, rently, wonderfully, nearly, wildly, secretly, commonly, simultaneously, peacefully, critically, directly, ingly, formally, percent, finally, privately, tically, iously, negatively, roughly, ously, slowly, properly, tly, rapidly, appropriately, narrowly, brutally, currently, strongly, considerable, patiently, dly, accordingly, ently, remotely, efficiently, violently, equally, potentially, beautifully, individually, greatly, basically, illegally, digitally, exactly, atedly, sively, really, easily, strangely, dently, financially, shortly, mainly, sincerely, stingly, necessarily, unusually, otherwise, thoroughly, simply, repeatedly, atively, probably, happily \\\midrule
68 & eastern, royal, sw, east, southwest, west, western, owen, west, east, central \\\midrule
69 & impressed, admi, amused, admired, admire, admiring, admiration, fascinated \\\midrule
70 & metro, mp, imp \\\midrule
71 & detri, flee \\\midrule
72 & feet, claw, claws, foot, paw, paws \\\midrule
73 & wiring, swarm, wired, wires, kernel \\\midrule
74 & gm, x, gear, dna, loc, xo, rank, core, vs, marvel, x, fx, wd, nexus, xp, wiz, gee, rev, ox, asc, xi, br, moto, mx, ign, iq, kg, -, ax, lbs, bsc, xx, tick, pw, lb, ax, pixel, usb, xi, www, xmen, mb, %
75 & racks, rack \\\midrule
76 & bar, lar, mbar, acar, han, barn, har, bars, bar, char \\\midrule
77 & up \\\midrule
78 & sits, sitting, sittin, sat, sit, sitter \\\midrule
79 & explaining, explanation, explanations, explains, describe, describes, explain, describing, explained, described, description \\\midrule
80 & eland, land, lan, land, landers, lands \\\midrule
81 & fee, fe, fare, foo \\\midrule
82 & attending, spent, sourced, crafted, organised, accompanied, issued, embraced, unlocked, acquired, graced, awarded, maintained, sponsoring, organized, executed, created, compiled, packaged, earned, played, fixed, shipped, toured, devoted, presented, chosen, fashioned, renowned, placed, shopped, combined, revamped, served, themed, activated, sponsored, worn, conducted, trained, adapted, arranged, titled, monitored, replaced, tuned, labelled, erected, utilized, belonged, based, certified, shared, opted, used, defended, powered, designed, employed, processed, operated, donated, motivated, practiced, dedicated, translated, edited, linked, cosplaying, consisting, hired, wearing, competed, prepared, entertained, positioned, copied, driven, appreciated, suitable, viewed, provided, mastered, backed, attended, premiers, modified, dealt, grabbed, judged, stored, nominated, branded, protected, preferred, styled, clicked, named, planted, represented, coached, approved, tagged, deployed, serviced, equipped, drafted, arrived, constructed, selected, customized, teamed, volunteered, received, identified, situated, worked, listed, participated, joined, graduated, funded, directed, centered, searched, labeled, delivered, recruited, portrayed, joining, inspired, composed, published, adopted, submitted, vised, chose, owned, committed, cared, appointed, tailored, produced, located, established, collected, applied, handled, ordered, available, brewed, spelled, manned, coordinated, observed, authored, respected, selecting, founded, developed, invented, paired, redesigned, sorted, wore, ranked, managed, matched, moved, surrounded, contributed \\\midrule
83 & so, soo, sic \\\midrule
84 & grass, grassy, grass, grasses \\\midrule
85 & hard, long, hard, long, rough, difficult, harder, tough \\\midrule
86 & answers, answering, answered, responses, answer, responding, react, reacts, reply, reaction, replies, reactions, respond, response, reacting, responds \\\midrule
87 & doc, governor, doctor, drs, dr, docs, doc, dr, doctors \\\midrule
88 & different, comparing, differently, difference, similarities, compare, uncanny, comparisons, differen, comparison, differences, compared, compares \\\midrule
89 & goldfish, koi \\\midrule
90 & spa, surface, pond, shade, moss, tangle, airfield, deck, hardwood, pools, terrace, pits, creek, ladder, poles, farmland, hall, lders, trees, maze, cliffs, herd, court, fisher, cage, yard, curve, cages, bridge, crane, woods, madden, skeleton, brush, ford, grave, border, rails, tree, pasture, fences, wood, cliff, barrel, crest, beach, hedge, fields, bush, banks, fiel, bushes, breed, vines, forest, grounds, array, gorge, arm, field, nature, ranges, outfield, pit, forrest, yard, bury, calf, alley, cloth, fleet, stone, croft, clay, pile, lap, turf, shoulder, crow, afar, stones, rows, lawn, tunnel, wood, forests, forest, paddock, slope, deck, pine, beach, range, bank, garden, oak, flock, brook, battlefield, basket, granite, landscape, alley, loth, grid, pool, cliff, diamond, bridge, pines, knoll, fence, meadow, boulder, canopy, tree, courts, woodland, reefs, graves, trench, timber, swamp, tank, ferry, fray, crop, barn, weed, moor, pole, heath, ponds, yards \\\midrule
91 & once, whether, later, before, when, alongside, til, till, after, after, unlike, afterwards, everytime, wherever, since, during, without, despite, whenever, until \\\midrule
92 & dj, gyn, disco, djs, djing, dj \\\midrule
93 & can, can, would, should, shouldn, couldn, cans, wouldn, could \\\midrule
94 & contacted, forced, failing, invalid, undefeated, eventual, wannabe, eliminated, mistaken, defeated, rejected, counted, threatened, betrayed, questioned, questionable, interrupted, respective, determined, retired, denied, sworn, backward, unwanted, suffered, convicted, imposed, refused, suggested, losing, disappeared, removed, stole, deemed, considered, associated, failed, dreamed, expelled, exploited, disappear, contradic, detained, varies, settled, falsely, dubbed, cancelled, extinct, yelled, fabricated, sustained, predicted, obtained, competing, declined, sighted, erased, delayed, reversal, canceled, calculated, deleted, expired, displaced, disguised, unlikely, disabled, elected, incarcerated, impending, suspended, occurring, originated, declared, conflicting, apparent, occurred, accused, neither, scheduled, optional, projected, exists, pronounced, possible, identical, lacking, punished, prevented, restricted, snagged, deceased, dreaded, mocked, outdated, anticipated, stolen, demolished, unnoticed, sufficient, irrelevant, resulted, refusing, illegal, acceptable, loses, accepted, backwards, ruled, exist, skipped, suppose, opposing, opposed, diagnosed, refuses, corrected, relative, separated, adjusted, known, withdraws, forbidden, traced, proven, unfair, dismissed, sought, suspected, charted, complained, qualified, unable, detected, withdraw, assumed, proposed, unclear, alleged, contested, desired, unsolved, meant, intended, recovered, transferred, excluding, limited, contained, defeating, specified, notable, repeated, aimed, assigned, concealed, overturned, abandoned, valid, conquered, infamous, unrelated, accounted, stalled, supposed, incorrect, unknown, designated, compromised, impossible, unsuccessful, unsafe, pending, expected, impaired \\\midrule
95 & arrest, jail, arrests, arresting, arrested \\\midrule
96 & civilian, intel, flannel, enlisted, honest, waterproof, intel \\\midrule
97 & tie, akes, annies, lds, lys, ws, letes, eds, urs, ghts, itters, ases, ags, rents, reds, shes, tons, aves, ts, tups, rays, acts, sts, ams, aris, phers, fts, shs, pies, ins, mats, phs, cts, icks, opes, ffs, tters, dders, bbles, sill, ons, qs, pods, bots, gents, rens, ews, stles, ries, kins, sils, ints, cers, ems, kets, wells, gens, inals, ld, wl, byes, olds, quins, ells, tles, rys, cies, dles, ots, mbles, dens, sies, oms, dits, fers, hs, tts, ute, vens, fes, ices, caps, ghs, ket, tors, nies, oos, vices, aties, dels, oods, lists, bbs, ows, gues, ns, asts, uts, aries, ours, izes, quets, rons, vies, ets, sps, bins, utes, dys, aths, ols, abs, pcs, lics, trics, irls, tle, eras, tis, elds, ats, gees, nets, gels, ands, jos, nts, ents, ures, mins, ettes, thes, zes, wers, eos, fies, chas, neys, dres, ides, rants, joes, ties, tides, stas, eves, dt, stors, ums, ames, eps, bells, acks, wines, gales, eld, ffins, fics, pubs, tonics, ills, tty, tvs, butes, bies, kens, tos, cubs, bergs, hoods, fees, ues, efs, dings, cons, omes, iners, tiers, ddings, achers, pats, prs, mists, acs, tots, gots, llers, nels, vets, leys, sties \\\midrule
98 & pa, pap \\\midrule
99 & burger, juice, lemons, steaks, taco, roti, potat, baguette, condom, canola, smoothie, guinness, shimi, tofu, dough, bananas, gelato, potatoes, sushi, nachos, sprinkles, oysters, berry, bologna, icecream, cucumber, beetroot, grape, cranberries, cheeseburger, grains, crepe, truffle, carrot, marbles, pickles, pebbles, onion, spices, sauce, crisps, onions, coca, mince, broth, stea, muffin, pork, garlic, coffee, cardam, gravy, pepper, marble, custard, thyme, cinnamon, saffron, lemon, beans, nuggets, tomatoes, parmesan, seaweed, pie, milkshake, celery, sandwiches, masala, desserts, porridge, cactus, toast, sprouts, blackberry, candies, dessert, pea, frosting, almond, lettuce, bacon, carrots, cranberry, ketchup, potato, tomato, slime, casserole, yogurt, garbage, sandwich, mango, honey, bagel, ginger, berries, chutney, breads, truffles, cocoa, biryani, nacho, salads, jelly, vanilla, salad, toothpaste, pumpkins, soybean, tart, gluten, butter, pork, sausage, heroin, bread, creme, lime, supper, toffee, squash, raspberry, cider, herbs, fillet, ffel, meatball, pastry, stew, marshmallows, mousse, grapes, dominos, strawberry, scotch, lasagna, beetro, peas, bean, lilac, soup, cream, pints, tortilla, soda, pineapple, raisin, nutella, probiotics, turmeric, salsa, miso, hamburger, basil, kimchi, meat, popcorn, leek, peanuts, clams, fruit, pancake, pearls, fondue, blueberries, iyaki, cereal, coconut, oyster, hotdog, charcoal, diamonds, eggplant, bubblegum, fleur, flakes, steak, tacos, banana, beets, asparagus, spinach, burritos, cherries, mushrooms, biscuit, clam, cookies, curd, beet, biscuits, olive, syrup, potion, fruit, crayons, pancakes, meatballs, peanut, creams, lavender, crayon, pumpkin, tarts, lollipop, spaghetti, sausages, pizza, herring, tuna, beer, maple, onnaise, gnocchi, spears, corn, granny, sirloin, sesame, muffins, cheese, lemonade, crumbs, poppy, marrow, mushroom, burgers, protein, milk, waffles, wheat, sundae, meats, digestive, crackers, pickle, smoothies, pepperoni, ginger, sprite, gingerbread, pizzas, cookie, crystals, watermelon, marshmallow, candy, quinoa, beef, burrito, kebab, barley, dynamite, cherry, snowball, sweets, vinegar, ricotta, caffe, blondie, chips, plum, paprika, gummy, vodka, bagels, citrus, relish, omelette, intment, cabbage, fruits, adish, sauces, bread, strawberries, cucumbers, mackerel, rum, papaya, snickers, melon, oranges, pudding, dumplings, pastries \\\midrule
100 & distinguished, highly, extremely, outstanding, exceptional, exceptionally, exemplary, extraordinary, sional, excellence, significant \\\midrule
101 & colouring, coloring \\\midrule
102 & ornaments, cables, keychain, whistle, sleeveless, frock, champagne, scarf, pencil, ribs, earrings, wrench, curls, sneakers, thighs, saddle, jackets, apron, umbrella, knobs, choker, smartphone, shovel, palette, purse, dice, sock, knuckles, ribbons, elbow, mustache, cleanser, jeans, hipsters, sandals, scrubs, beads, backpacks, strap, pullover, sax, laptops, pajamas, leash, garments, perfume, pant, sleeves, headphone, denim, pendants, antlers, braids, bracelet, kimono, wallet, bouquet, headlights, socks, wrist, suit, suv, skulls, stocking, pencils, lace, laces, converse, condoms, accessories, knees, eyelashes, necklaces, sunscreen, pants, mascara, sleeve, necklace, sweats, stripes, wedges, vase, headband, bruise, flats, medal, braid, jacket, eyeshadow, lashes, lipstick, coasters, nipples, guitars, visor, cheque, shoe, tiara, robe, onesie, beers, garment, sandal, straps, earring, candle, flask, braces, handbag, heels, headphones, badge, nipple, slippers, lenses, knuckle, breasts, sunglasses, logos, vests, ukulele, footprints, romper, earphones, glasses, shoes, straws, shawl, hijab, specs, textbooks, cardigan, wrist, thong, stationery, saree, shoulders, tires, culars, bangs, foal, corset, zipper, candles, fedora, cigarette, flares, cleavage, manicure, leather, swords, eyeliner, wallets, plaid, tissues, cuffs, pillows, cleats, fabrics, beanie, umbrellas, boots, scarves, pinky, tyres, balloons, monogram, heel, putter, jewelry, pens, chairs, trunks, harness, ankle, thigh, muscles, moustache, knives, scissors, ankles, calves, tights, forks, halter, stockings, luggage, cigarettes, rims, pedals, boot, smartphones, collar, trousers, feathers, cuff, panties, lanyard, appliance, jumpsuit, cologne, cruiser, headset, stripe, soles, goggles, accessory, footwear, backpack, veins, cloak, handbags, clothes, ribbon, wigs \\\midrule
103 & continues, continue, beginnings, portions, beginning, revolution, chapter, continuing, continued \\\midrule
104 & smuggling \\\midrule
105 & sc, s \\\midrule
106 & sse, ss, ssi, ssc \\\midrule
107 & flash, flash, flashes \\\midrule
108 & report, allegations, reported, reports, reporting, updating, updates, update, inform, predictions, forecast, testimony, prediction \\\midrule
109 & d, ray, ady, cd, reed, di, dart, d, dd, ddle, du, dell \\\midrule
110 & s, fs \\\midrule
111 & saf, ff, az, fis, af, f, fi, if, ef, waf, baf \\\midrule
112 & silver, silver, gold, copper, steel, bronze \\\midrule
113 & layout, finals, pair, tasks, selection, surgery, practice, attire, team, demo, efforts, task, craft, exercise, pilot, shift, skills, tour, mode, working, draft, batch, comp, goals, recipe, work, skit, skill, trip, job, edit, routine, copy, project, scenery, recruit, tweak, kit, chores, fail, tool, crews, tricks, workout, ateam, edits, quiz, prototype, therapy, hustle, skill, incident, course, meetup, haul, motion, iteam, prep, edition, injury, budget, tools, remake, toolkit, labour, hardwork, trial, jobs, session, scheme, tutorial, schedule, phd, labs, entry, kits, process, cycle, failure, ceremony, clinic, squads, team, feedback, delivery, practise, homework, stest, contest, exercises, practices, mess, projects, stunt, teams, rehearsals, hire, degree, exam, yoga, effort, rehearsal, training, routines, teamwork, supply, collaboration, grind, style, goal, collection, works, action, ritual, protocol, activity, tactics, trainees, workshop, warmup, duo, roster, version, duties, actions, tutorials, labor, rituals, trials, squad, work, duty, event, overtime, sessions, lab, howto, gig, diet, exams, throwback, crew, helpers, workouts \\\midrule
114 & males, male, female, females \\\midrule
115 & broken, ripped \\\midrule
116 & distributed, retailer, distribution, distributing, distributor, representation, distributors, dealership, implementation \\\midrule
117 & leone, nie, ines, rice, stine, tine, niki, ine, ene, stle, ingle, naire, ine, aine \\\midrule
118 & mar, erie, ital, cn, chan, sin, ium, anti, et, lon, din, dom, tti, dic, sur, dn, uit, semi, quin, ren, nn, han, tan, vin, van, dem, ian, bin, ens, dron, aman, sian, en, gin, tian, pian, lan, ir, vor, gen, fin, len, ban, wen, cian, lyn, nan, den, aux, wan, ham, ult, hin, ssen, ev, wn, een, rin, dans, ton, ian, leton, hem, shin, mel, mir, nin, nier, wee, mann, stal, tre, em, enne, raj, cen, ston, lum, con, ven, bian, jin, dian, chen, nis, aston, eng, yan, ardo, mon, elli, eed, anian, yen, mont, lian, mit, ison, ort, oot, athan, yn, rien, und, von, ion, ni, nel, tans, ein, sham, sn \\\midrule
119 & head, headed, head, heads, heading \\\midrule
120 & bun, bun, buns \\\midrule
121 & wear, wear \\\midrule
122 & hou, ho, kim, hoo, tho \\\midrule
123 & qua, ike, tov, reau, bon, twp, mono, ioc, urt, oxide, taw, wak, akin, ido, dote, yne, kung, mier, bide, tonic, olor, bey, vide, pico, mach, asin, sung, coll, yaki, cdc, sette, ome, whi, zell, cade, ound, lieu, pone, singh, ooh, aron, illin, pong, cle, abu, watt, shaw, sune, levin, ican, dim, poon, pans, kalyan, ntv, atti, aloud, lidge, ggly, tri, lac, kly, ende, guk, tur, comb, gil, avan, dine, tipton, quette, teed, nae, itten, fic, downey, dant, ghee, ande, pon, awal, gol, nep, acle, tronic, aos, tant, inous, zzie, oue, nay, tary, gama, pires, grande, tema, goa, rood, tate, olson, chino, quet, durant, tosh, iton, tye, abou, ril, gam, bono, mple, alter, bain, oor, pan, dden, phan, hone, wati, deo, liver, tern, sine, bates, vail, oll, gely, funk, pol, caine, aut, allen, minton, bate, eyre, lete, lic, pinto, ghe, wnt, atee, sium, fore, nish, duk, ust, rial, toms, amp, aten, tem, lung, inan, maging, reno, ual, giri, garde, akan, nik, itchen, aty, loin, tose, tiff, edon, leon, thm, atoms, yong, ought, chner, coli, tir, acco, mbo, deg, elen, ellin, derby, hutch, lop, dyer, ern, havan, atten, gogo, moulin, vig, gong, sew, xin, oat, duce, bard, orient, inette, ateur, caste, hore, liu, cane, inge, cket, gano, ggan, akis, dion, gli, wain, cal, olin, agame, uke, rove, monds, rot, sone, foe, erina, rae, agarwal, tache, dow, brite, otta, outer, uci, tome, llo, wad, nene, lam, rette, cystic, vion, tong, bib, oling, abd, yed, qing, loe, vey, chee, chow, tawa, crae, dol, nar, hanks, ide, soy, atom, oose, hew, bord, igan, dion, nye, cinco, onex, pun, bg, isch, edy, verde, eon, hind, fro, cone, isc, tait, ckey, agos, frey, dame, twine, notre, tric, elie, idge, zee, ince, stig, brane, vial, ove, ingham, lok, dess, devi, roux, mance, adic, paco, inee, foo, fins, oke, dall, mund, tise, ough, gland, newton, ilio, tify, oom, ode, kees, hays, polk, aton, quist, ape, hol, ffin, rid, dred, kap, ime, chum, cino, fats, bou, onent, shp, avant, dely, num, weiler, tue, fre, awan, nex, dag, omega, ather, ilian, dair, gart, gue, igh, fron, ween, ean, atri, anil, pel, kke, minh, yon, icial, yoke, seum, nad, chor, jfk, illie, dal, gale, pras, geon, lager, yte, rive, zinc, colt, liet, tet, ulo, kang, yam, oun, cann, rang, mone, elic, acles, ild, ives, yani, spi, mak, deon \\\midrule
124 & interview, conferences, interviews, lectures, testifying, interviewing, interviewed, articles, pipelines, languages, styles \\\midrule
125 & smell, taste, flavor, tastes, smelling, smells, tasted \\\midrule
126 & wanna, wanted, wants, want, wanting \\\midrule
127 & cc, ac, ic, ec, pac \\\midrule
128 & ak, gra, ag, poke, ig, aga, coo \\\midrule
129 & assemble, assembling, gather, packing, assembled, gathered, assemb, organizing, gathering, assembly, gathers, organize \\\midrule
130 & sio, tora, ama, ma, atas, lama, iam, tia, mat, grams, mass, vane, mna, vah, gma, cena, qa, nova, amma, inga, illas, vil, aria, vea, casa, anda, amas, oma, stri, abra, mba, bri, mars, cruz, tras, sil, val, sari, ayo, vita, lla, ias, rella, asis, gala, rim, kali, masa, vada, halla, eta, kai, santa, tivo, epa, phia, atha, sis, sal, natal, aura, va, thy, ange, itian, ira, mal, pia, eba, inda, elia, adas, alea, tum, aqua, ronda, sama, cara, khar, ada, gram, kka, mana, kia, dah, atus, alba, elisa, aque, boa, vista, tona, andra, kal, oris, ula, yana, taj, mas, ibn, coma, anas, fia, ava, sha, char, pta, anga, unas, mia, kasi, cma, lala, mara, sta, uda, manga, mati, eva, gara, rax, bras, paa, bora, aba, esa, ima, nas, teria, juana, dum, mino, nia, lor, asa, ata, ala, kan, tam, vale, arium, sata, kara, dana, rana, wal, hana, taya, lea, moma, bra, acia, gura, leia, arma, maya, bex, forza, mania, lara, inal, jama, para, anta, mai, var, mam, sus, dra \\\midrule
131 & wash, washing, washer, washes, wash, washed \\\midrule
132 & egg, eggs, egg \\\midrule
133 & gymnasium, preschool, class, nurses, school, junior, auditorium, teachers, homecoming, elementary, senior, academic, prom, church, conference, scholar, class, college, cafeteria, students, kindergarten, mcdonalds, schoolers, hospital, graduates, orphanage, teacher, scholars, classmates, starbucks, graduating, freshmen, schools, highschool, university, institute, seniors, graduation, student, classrooms, school, campus, faculty, graders, household, educators, colleges, bachelor, nursery, classes \\\midrule
134 & sanitary, sanitation, plastic, groundwater, dialysis, detergent, menstru, diagnostics, operating, semiconduc, radiation, plastic, pesticides, moisture, membrane, islamophobia, infrared, porcelain, menstrual, thermal, glucose, malaria, chemicals, plastics, optical, semiconductor, tornadoes, electronics, optic, antarctica \\\midrule
135 & mother, mother, mothers \\\midrule
136 & bio, bio, profile, bios, biography \\\midrule
137 & batman, bat, donkey, bot, batting, bat, bats \\\midrule
138 & tering, button, tter, iner, ters, ter, ometer, amer, copter \\\midrule
139 & mesmerizing, rad, killer, awsome, funniest, stunning, dazzling, breathtaking, flawless, fascinating, tremendous, outrageous, terrible, amazing, devastating, genius, amusing, masterful, magical, unbelievable, marvelous, speechless, thoughtful, awesome, great, inspiring, awful, entertaining, interesting, spectacular, innovative, motivating, horrible, terrific, amaze, thrilling, wonderful, exhilarating, sensational, talented, ridiculous, greatest, enthusiastic, superb, unreal, frightening, powerful, impressive, inspirational, amazingly, epic, intense, brilliantly, majestic, heroic, hilarious, excellent, fabulous, astonishing, exciting, horrific, magnificent, brilliant, incredible, remarkable, fantastic, brutal \\\midrule
140 & settlers, folk, servants, survivor, tourists, personnel, worker, human, fellows, viewer, somebody, civil, inmate, individual, peoples, witnesses, immigrants, victims, relatives, attendant, competitor, persona, species, human, captivity, parents, pedestrians, addicts, neighbor, follower, roommate, user, employee, user, customers, crowds, patient, yorkers, strangers, person, parent, victim, religious, explorers, motorists, persons, voters, folks, muslims, hindu, humans, someone, patron, veterans, subscriber, listener, servant, pilgrims, coworkers, passengers, person, beings, migrants, academics, enthusiast, employees, pupil, enemies, roommates, haters, patrons, newcomers, opponents, natives, followers, spectators, voter, civilians, caregivers, people, users, holders, colleagues, cashier, demographic, peeps, neighbors, crowd, individuals, workers, residents, adults, prisoner, population, foreigners, subscribers, adolescents, classmate, inhabitants, gender, adult, inmates, locals, viewers, citizens, survivors, troops, refugees, infants, pupils, opponent, feminist, passenger, refugee, prisoners, ancestors, customer, watchers, goers, bystand, supporters, speople, neighbour, villagers, tourist, peasant, spectator, patients, parental, peasants, lovers, physician, shoppers \\\midrule
141 & sands, sand, sand \\\midrule
142 & dance \\\midrule
143 & drops, dump, drop, dro, orbit, dropped, dropping, drop \\\midrule
144 & practitioner, personal, leadership, expertise, speciality, authenticity, entrepreneurship, profession, lifestyles, professi, experts, specialty, professional, adventures, professionally, expert, innovations, professionals, profession, authentic, invention, career, careers \\\midrule
145 & jaguar, blur, blurred, muted, blur, blurry \\\midrule
146 & research, researching, resear \\\midrule
147 & ati, iti, atu \\\midrule
148 & ro, ros \\\midrule
149 & surf, surfer, surfers, sur, surf \\\midrule
150 & sy \\\midrule
151 & swim, swim, swimming \\\midrule
152 & sons, daughter, daughters, son, grandmother, grandma, grandson, grandpa, ghter, grandparents, granddaughter, grandfather \\\midrule
153 & als, ial, aling, aters, ais, rers, mals, irs, vels, aked, alds, aks, ials, ticals \\\midrule
154 & story, reality, weather, view, meme, scandal, theme, media, evidence, poverty, broadcast, comedy, sport, signal, warning, gems, narrative, feminism, magazine, petition, health, rpg, crisis, databases, tv, math, broadcasting, autobiography, anatomy, gofundme, election, tickets, ethics, discount, newscast, journal, science, logic, hashtag, scare, crime, opinion, classics, fiction, essays, article, maths, rhyme, appeal, loid, subject, econ, title, page, facts, headline, buzzfeed, fanfic, podcasts, novel, textbook, democracy, novels, news, pages, bible, discourse, propaganda, sexism, deaths, questions, news, rights, calendar, msnbc, sport, sports, drama, truth, account, chart, captions, awards, humor, word, opinions, quest, television, foxnews, psychology, comics, ethic, sports, poem, fashion, parody, blogging, amovie, referendum, mystery, sitcom, public, agenda, prophecy, satire, email, column, trend, survey, lyric, spam, link, cultural, quote, phrases, playlist, geography, gps, disease, writings, script, virus, chronicle, cnn, scoop, question, trivia, iteracy, headlines, warnings, legacy, campaign, bulletin, tales, spoiler, dialogue, accounts, stories, quotes, postcard, racism, gov, search, ticket, wiki, newspaper, message, thread, skynews, apology, letter, history, criticism, hobby, health, phrase, confession, deadline, medicine, internet, tragedy, letters, poetry, enquiry, justice, content, newspapers, login, complaint, blogs, nature, puzzle, drugs, arts, database, algorithm, autograph, diary, link, conspiracy, traffic, editorial, onews, horror, trending, disaster, trends, genre, caption, blogger, azine, physics, gospel, gossip, advice, fauna, theory, topic, statistics, essay, messages, climate, messaging, memes, bloomberg, radio, culture, gmt, crimes, epidemic, sermon, biology, decision, slogans, magazines, titles, award \\\midrule
155 & figh, combat, fight, killing, battle, battles, fight, fights, fighters, fighting, fighter, fought, battling \\\midrule
156 & outdoors, upstairs, outside, downstairs, infront, indoor, opposite, poolside, inside, underground, backyard, overhead, exterior, outdoor, somewhere, anywhere, outdoor, patio, indoors, surroundings, daylight, onboard, courtyard \\\midrule
157 & ver \\\midrule
158 & kardashian, khloe, kardashi \\\midrule
159 & profiles, appeared, cameo, including, previews, staring, contain, feature, teased, depicting, glimpse, featuring, depicted, features, teasing, teases, starring, feat, teaser, nestled, preview, participating, starred, predicting, poking, depicts, stared, targeting, appearing, debuted, featured, included, tease, headlining, accompanying, appearance \\\midrule
160 & ken, ken \\\midrule
161 & arian, ar, ar, ars, ara \\\midrule
162 & mines, hers, miners, mine, mining, minerals \\\midrule
163 & cre \\\midrule
164 & rallying, ailing, rally, piled, nationwide, campaigning, rallies, picket, trailing \\\midrule
165 & ariel, kr, r, rs, rr, r \\\midrule
166 & dc, cs, c, cc, cl, cr, cl, ct, ct, cent, nc, bc, cw, duke, ac, sc, sci \\\midrule
167 & swi \\\midrule
168 & visiting, guess, notice, heard, visits, sees, discovered, receive, meets, knows, noticing, met, see, seeing, find, visit, wears, finds, meet, peek, grab, seek, spy, saw, see, found, seen, browse, visited, witness, join, hear, spotted, know, view, hears, witnessed, meeting, realize, knew, noticed \\\midrule
169 & ke, ko, kal, ka, kar, kad, kan, kaz \\\midrule
170 & down, down, downs \\\midrule
171 & musician, music, melody, language, music, hiphop, lyrics, tunes, musicians, entertainment, musical, tainment, soundtrack, musi \\\midrule
172 & tes, ttes, que, te, ta, tas, mble, ques, que, atin, tres, ffle, ote, teo, tta \\\midrule
173 & mashup, remix \\\midrule
174 & embarrassed, embaras, humili, embarra \\\midrule
175 & leggings, kini, swimsuit, bikin, apparel, sportswear, clothing, bikini, swimwear \\\midrule
176 & pinning, spoon, pin, pin, pinned, pins \\\midrule
177 & tale, clue, base, deal, aid, note, fix, tax, born, word, tag, fits, cost, lost, half, exit, name, count, card, cure, stock, alone, match, term, matters, share, weight, level, worth, alike, sight, target, apart, usage, bid, round, minus, purpose, proof, otes, laws, fit, rules, scale, limit, act, matter, due, case, wave, rip, ease, code, feast, kick, edge, rate, rise, way, use, far, hint, ounce, saving, beat, dating, native, rates, kill, save, counts, step, spell, number, date, cases, law, force, risk, text, ounces, volume, sure, lead, loss, trick, value, sums, meaning, pace, bonus, notes, rival, idea, wait, names, offs, saves, map, guide, grade, ways, aside, fact, list, move, reason, safety, verse, dates, order, amount, ages, mistake, sake, reward, pre, credit, numbers, fund, lose, words, alert, dollar, birth, ahead, age, cards, prize, source, row, codes, saved, rule, terms, role, phase, lot, money, error \\\midrule
178 & slowed, split, trimmed, transported, warped, toned, sunken, shaved, trough, quilted, skinned, clad, sewn, edged, shredded, raced, scripted, crowned, tamed, laden, hooked, scrambled, peeled, occupied, adorned, polluted, divided, submerged, braided, wounded, fade, eaten, buried, dyed, mashed, hooded, tinted, haunted, dented, scanned, battered, spoiled, escaped, molten, sealed, dotted, drowned, waved, bankrupt, reunited, spiked, struck, parked, striped, energized, corrupt, kicked, suited, bullied, warmed, draped, faded, bleeds, wound, coupled, scaled, chilled, curled, drilled, possessed, narrated, tainted, jailed, tattooed, bowed, stuffed, overflowing, jacked, wrecked, smoked, refreshed, laze, crushed, engul, smashes, dipped, tortured, muddy, rigged, smashed, abused, brushed, dragged, stacked, shank, drenched, tackled, slit, altered, ruined, padded, burst, photoshopped, slammed, fired, scratched, healed, studded, armed, jammed, dried, infused, kidnapped, deserted, vacant, anchored, chained, squeezed, curved, anned, canned, preserved, footed, landed, strapped, reversed, sown, melted, shut, laced, drained, hydrated, explodes, beaten, lifted, infected, collapsed, raped, starving, assaulted, wet, glued, hospitalized, bundled, swallowed, clipped, contaminated, drunken, staining, split, torn, amped, unwind, perched, priced, bottled, shifted, uncut, bodied, stabbed, tore, dumped, ridden, slain, walled, melts, soaked, sweating, censored, bleed, crooked, colorized, shaded, smash, potted, mounted, sprayed, burnt, slapped, snatched, prized, blinded, peaked, cured, woven, wasted, slept, burnout, swollen, fading, crusted, shred, sped, naked, swept, whipped, barred, damaged, murdered, sunk, leaking, poured, strung, sparked, sank, sacked, leftover, exposed, killed, stitches, pregnant, rushed, horned, destroyed, towed, tucked, athered, invaded, feral, robbed, fled, sweaty, cursed, consumed, explode, untouched, pumped, tossed, patchwork, paced, cycled, stripped, stitched, prepped, hyped, burned, twisted, grounded, rested, tangled, spilled, housed, messed, choked, lowered, leaked, intact, drown, scattered, detox, docked \\\midrule
179 & classroom, studio, gym, workplace, apartment, interior, library, showroom, workspace, bedroom, entrance, studio, office, suite, staff, office, desk, salon, station, dorm, kitchen, microsoft, restaurant, retail, laboratory, service, offices, newsroom, hq, lobby, interiors, chamber, desktop, apartments, dept, studios, department \\\midrule
180 & tor \\\midrule
181 & pad \\\midrule
182 & techno, technical, robotics, theft, tech, tech, innovation, techn, itech, technology, techno, technician, technologies, stech, technological \\\midrule
183 & gan, san, gin, an, san, ana, gan, alan, ram \\\midrule
184 & wizard, wizards \\\midrule
185 & designing, fabric, wooden, handwriting, designs, painting, design, drawings, ceramic, prints, wallpaper, maps, decoration, paints, etching, welding, origami, paint, sketched, decorating, pottery, knitting, embroidery, mapping, drew, draw, drawing, doodles, artwork, carving, sculpted, decorate, ceramics, beaded, painter, canvas, paint, drawn, knit, design, knitted, woodwork, acrylic, ornament, decal, lettering, rendering, carve, paste, clipping, handwritten, painted, stitching, art, machining, sketch, decor, crafting, paintings, sketches, marker, doodle, collage, carvings, decorations, decals, sculpting, caricature, carved, miniatures, crafts, draws, crochet, drawing, stencil, sculpture, cosplay, canvass, art, murals, artworks, sculpt, decorated, sketching \\\midrule
186 & gl, gen, lu, hol, gh, gi, dg, glo, ga, gla, ggy, g, gg, g, gol, gle, gs, eg, gil, gn, gg, gy \\\midrule
187 & walton, rivers, shore, waters, hooks, waves, hook, powers, warrior, shore, beaches, shores \\\midrule
188 & hanged, hang, hangout, hanging, hangs, hang, hangin, hung \\\midrule
189 & play, play \\\midrule
190 & hand, hand, hands \\\midrule
191 & elder, elder, elders \\\midrule
192 & da, daf \\\midrule
193 & flat, flat \\\midrule
194 & spe \\\midrule
195 & pur, du, pu, rol \\\midrule
196 & se, nas, sel, ve, te, bin, leg \\\midrule
197 & promo, promoting, promote, publicity, promo, promotional, promotions, promotion, promoted \\\midrule
198 & bor \\\midrule
199 & chandra \\\midrule
200 & calories, previously, freshly, plumbing, halftime, midway, technically, tallest, calorie, halfway, unexpectedly, kilometers \\\midrule
201 & snacking, snack, snacks, snack \\\midrule
202 & ggi, ng, cgi, lang \\\midrule
203 & ssy, gy, sy \\\midrule
204 & naruto \\\midrule
205 & hill, earth, bluff, plain, moun, plains, hillary, hills, hilly, cloud, dale, ridge, mt, mountain, hill, moon, mole, mound, bell, foothills, gulf, hills, cape, mount, hillside, liberty, mountain, mineral, ridge, hilltop, mt, monte, earth, volcano \\\midrule
206 & locks, key, key, keys \\\midrule
207 & listen, watch, watches, streaming, watching, watch, stream, streams, listening, watchin, listened, listens, streamed, watched \\\midrule
208 & dolphin, dolphins \\\midrule
209 & air, air, ir \\\midrule
210 & suns, sun, sunshine, sun, sunlight, sunny, solar, vijay, moon \\\midrule
211 & major, eddie, huge, giant, lil, big, enormous, gigantic, bigger, bigg, large, wide, biggest, massive, largest, jumbo, larger, big, giants \\\midrule
212 & appears, recognize, attracts, pronounce, threatens, demonstrates, revealing, encouraging, defeats, prompted, invited, encouraged, joins, indicate, highlights, extends, occurs, shouts, understands, mentions, shouted, expressing, surrounds, replaces, identify, confirming, convey, exposes, uncovered, involves, fyi, solves, declare, acknowledging, represent, resembles, declares, apologize, endorse, advise, ignores, recaps, praises, consists, according, ignore, pleads, denies, maintains, obvious, expresses, interested, identifies, appear, regards, appreciating, recognized, involving, agrees, accepts, notices, begs, identifying, noted, destroys, stating, endorses, advises, defends, insult, include, reminiscent, writes, accept, condemns, invite, appreciates, boast, understood, admitted, appealing, disclosed, acknowledge, proposing, praised, invent, informing, depends, plead, proposes, accepting, contributes, participates, mention, provides, involve, relating, admitting, indicates, concluded, informed, agree, owns, whispers, appreciate, mourns, represents, praising, proceeds, thanking, highlighting, reveals, mentioning, containing, refers, indicated, prefers, abound, witnessing, inviting, mentioned, encourage, proves, diagnose, directs, accusing, proclaimed, resemble, justify, criticized, expressed, thanked, admits, apologizes, entitled, specializes, exposing, exclusive, suggesting, translates, prompts, avoids, accuses, owes, suggests, allows, approves, predicts, versus, dismisses, courtesy, attends, accommodate, guessed, revealed, confirms, criticize, receives, complains, highlighted, consist, citing, noting, determines, admit, bragging, includes, relates, ignoring, respondents, boasts, informs, defines, congratulation, warns, discovers, endorsing, honored, quoting, applies, interrupt, realizes, invites, contains \\\midrule
213 & master, widows, nazi, emen, dodgers, barber, lion, danger, beard, avenger, horrors, marine, fiends, hawks, racist, tress, reverend, jihad, rams, fools, superman, mans, horns, elves, minions, hitman, terror, groom, pioneer, goat, boss, gorilla, man, emperor, angels, war, heros, betrayal, doom, idol, martyr, samurai, souls, hawk, mistress, chap, elite, guard, legend, trek, gangster, eaters, junkies, holmes, saints, hero, stranger, ravens, freeman, guru, man, nun, banger, sailors, cancer, dragon, monster, guyz, sins, grinder, godfather, butcher, brains, christ, assassins, scum, goblin, raider, creed, ghoul, bearded, guardian, clown, rat, deman, babs, beast, demons, jester, tribes, goon, soldier, jesus, pion, prophets, god, ghost, thugs, rockets, lambs, mafia, cyborg, jones, hog, mage, uncle, oness, rapist, protector, priest, undead, beards, gangs, gang, thieves, titan, witches, aunt, hammer, panthers, itans, hells, diva, liar, hero, finder, tman, villains, merchant, defenders, oldman, wolf, bulls, bullets, trooper, slave, bald, pawn, riot, monk, assassin, slayer, coward, goddess, shepherd, chman, maniac, unner, menace, maid, goth, death, vader, murderer, masters, derman, knight, witch, thug, hounds, trolls, pillars, dons, hogan, feud, foes, filth, rangers, khan, killers, rebel, lowes, rats, titans, maiden, wars, cop, monarch, goons, banker, mule, elf, legends, dealer, fox, jew, anger, mane, raid, joker, slaves, soldiers, bandit, idols, knight, fool, potter, horde, bond, dragon, fury, lions, craftsman, bridal, thorns, tribe, eater, monsters, jews, shepard, dman, anist, grim, thief, gods, widow, digger, stag, lynch, sailor, heir, serpent, beatles, punks, predators, smen, dagger, boar, psycho, generals, puppets, dummies, lion, angel, sharma, maniacs, preacher, murder, negro, enemy, beasts, hornet, strife, ripper, cops, vikings, ssor, reaper, fist, troop, knights, robber, spurs, thorn, hermit, nazis, ghosts, raiders, marines, heroes, junkie, mayhem, trader, hound, fireman, scout, comrades, greed, rebels, buster, busters, starwars, dwarf, punk, pioneers, falcons, jokers, lord, bull \\\midrule
214 & guests, visitor, visitors, guest \\\midrule
215 & finish, progress, commission, detailed, completed, finishing, paved, completes, completing, numbered, detailing, furnished, render, polished, stained, termin, finished, rendered, complete, unfinished, finishes, resting, renders, finisher, overall, completion, progressing, restored, incomplete \\\midrule
216 & cross, crossing, cross, crosses, crossed \\\midrule
217 & fa \\\midrule
218 & stand, stand, standing, stall, standup, stands, stood \\\midrule
219 & bottoms, top, bottom, topped, topping, atop, tops, top, highest \\\midrule
220 & folded, folds, fold \\\midrule
221 & genome, genes, gene, gene, genetic \\\midrule
222 & pharmaceuticals, biotech, biotechnology \\\midrule
223 & imagin, imagine, imagining, imagined, imagines \\\midrule
224 & imagination, uncertainty, messing, investigating, utilizing, experiments, experimental, experimenting, accidentally, experiment, risky \\\midrule
225 & prawn, shri, salmon, prawns, shrimp, chicken, lobster, seafood \\\midrule
226 & flir, flirt, flirting \\\midrule
227 & grey, grey, gray, greys, gray \\\midrule
228 & monitors, monitoring, monitor \\\midrule
229 & situation, audience, engaging, interaction, audiences, engagement, engaged, experience, experiencing, experienced, engage, encounter, interact, journey, situations, proceedings, happening, interacting, relationship, experiences, interactions, conversations, relationships, opportunities, friendships, encountered, conversation, presence, environment, encounters \\\midrule
230 & ads, ad, add, logo, advertisement, special, flyer, commercial, banners, listing, ad, adverti, advertised, rand, advertising, seeds, adds, brand, commercials, banner, advertiser, seed, advert, spon, addy, catalog, billboard, added \\\midrule
231 & tal \\\midrule
232 & demonstration, instructional, teach, pedagogy, parenting, nursing, lecturer, teaching, coaching, lecture, teaches, taught, preaching, advising, instruction, seminar, educate, teachings \\\midrule
233 & ener, fer, er, ger, sher, ther, ers, eri, terr, vern, her, met, sed, der, nel, ater, ere, ler, ze \\\midrule
234 & speeds, better, faster, speed, speed, fastest, easier, farther, cheaper, slower \\\midrule
235 & ju, jama, jum \\\midrule
236 & vegetable, kale, vegetables, veg, veggies, veggie \\\midrule
237 & wat, mun, watts \\\midrule
238 & piers, pier, boardwalk, pier \\\midrule
239 & snapshot \\\midrule
240 & ww, wr, w, aw, sw, wt, wn, ws \\\midrule
241 & slick, frozen, slippery, icy, salted \\\midrule
242 & apples, apple, apple \\\midrule
243 & analy, analyses, analysis, analyse, analytics, analyze, analyzing, analyst, analysts \\\midrule
244 & ffe, ce, ces, rees, antes, ste, sie, dez, aces, fe, se, cles, zzle, ise, bes, ree, ze, ere, pe, sche, ssel, ente, qe, ales, ash, ase, ises, ire, ges, ece, cie, bie, oe, sse, ale, ae, sel, ese, bre, aire, ses, eces, ure, ric, ires, es, gne, sso, lei, nes, rie, ess, est, ense, sage, nese, tess, Ã©e \\\midrule
245 & vid, mobile, funny, ebook, gifs, youtube, story, video, itunes, video, vid, videos, replay, vide, footage, instant, animation, trailer, visuals, podcast, videogames, infographic, trailers, audio, multimedia, viral, audio \\\midrule
246 & stroll, walked, walking, walk, walk, strolling, walkway, walks, strol, walkin \\\midrule
247 & bas, sul, bal \\\midrule
248 & talk, talking, talk, talks, speaking, talkin, spoke, speak, talked, speaks, speak \\\midrule
249 & slip, slipping, slips \\\midrule
250 & ser, ser, sen \\\midrule
251 & philippines, philippine \\\midrule
252 & sky, sky, skies \\\midrule
253 & ce, cen, cel, cer \\\midrule
254 & perfor \\\midrule
255 & octagon \\\midrule
256 & bbq, barbecue, nishings, dietary, cookery, culinary, textiles, cooker \\\midrule
257 & overseas, syrian, ghana, korea, zealand, tamil, carolina, indonesia, argentina, nepal, cuba, hawaii, egypt, american, indian, spain, baltic, india, palestinian, pakistan, colorado, nigerians, pakistani, australia, euro, atlantic, iraqi, caribbean, olympics, thai, jamaican, idaho, utah, greece, texas, indonesian, ethiopia, italians, cambodia, dutch, hebrew, cyprus, yemen, palestine, americas, soviet, uruguay, russia, greeks, disney, muslim, iranian, ireland, kenya, european, arabic, canadian, maryland, mandarin, germany, chile, greek, bollywood, wisconsin, siberian, texan, texans, missouri, foreign, migrant, roma, lankan, hollywood, malaysian, brazilian, filipino, austria, african, bengal, pacific, hispanic, usa, afghan, latino, christian, ohio, latina, finland, alabama, ethiopian, romania, americans, trans, worldcup, louisiana, arab, olympic, isis, scotland, islam, scottish, israel, nationals, iraq, arizona, brazil, israeli, iowa, nordic, venetian, gujarat, nigeria, isreal, jewish, mexico, china, naval, united, uae, british, lanka, italy, mississippi, indo, kentucky, yankees, afghanistan, slovenia, tasmanian, iceland, thailand, taiwanese, global, australian, pinoy, tanzania, immigrant, syria, arctic, belgium, finnish, egyptian, europeans, florida, japan, turkey, nebraska, islamic, arkansas, appalachian, iran, hungary, lebanon, venice, england, europe, indians, alaska, tennessee, korean, mexican, newzealand, oriental, uganda, germans, netherlands, norway, scandinavian, brasil, somali, wwii, michigan, africa, irish, nigerian, britain, orleans, persian, romanian, norwegian, rican, australians, arabs, canada, wales, africans, morocco, hawaiian, france, kansas, america, wyoming, airlines, arabian, japan, vietnam, anistan, virginia, turks, oregon, tunisia, peruvian \\\midrule
258 & upcoming, new, fresh, new, future, newer, old, incoming, nueva, recent, prospective, limited, newest, former, fresh, forthcoming, latest, current, future, updated, potential, newly, original, old \\\midrule
259 & mal, al, atal, val, lud, al, cal, gal, alco, lic, lad, tau, dal, alli \\\midrule
260 & reserve, reserves \\\midrule
261 & homeless, turnover, suicide, adoption, bonding, subscription, retiring, pollution, motoring, digestion, shopping, composing, hygiene, labeling, admission, icides, scaffolding, deforestation, dental, complaining, injuries, funding, outing, booking, clearance, transcript, costing, separation, dermatology, pregnancy, cleansing, patent, siding, logistics, holdings, counseling, clutter, banter, ruling, attendance, acquiring, homicide, seasoning, childcare, spelling, lobbying, inspection, consumption, acquisition, taxpayer, kidnapping, camping, reservations, permit, toxicity, charter, plating, borrowing, fingerprint, lending, budgeting, editing, breastfeeding, chemotherapy, servicing, finances, leisure, extraction, volunteer, commuting, harvesting, marriage, rement, grooming, bankruptcy, monetary, ership, auditions, mentoring, poaching, archival, catering, fanning, wealth, stabbing, offshore, qualifying, filtration, breeding, birthdays, cleanse, censorship, backup, touring, sales, sightings, merger, expense, sampling, correctional, registering, humidity, longing, tioning, legal, hydration, shaming, dience, clubbing, subscriptions, diversion, relocation, boardroom, conferencing, spending, uments, trucking, offense, housing, sequencing, robbery, unboxing, hiring, commuter, debt, torture, mobility, gambling, wrinkles, denial, copyright, foraging, logging, migration, wellness, negotiating, cybersecurity, spotting, nesting, appetizer, ordering, caregiver, hangover, mailing, sparring, mgmt, tagging, marriages, donation, tutoring, payer, advocacy, signaling, merchandising, detention, naming, productivity, privacy, liability, lawsuit, persecution, clause, collaborating, ownership, width, judicial, canning, thrift, refining, shipping, unemployment, slavery, misconduct, intake, abuse, recycling, lottery, fiscal, legalization, loyalty, salvage, fertility, compost, loan, abortion, suction, bidding, profiling, globalization, stuffing, education, blockchain, skincare, computing, patents, fittings, negotiation, transplant, fraud, immigration, license, salaries, consulting, poultry, adopting, reduction, forage, voucher, hostage, removal, translation, corruption, scouting, inventory, possession, audit, surveillance, adhesive, grading, citizenship, towing, sealing, cravings, surveying, volunteering, steward, cultivation, inflation, commencement, trafficking, longevity, cheating, underage, pairing, bottling, swearing, zoning, mourning, custody, induction, internship, fermentation, burial, bullying, savings, deportation, income, gation, salesman, suing, loans, spying, geology, demise, phishing, vending, conservation, expansion \\\midrule
262 & graph, graphers, graphic, graph, grapher, graphical, graphy, graphics, graphs \\\midrule
263 & falls, fallen, fell, springs, waterfalls, waterfall, fall, lake, falling \\\midrule
264 & shoo, sho \\\midrule
265 & roa, roasting, roasted, roast \\\midrule
266 & tb, b, b, bs, ba \\\midrule
267 & holo \\\midrule
268 & ru, roo, rou, skir, kru, rup, ral \\\midrule
269 & macaroni, car, mac, mac, macs \\\midrule
270 & soccer, basketball, golf, basketball, tennis, hoops, softball, lacrosse, futbol, rugby, cricket, football, golfing, hockey, baseball, gymnastics, baseball, golf, bruins, soccer \\\midrule
271 & low, higher, low, high, high, lows, slow, lower, highs, lowest, upper \\\midrule
272 & underway, starts, started, concludes, begins, start, commences, kicks, begin, began \\\midrule
273 & block, blocking, blocked, blocks \\\midrule
274 & doo, dor, do, dou, doo, vac, yogi \\\midrule
275 & hug, hugging, hugs, hugged, cuddling \\\midrule
276 & super, super, mega, ultra \\\midrule
277 & raining, rains, strom, downpour, storms, rained, misty, storm, tornado, rainy, snowing, snowstorm, earthquake, hurricane, drought, thunder, stormy, storm, rain, tsunami, storming, tornad, cyclone, thunderstorm, earthquakes, rain, blizzard, thunder \\\midrule
278 & elderly, youngster, budding, youths, oung, older, youth, youth, young, adolescent, juvenile, younger, young, youthful, youngsters, youn \\\midrule
279 & ach, dries, aches, ache, aching, achs, peppers, ached \\\midrule
280 & stur \\\midrule
281 & magni \\\midrule
282 & mama, mommy, mom, mamma, daddy, momma, papa, mummy \\\midrule
283 & live, living, live, worldwide, online, alive, lived, livestream, living \\\midrule
284 & finger, fingers, finger, thumb \\\midrule
285 & seduc, seductive \\\midrule
286 & tack \\\midrule
287 & rocking, rap, buchanan, trash, rock, rocks, rocked, rocky, ocks, rock, brick \\\midrule
288 & joke, kidding, joking, jokes \\\midrule
289 & cleaner, clean, cleaners, empty, cleans, cleaned, clean, cleaning \\\midrule
290 & silhouette, silhou \\\midrule
291 & hid, hides, hide, hiding \\\midrule
292 & hun, phar, lap, sper, henry, pi, pha, aper, per \\\midrule
293 & globe, bal, ball, balls, balling, ball, tball, baller \\\midrule
294 & hump \\\midrule
295 & rubbing, rubs, rubbed, rub \\\midrule
296 & tac, ta, tai, cho \\\midrule
297 & drives, drove, driving, drive, drive \\\midrule
298 & ths, nd, th, ther, ght, eighth, fourth, rd, th, tenth, fifth \\\midrule
299 & cla, cra \\\midrule
300 & alien, alien, aliens, mutant \\\midrule
301 & karate, taekwondo \\\midrule
302 & flow, flow, flows, flowing \\\midrule
303 & travel, tourism, traveled, travelling, travels, traveller, travel, travelers, travellers, traveling, traveler, travelled, transportation \\\midrule
304 & spinning, spin, spin, spins \\\midrule
305 & cooking, cook, chef, cooked, cook, cooks, cookin \\\midrule
306 & mixed, mixers, mix, mix, mixes, mixer, mixture, mixing \\\midrule
307 & fortress \\\midrule
308 & switches, switch, switching, switch, switched \\\midrule
309 & fire, fires, fire \\\midrule
310 & ninja, ninjas \\\midrule
311 & flint, ced, ed, ssed, ted, ted, ting, tedx, ffed, ged, edward \\\midrule
312 & bab, deli, baby \\\midrule
313 & curry \\\midrule
314 & hatchback, sedan \\\midrule
315 & mascots, mascot \\\midrule
316 & stark \\\midrule
317 & late, early \\\midrule
318 & upload, polls, post, mail, tweeting, tweet, tweets, poll, postman, uploaded, posted, posts, posting \\\midrule
319 & tiny, medium, little, small, bright, small, smaller \\\midrule
320 & camo, dong, ento, azi, gomez, alpha, ano, leche, asco, ante, ayan, tula, ane, uno, itar, jenkins \\\midrule
321 & kiss, kissing, kisses, kissed, kiss \\\midrule
322 & bit \\\midrule
323 & remo \\\midrule
324 & forces, scratches, drafts, shifts, raps, pests, clashes, acids, tokens, matches, ranks, overs, scoops, sneaks, seas, stare, clones, swims, revs, drains, strokes, sirens, ruins, strains, aids, stalls, murders, disappears, grants, backers, vents, stains, juices, hurdles, peaks, ffles, heals, streaks, shelters, alarms, buckets, salutes, longs, balances, wrecks, teas, plays, scans, allies, suits, hints, sobs, charters, pockets, dots, tiles, licks, jails, controls, billions, limbs, signals, bets, brushes, ramps, soups, cures, flee, bullies, smokes, links, loops, alizes, casualties, briefs, fails, strates, props, radius, bases, floats, combs, layoffs, relays, ropes, bursts, stems, emails, slots, rises, clocks, rests, staffs, opers, stries, dives, batteries, riots, verses, rewards, fades, stalks, spikes, charts, crises, brakes, contests, logs, prices, moves, trophies, stadiums, spells, rifles, airs, coins, specials, heats, sues, lowers, flops, chups, tours, wounds, rushes, accents, rhymes, cues, views, jewels, dunks, crushes, spoils, primaries, orders, stroke, puffs, leaps, levels, insults, wipes, scales, mentors, broadcasts, spires, beams, samples, spoons, pounds, rounds, errands, eats, costs, exits, rts, swings, ancers, waits, reps, paces, oils, spares, strips, stacks, laps, surfaces, filters, deposits, stewards, treats, sticks, shrubs, reels, minors, masses, spends, pairs, clubs, dumps, soars, extracts, depths, supplies, kills, mands, pulses, creeps, dishes, commands, rollers, cylinders, patrols, cubes, texts, globes, lants, cones, speeches, bolts, contacts, mocks, staples, peers, fuels, grades, antics, slopes, lifts, resumes, inches, searches, steps, paths, gains, selects, commits, shines, quests, angles, splits, prizes, poses, rages, spreads, pokes, discounts, anchors, plets, curves, settles, favorites, grabs, unrest, footsteps, leans, sources, labels, guards, clicks, stunts, limits, grooves, winds, courses, nests, taps, rivals, solids, pours, stares, cruises, sights, preps, escapes, puzzles, snippets, ounts, dyes, icons, bids, twists, collapses, deals, teasers, spies, takers, guides, slays, plight, pennies, receipts, cords, savers, perks, harms, suites, sprints, scams, buffs, scapes, hops, spills, wares, rebounds, upsets, hires, lengths, thrills, dues, desses, grips, alies, stakes, spans, cutters, funds, advances, slaps, moons, shares, sings, leads, copies, jams, digits, surveys, sinks, roles, dips, oldies, fashions, scripts, traces, blondes, sheds, losses, trusts, bonds, branches, accidents, drags, colonies, flavors, playlists, whoops, spree, barrels, tags, cels, seizures, noises, rods, edges, crops, taxes, fines, breeds, fuls, sweeps, musicals, gases, modes, raids, lunches, planets, sacks, missiles, haves, sunsets, bucks, pumps, doses, sidelines, bounds, brews, totals, unders, metals, bonuses, dimes, ticks, miles, touchdowns, cells, fixes, clans, fronts, stocks, routes, dents, clusters, circuits, tages, bills, shuts, warts, tabs, germs \\\midrule
325 & fro, cro \\\midrule
326 & chocolate, cupcake, cake, chocolates, cake, cakes, cupcakes \\\midrule
327 & levit \\\midrule
328 & accessing, education, discovery, learns, learn, finding, learned, learning, hearing, growth, understanding, earning, knowledge \\\midrule
329 & pol \\\midrule
330 & spo \\\midrule
331 & shadows, shadow, shadow \\\midrule
332 & placing, putting, puts, put, ttin \\\midrule
333 & ha \\\midrule
334 & rece \\\midrule
335 & murray, berkeley \\\midrule
336 & ate, ite, ated, eat, ast, ating, ates, ated, ites \\\midrule
337 & greeting, greets, welcomes, greet, welcome, welcomed, welcoming, greeted \\\midrule
338 & toys, packs, boxed, packaging, bag, packages, bags, package, box, boxing, box, boxes, pack, envelope, packet, pkg, cardboard, packets \\\midrule
339 & express, expre \\\midrule
340 & blow, blow, blows, blown, blowing, blew \\\midrule
341 & automatically, continuous, automated, automation, automatic \\\midrule
342 & roads, road, streets, road, highway \\\midrule
343 & eating, smoking, wine, drinking, drin, drinks, drink, married, drank, beverage, smoke, sipping, alcohol, dining, drunk, beverages \\\midrule
344 & objects, pieces, goodies, object, something, parts, buttons, bit, chunks, items, bobs, bits, stuffs, abit, attached, item, thing, goods, things, discs, particles, somethin, related, gadgets, crap, thing, piece, chunk, spheres, stuff, detail, something, creations, part, scraps, critters, joints, happenings \\\midrule
345 & lo, l, yl, ll, el \\\midrule
346 & chu, chun \\\midrule
347 & plant, flowering, flower, blooming, bloom, flower, blooms, petals, floral, plants, blossom, flowers, harvest, blossoms \\\midrule
348 & heavenly, heaven \\\midrule
349 & marijuana, cannabis \\\midrule
350 & myself, selves, himself, yourself, self, oneself, self, themselves, ourselves, herself, itself \\\midrule
351 & template, framed, frame, framing, frames \\\midrule
352 & mor, battle \\\midrule
353 & followed, follow, following, follows \\\midrule
354 & closing, closes, closed, closure, conclusion \\\midrule
355 & ice, iced, ice \\\midrule
356 & inhabit, adaptation \\\midrule
357 & injured, hurt, hurting, hurts \\\midrule
358 & dun, wool, dur, lang \\\midrule
359 & dress, dresses, dressing, dressed, dresser, dress \\\midrule
360 & masked, masking, mask, mask, skull, masks \\\midrule
361 & reflects, mirror, reflect, mirrors, reflection, mirro, reflected, reflecting, reflective, reflections \\\midrule
362 & calling, call, call, calls, called \\\midrule
363 & kittens, kitten, dogg, doggie, doggy, bunny, piggy, puppies, pup, pig, dogs, canine, pups, dog, kitty, puppy, dachshund, pony, pug, adog, ponies, cat, pigs, dog \\\midrule
364 & sponge, sponge \\\midrule
365 & kes, ek, ke \\\midrule
366 & voiceover \\\midrule
367 & belle, bol, pil, chor, bel, bell, bul, gall, sla, mel, stock \\\midrule
368 & slide, slide, slides, sliding \\\midrule
369 & pulls, rolling, pulling, roll, rolled, roll, pull, rolls, pull, pulled \\\midrule
370 & decent, free, free \\\midrule
371 & doubles, triple, double \\\midrule
372 & thrones, akon, mn, ffa, minnesota, evers, kn \\\midrule
373 & starting, start, kicking, transitioning, transfer, tackle, transferring, transfers, beginner, starter, tackling, transition \\\midrule
374 & pretzel, doughnut, donut, donuts, doughnuts \\\midrule
375 & c, cu \\\midrule
376 & testim, portfolio, refer, references, reference, ref, refs, referring, referen, hex \\\midrule
377 & she \\\midrule
378 & pro, pros, pro \\\midrule
379 & seating, seat, seat, seats \\\midrule
380 & figurine, figuring, figured, figure, figures, figur \\\midrule
381 & crou \\\midrule
382 & bru, bro, bro \\\midrule
383 & squ \\\midrule
384 & our, their, her, our, my, his, your, ur \\\midrule
385 & karaoke \\\midrule
386 & strike, striking, strike, strikes \\\midrule
387 & littlest \\\midrule
388 & rac, gas \\\midrule
389 & metrics, estimates, measured, measuring, measures, measure, valuation, metric, estim, estimate, benchmark, measurements, observations, measurement \\\midrule
390 & mustard \\\midrule
391 & keynote, attendees, delegate, sponsor, panelists, moderator, participant, delegates, presentation, judge, judges, speaker, speakers, nominees, presenter, applicants, remarks, contestants, judging, finalist, panels, committee, instructors, speaker, presentations, nominee, candidates, sponsors, panel, participants, competitors, contestant, presenters, jury \\\midrule
392 & racing, acing, races, racer \\\midrule
393 & tro, itos, sto, e, o, os, illo, io, dio, ato, jr, oo, rio, ello, ino, ace, tron, ka, icon, tto, aco, aldo, sco, dor, ado, ori, ond, bo, q, dos, cio, oes, allo, zo, aro, vee, bos, ero, ko, mos, gio, gos, zzo, inos, om, iro, za, cho, ando \\\midrule
394 & sheep, bird, doves, goats, whale, blackbird, seagull, arrows, snowflakes, crows, gulls, wolves, cow, cats, snail, squirrels, fairy, birds, penguin, deer, pigeon, birdie, foxes, insects, reindeer, fairies, frog, rabbit, owl, bunnies, hedgehog, mice, monkey, sheep, seagulls, butterfly, snowflake, butterflies, squirrel, bee, swallow, dove, toad, frogs, cattle, bees, wildlife, rooster, swallows, insect, owls, monkey, snails, rabbits, chickens, penguins, bird, cows, antelope, monkeys, camels, whales, beaver \\\midrule
395 & tipped, tips, tip, tipping, tip \\\midrule
396 & engineer, engineering, logists, researcher, scientist, scientific, scientists, surgeons, surgeon, technicians, economists, physicist, researchers, science, engineers, sciences, chemist \\\midrule
397 & method, methods \\\midrule
398 & pilots, bombing, medals, bomb, bombs, bombings, bombed, bomber \\\midrule
399 & black, dark, black, white, white, darker, whites, blacks \\\midrule
400 & covered, covers, cover, covering, coverage, cover \\\midrule
401 & below, underneath, near, under, toward, beside, entering, nearby, beyond, within, approach, survives, besides, aboard, among, contact, nearing, approaching, nears, amidst, amid, amongst, between, beneath \\\midrule
402 & poo, poo \\\midrule
403 & gus \\\midrule
404 & insi \\\midrule
405 & senate, patriotic, democratic, socialist, democrats, republican, conservative, political, governors, senators, presidential, congressman, gop, policemen, tory, government, federal, communist, catholic, congress, criminal, politics, socialism, equality, liberals, republicans, liberal, communism, politically, coalition, bipartisan, police, politician, senator, professors, policeman, govt, democrat, celebrities, tarians, patriots, politicians, dollars \\\midrule
406 & flipped, flipping, flip, freaking, flips \\\midrule
407 & cute, adorable, fluffy, cuteness, cutest \\\midrule
408 & announcement, advertise, reveal, announced, announcing, asking, suggestion, congratulations, announces, announce, unveil, unveiling \\\midrule
409 & function, functions, functioning, functional \\\midrule
410 & program, programming, programmer \\\midrule
411 & oven \\\midrule
412 & squid, squid \\\midrule
413 & / \\\midrule
414 & sounds, sound, sounding, sounded, sound \\\midrule
415 & protester, protests, protest, protestors, protesting, demonstrators, protesters \\\midrule
416 & tune, trail, label, track, trails, fault, tracking, tracks, tracker, track, trail, tracked, trax \\\midrule
417 & tney, cot, tog, crawl, acup, turbine, crawling, cotton, saur, potty \\\midrule
418 & them, the, athe, my, then, charlie, sthe \\\midrule
419 & door, door, doors, doorway, doorstep \\\midrule
420 & shia, ina, illa, ia, ola, ra, rica, ila, inas, ena, na, ska, ina, ana, tel, ura, gia, ica, lia, enas, ona, ita, cia, dia, tina, sia, alia \\\midrule
421 & with, what \\\midrule
422 & jo, jol, plo \\\midrule
423 & coriander, cilantro, cumin, parsley \\\midrule
424 & bur, tur, burg, kro \\\midrule
425 & we, med, me, a, ep, ei, ea, as, es, ed, is, be, e, eco, dge, ade, wee, ap, eh, ele, ae, age, aa, ey, cep, eur, inge, ale, Ã©, est, ame, eme, eas, esp \\\midrule
426 & ll, l, ls, hl \\\midrule
427 & addresses, address, addressing, addressed \\\midrule
428 & sign, cycles, flag, signs, flags, symbols, signage, signed, symbol, signing \\\midrule
429 & ally, aly, aly \\\midrule
430 & nest, nest \\\midrule
431 & wing, winged, wing, wings \\\midrule
432 & programme, program, programmes, programs \\\midrule
433 & ring, piercing, rings, ring, ringing \\\midrule
434 & ends, end, ending, ended \\\midrule
435 & animals, creatures, animal, animal, mammals, creature \\\midrule
436 & puree \\\midrule
437 & dugg, ali, sil, ali, alle \\\midrule
438 & vo \\\midrule
439 & trips, ride, riding, rides, rode, riders, rider, ride \\\midrule
440 & ent \\\midrule
441 & ark, ark \\\midrule
442 & ul \\\midrule
443 & through, throughs, thru \\\midrule
444 & buy, bought, purchase, purchases, buy, invest, purchasing, buys, buying, buyers, buyer, purchased \\\midrule
445 & revival, revive, revived \\\midrule
446 & tain, tains \\\midrule
447 & winter, snowy, snow, snow, snowfall, winter \\\midrule
448 & won, swing, winners, votes, win, wins, voted, defeat, winning, vote, winner, victories, victory \\\midrule
449 & hearts, star, stars, star, tar \\\midrule
450 & blu, waver, red, blue, blue, blues, blu \\\midrule
451 & hunter, hunting, hunt, hunted, hunts, hunt, hunters \\\midrule
452 & vip, pet, pet, pets \\\midrule
453 & cord, toy, bust, clock, pipes, fart, spit, mud, buff, dizzy, burr, foam, rhythm, joss, pipe, scrum, hollow, brew, tumor, clap, tuck, ink, strain, lift, twist, sewage, ress, soil, raft, dew, poop, dip, hood, flesh, cub, tug, hurdle, drift, tubes, pump, loom, tear, burns, hoax, boil, strings, rag, curl, boiler, thrash, vacuum, pigment, screws, razor, clash, loop, pour, stereo, hoop, sweat, disk, fryer, rape, tile, drum, missile, drain, pill, steam, kraft, pills, stick, bubble, spill, streak, tube, puff, glue, prey, clamp, seam, urine, mash, dread, thaw, hose, bulb, skid, bricks, odor, slash, power, stain, scrub, mould, guts, sugar, organ, fluid, spear, poker, powder, jug, tyre, jingle, gauge, relic, oil, tubing, fibers, putt, bullet, sack, turbo, fork, slap, smack, cement, ply, debris, lump, bones, noise, scratch, slug, slum, bone, pulp, spine, bolt, power, runoff, baton, bulbs, knot, frost, twin, brawl, crust, prick, rash, duct, shave, bail, bark, horn, tread, screw, beak, strut, tweed, dye, soak, morph, gas, mortar, punt, roach, vinyl, fog, boogie, burrows, feather, kidney, spar, metal, pita, dust, fuel, wool, grain, swirl, enamel, drag, serum, starch, salts, floppy, junk, grit, palm, grip, paddle, flare, burn, oil, joint, thrust, pee, knots, pollen, surge, quad, chalk, harden, jewel, smoke, stomp, poke, bubbles, blaze, clutch, stopper, strip, fiddle, boiled, rope, grease, waste, drip, freeze, string, cigar, bead, plow, poison, pinch, straw, stitch, tinker, grub, valve, tumour, pep, rib, bite, fat, rattle, laser, organs, squeeze, blood, fiber, pulse, plaster, acid, sledge, pedal, spur, flame, batter, leach, pebble, yeast, smog, foil, splash, dirt, glide, plunge, gravel, spool, fluff, tide, chord, flap, liter, wipe, poly, glaze, spout, wedge, torch, filter, diesel, piping, jam, crater, funnel, cable, cork, groove, cavity, muscle, carbon, lite, rust, glass, melt, liquor, cling, fur, hoof, balm, tire, bonnet, abyss, toss, root, brass, wart, particle, rubber, lazer, puck, upward, coal, silk, powder, gravity, pound, crumb, steam, dummy, chip, lumber, stack, scar, plume, spruce, crease, stump, palate, crank, lsd, bleach, shutter, cracker, petrol, axle, flea, pint, exhaust, fps, needle, crunch, tissue, flex, freight, rotor, soap, rumble, fluids, wiggle, shaft, gut, gears, rage, staple, knob, hips, fleece, stamp, burner, battery, fuse, roller, bladder, sweep, needles, muck, coup, coil, cash, valves, tack, roots \\\midrule
454 & others, much, lots, assorted, thousands, elsewhere, often, many, common, hundreds, countless, millions, several, various, plenty, sometimes, popular, frequently, numerous, thousand, dozens, perhaps \\\midrule
455 & ghting, light, lightening, lit, lights, light, lighted, lamps, lamp, lighter, lighting, candlelight, lightning, ligh \\\midrule
456 & asia, asians, asian \\\midrule
457 & axes, axe \\\midrule
458 & pitch, pitches, pitch, pitching, pitched \\\midrule
459 & spec, speci, special \\\midrule
460 & ant, ants \\\midrule
461 & behaviour, behavior, behave, behavioral, habits, behavi, behaviors \\\midrule
462 & spectac, spectacle \\\midrule
463 & minecraft \\\midrule
464 & secrets, secret, hidden, secre \\\midrule
465 & flooded, flooding, floods, flood \\\midrule
466 & leap, leap \\\midrule
467 & com \\\midrule
468 & spiderman, spider, spiders \\\midrule
469 & inte, int, inst \\\midrule
470 & short, shorts, short, shorter \\\midrule
471 & sai \\\midrule
472 & gopro \\\midrule
473 & gloves, hat, lid, hat, lids, hats, helmet, glove, helmets \\\midrule
474 & intro, introduced, introduce, introduction, introduc, introduces, introducing \\\midrule
475 & wered, filtered, led, omed, bled, ular, bound, gether, yed, ized, elled, ored, angled, tered, sed, thed, outed, stered, itated, gged, eded, mented, tened, zed, dged, iled, ved, ringed, onized, mmed, ented, cted, treated, ased, ined, wned, educated, ished, pered, inted, bred, aged, tured, ised, legged, lied, cated, eled, zzled, nished, fted, lish, thered, solved, tful, alized, tained, rowed, ked, oned, plated, shed, eved, fied, veled, pped, aded, sided, tioned, ddled, dered, ured, ared, dated, ned, amed, ited, bbed, eared, ened, aled, aired, ned, tified, tied, mized, vered, acted, sued, fed, ounded, inged, ified, ied, sured, gree, icked, posed, anced, coded, capped, itting, aved, ried, gated, kered, cled, enced, mated, acked, guided \\\midrule
476 & or, nor, ors, etc, non, ore \\\midrule
477 & onstage, backstage, stage, glamour, stage, stages, venue, staging, staged \\\midrule
478 & qualifiers, dominance, elevation, textures, economics, passage, sements, attitudes, hormones, mechanism, preferences, pathway, enthusiasm, intimidation, directions, resolution, breakdown, compatibility, philosophy, category, materials, generosity, composition, virtues, nomination, morality, responsibilities, emphasis, variety, quantities, horizons, origin, intervals, transparency, intentions, illusions, impressions, punctuation, downside, intent, examination, calculus, statement, factor, interests, descendants, confrontation, fixture, disclaimer, topics, calculations, material, sentences, accuracy, defenses, confirmation, diameter, effectiveness, synthesis, chemistry, aspects, turnaround, deline, texture, currents, descriptions, gradient, inauguration, personality, offspring, initiation, evolution, portion, sentiments, sequence, toppings, interest, outlook, expectations, decisions, dedication, solution, perfection, boundaries, incentives, backgrounds, personalities, possibilities, paragraph, markers, narratives, aesthetics, negligence, modification, duration, transactions, judgement, dimensions, direction, assortment, attraction, locations, electricity, substances, proportions, portrayal, involvement, pressure, decay, beginners, influences, rendition, behalf, requirements, shenanigans, permission, habitats, frontiers, quantity, illusion, principle, inputs, strengths, participation, outsiders, values, leftovers, choreography, conjunction, upwards, compositions, ordinance, conflicts, ameter, attachment, selections, processes, guidance, efficiency, sensitivity, encies, sentence, hobbies, contents, mistakes, advantages, distances, positions, terrain, prevalence, flexibility, essentials, agility, example, limitations, motivation, fragments, context, scenarios, ativity, intensity, signatures, inequality, ingredients, interpretation, cinematography, penalty, sequences, prospects, strength, dynamics, transformation, encouragement, hazards, amounts, tension, substance, designation, purposes, obstacle, notifications, compounds, generations, qualification, supervision, expressions, objectives, futures, transitions, sentiment, autonomy, dimension, mutations, awareness, brightness, scenario, redemption, findings, phases, prescription, regions, errors, relevance, mutation, hazard, genetics, commodity, instructions, candidacy, background, rences, specifications, dangers, possibility, significance, fixtures, tiveness, curriculum, atrocities, talents, alities, asure, nutrient, devastation, indication, thickness, probability, phenomena, latitude, pathways, capacity, shortage, intention, components, examples, inability, pressures, willingness, availability, failures, attributes, diplomacy, stereotypes, height, erosion, existence, abilities, characteristic, format, boundary, subjects, perception, visualization, attitude, concept, entirety, tability, capabilities, frequencies, flavours, symptoms, perspectives, finesse, resonance, placement, responsibility, basis, appearances, phenomenon, aftermath, complications, fatalities, outcomes, extension, advantage, obedience, exclusives, succession, settings, distinction, depiction, combinations, ditions, mysteries, mathematics, positioning, observation, proclamation, combination, divinity, occasion, integration, assessment, elimination, adversity, projections, artifacts, restrictions, viewpoint, categories, status, prejudice, ethnicity, circumstances, flavour, supremacy, currency, chords, perceptions, vegetation, aspect, sideline, discoveries, implications, arrangement, synopsis, observers, storyline, continents, discography, judgment, atmosphere, correction, adjustment, consequences, diagnosis, imitation, themes, advancement, recognition, extensions, punishment, agreements, natures, pattern, submission, appreciation, periods, opposition, territory, conception, consistency, options, fairness, criteria, outskirts, agreement, tranquility, position, convenience, incentive, sportsmanship, manipulation, theories, exhaustion, utilities, meanings, insight, integrity, transmission, grammar, mischief, inspirations, determination, instinct, submissions, definition, ventilation, stures, execution, dialogues, specification, areas, difficulty, convocation, complexion, precautions, offerings, recipes, entries, enquiries, whereabouts, sexuality, identification, downfall, stance, contrast, reasoning, mentation, orientation, assignments, misconceptions, output, versatility, equation, domination, enjoyment, occasions, component, equations, templates, ppings, essence, attractions, entation, destruction, expression, elements, disappearance, volatility, qualities, impression, proportion, milestones, adjustments, distance, configuration, ingredient, iority, disruption, incidents, factors, relation, suspension, remnants, frequency, versions, barriers, segment, patterns, characteristics, contribution, indicator, backdrop, invitation, adulthood, popularity, currencies, premise, identity, quotation, obstacles, degrees, stability, revision, pancy, depth, syndrome, variation, assignment, ference, amenities, intervention, conflict, element, statements, varieties, concepts, preference, percentage, anticipation, qualifications, invitations, opportunity, genres, visibility, projection, certification, solitude, progression, formity, functionality, posture, origins, fundamentals, formats, segments, benefits, paperwork, pointers, input, minimum, complexity, density, markings, principles, contributions, undertaking, alternatives, expectation, stances, traits, achievers, exploration, capability, reforms, signature, segregation, intolerance \\\midrule
479 & roman, roman, romans \\\midrule
480 & left, correct, wrong, right, straight \\\midrule
481 & bytes, surfing, whil, alot, kitch, kuma, being \\\midrule
482 & danc, dancer, dance, danced, dancers, dancing, dances, dancing \\\midrule
483 & liquid, liqui, liquid \\\midrule
484 & slic, slice, sliced, slices \\\midrule
485 & tell, tells, spoken, asked, stated, asks, saying, says, telling, said, ask, told, say \\\midrule
486 & website, blog, web, webs, web, websites, webpage, brochure, sites, site, homepage \\\midrule
487 & jer, fle, fri \\\midrule
488 & moving, touched, disturbing, touching, touches, touch, touch \\\midrule
489 & oatmeal, mozzarella, guacamole, paella, chipotle, pesto \\\midrule
490 & recommendations, summary, giveaway, review, reviewing, reviewers, highlight, critic, recommended, reviewer, reviews, recommend, recap, critics, critique, recommendation, recommending, overview, recommends, reviewed \\\midrule
491 & promotes, collects, celebrates, encourages, celebrated, celebratory, celebrating, congratulate, commemorate, removes, embraces, celebrate, congratulates, celebr, celebrations, embracing, congratulated, celebration, congratulating \\\midrule
492 & od \\\midrule
493 & dri \\\midrule
494 & pops, popped, pop, popping, pop, popu \\\midrule
495 & neighboring \\\midrule
496 & rescuing, rescues, rescue, rescued, rescu \\\midrule
497 & domin \\\midrule
498 & arse, asses, reef \\\midrule
499 & attack, attacks, attacking, attackers, attacked, massacre, threats, assault, targeted, threat, explosion \\\midrule
500 & earnest, formal, uncommon, mutual, polite, vious, speedy, thinner, rapid, getic, bulk, ssive, deep, filler, careful, every, damp, coy, prime, smarter, varying, seasoned, icted, less, brave, bare, narrow, ample, strong, easy, hefty, dient, cheap, sory, sense, tricky, uphill, certain, capable, sane, richer, dull, softer, humble, more, motley, strait, strongest, busy, vile, mature, innocent, tall, only, shy, weak, faint, false, distant, sincere, sly, tougher, forth, blank, minor, loud, broader, catchy, vary, crowded, supreme, wise, lack, simple, swift, deeper, dest, needy, vicious, diverse, louder, fond, ful, fellow, standout, steady, tiest, keen, enic, same, foul, bad, steep, tame, spare, tender, equal, noisy, modest, annual, silent, cruel, salty, scarce, moral, actual, stiff, rusty, single, immune, taller, safer, abour, proper, ripe, esque, bold, sour, sheer, generous, broad, smart, eventful, safe, biased, foggy, pure, guilty, loyal, gentle, ordinary, wild, costly, healthy, standard, barren, baddest, peculiar, stable, pale, caring, anew, loose, idle, sole, manner, almighty, iest, hazy, thin, poor, true, noble, childish, foolish, orderly, tragic, stubborn, basics, regular, slight, earliest, wavy, familiar, bland, sudden, petty, strict, mental, midst, hearted, slim, brighter, ible, tailor, brief, endless, usual, eldest, eager, cooler, faithful, finer, tuff, thick, soft, warms, greasy, serious, cial, typical, quality, longer, rookie, ight, spirited, vivid, quiet, void, aky, rotten, rampant, constant, soggy, diest, amateur, simple, stout, heavier, chaotic, maximum, soft, basic, oldest, vain, easy, fiable, messy, raw, inner, cise, ideal, thicker, extra, itable, hectic, sick, windy, exact, uneven, sharp, vague, naive, divide, reliable, lazy, dense, decisive, lone, rious, ruff, harsh, dirty, crude, utter, softly, msy, varied, solid, aneous, pless, main, fluent, unseen, useless, toxic, severe, mild, tense, prone, rural, rare, lengthy, dious, yearly, vast, finely, heavy, stray, weaker, tidy, other, active, longest, shallow, greater, worse, easiest, evenly, handful, average, local, poss, heavy, tious, sore, wider, worst \\\midrule
501 & lame, random, idiot, stupid, wacky, boring, craziest, nerds, crazy, surreal, smelly, freaks, weird, freak, stinky, ugly, pointless, gross, crazy, weir, nasty, dumb, nerdy, bizarre, eerie, abnormal, annoying, dork, odd, strange, normal, trippy, nonsense, weirdo, normal, crappy, geek, silly, freak, nerd, idiots, awkward \\\midrule
502 & sing, sing \\\midrule
503 & crack, cracks, crack, cracking, cracked \\\midrule
504 & cola, coco, cess, co, co, cos, cou, prop, tec, loc, slo, eco, colo, coco, col, mol, coo, county, pom \\\midrule
505 & aur \\\midrule
506 & knocked, knock, knocks, knock, locked, knocking \\\midrule
507 & sters, mouse, ster, ater, simpson, gger, lett, ster, stery, stor \\\midrule
508 & sar, sas, par \\\midrule
509 & brown, brown, browns \\\midrule
510 & check, check, checked, checks, chec, checking, checker \\\midrule
511 & bear, elephant, bears, seals, elephants, seal, bear \\\midrule
512 & brain, impy, hitler, idc, oop, cky, hip, icky, ipod, bud, wag, nist, kpop, mets, mug, wich, cum, rude, bug, bum, oup, gay, bbc, wwf, whoop, pple, adn, fbi, dino, iphone, ios, moo, ugh, haram, diss, elot, irl, emo, fuk, whore, goofy, eachother, scom, wight, redneck, beech, augh, yum, thumbs, init, bub, nude, mugs, whit, butts, queer, butt, kkk, fatty, noir, meow, ggin, bic, itch, guay, tumblr, doh, manly, espn, nephews, ipad, ffee, oops, iphones, lego, oppa, pinup, nuts, losers, dod, bugs, wii, peds, amen, hoe, wah, shaq, ass, wassup, giddy, bby, yup, nut, phone, slang, pose, leggo, boo, gills, nasa, chio, phone, oof, mpy, frat, rnb, nintendo, hunk, pooh, awwww, sex, amuse, tey, ect, diddy, sous, mish, dada, phones, ebay, tit, fetus, etsy, pez, emoji, rome, ople, aise, aby, onies, lesbian, jk, pow \\\midrule
513 & cheer, cheered, cheerleading, cheer, cheerleaders, cheerleader, cheers, cheering \\\midrule
514 & passing, pass, passed, passes \\\midrule
515 & cool, favourite, wicked, friendly, pretty, good, best, fine, nice, icious, yummy, enjoyable, delicious, sweet, tasty, favorite, nicely, perfect, gorgeous, beautiful, dope, finest, lovely, charming, pleasant, precious, splendid, attractive, neat, handsome, tiful, good, nicest \\\midrule
516 & pushing, pushes, push, pushed \\\midrule
517 & lowing, hailing, dashing, braving, asting, daring, spitting, rising, scrolling, diving, plying, firing, skipping, melting, avoiding, dripping, soaring, settling, bearing, speeding, stepping, storing, haunting, wrecking, fixing, tying, weeping, chilling, piling, dumping, mocking, warming, jamming, undering, scratching, hovering, exploding, bowing, icking, shifting, raving, watering, lurking, pering, leaning, towering, wasting, sping, assaulting, ating, tumbling, weighing, bleeding, aping, resisting, roaming, circling, airing, sticking, aring, begging, ddling, directing, creeping, brushing, ounding, sweeping, freezing, splitting, acking, hauling, threatening, inting, soaking, oming, whispering, absorbing, biting, spilling, bouncing, turing, snoring, sensing, banging, rounding, tuning, drafting, handling, boiling, shaving, invading, mering, beating, rying, balancing, stirring, mating, fielding, stacking, mounting, ancing, whipping, landing, curling, curing, sunbathing, playing, cooling, oring, burning, solving, breathing, wandering, owing, floating, accelerating, dividing, lowering, locking, spraying, powering, paddling, bursting, dipping, grazing, drifting, swapping, stealing, winding, howling, calming, patrolling, boosting, leading, tapping, raging, abusing, lounging, lifting, molding, yelling, transporting, dusting, drooling, roaring, collecting, smashing, forcing, shrinking, veling, flaming, clicking, cting, rowing, swinging, rafting, shredding, disappearing, ripping, booming, brewing, stering, arranging, grabbing, revisiting, pacing, milling, mbling, posing, uniting, treating, porting, illuminating, drumming, gripping, marrying, iving, linking, descending, petting, hawking, pounding, inspecting, playin, shining, gating, owning, buzzing, fleeing, docking, refreshing, shouting, removing, barking, exercising, robbing, gazing, sinking, suring, escaping, browsing, comforting, guiding, weaving, shutting, turning, flushing, tearing, driving, pouring, rooting, choking, schooling, blazing, striving, pumping, slaying, tracing, grinding, bashing, ranging, ticking, aking, raping, looming, tending, capping, licking, spreading, peeling, downhill, venting, stalking, stripping, damaging, guarding, crushing, chewing, spanning, staking, drowning, navigating, waving, irling, taining, easing, dominating, copying, filtering, flexing, busting, enting, dragging, lingering, hooking, flashing, unlocking, shading, slowing, stomping, cruising, peeking, shedding, mping, fling, brightening, fooling, exiting, thering, separating, behaving \\\midrule
518 & catwalk, runway \\\midrule
519 & another, a, some, one, which, some, how, an, own, no, such, dis, its, there, the, anybody, what, other, thee, whoever, enough, why, real, only, so, where, here, theirs, if, them, few, this, ones, very, whatever, theres, that, same, these, either, else, whose, more, anyone, that, most, those, wth, nothing, nobody, even, anything, who, dear, rather, any, thus, whom, whats, yours \\\midrule
520 & din \\\midrule
521 & ni, ne \\\midrule
522 & and, n, +, but, &, and, plus \\\midrule
523 & ie, ies, ette, cini, inet \\\midrule
524 & scooby \\\midrule
525 & cg, gini \\\midrule
526 & fumble \\\midrule
527 & showcases, showcasing, showcase, showcased, spotlight \\\midrule
528 & cars, vehicles, vehicle, car \\\midrule
529 & expose, reception, compilation, exhibit, retrospective, display, vendors, reproduction, exhibits, exhibiting, arra, exhibition, vendor \\\midrule
530 & lab, pos, smil, find, rhi, rot, ear, wal, thu, pott, off, minic, cup, fon, hop, polit, sli, lun, manu, guar, toa, put, ordin, sali, andro, quar, ur, cru, dat, ilan, fli, rum, bu, audi, tel, simp, dol, for, use, base, log, crum, rich, cop, ott, plac, how, py, fil, pen, syn, las, sharp, stil, thumb, bick, sati, sig, sol, fom, gau, blin, port, atul, won, cir, ridd, att, snoo, bean, enig, tto, phon, toge, til, cent, net, gran, syl, snor, snu, lip, claudi, sau, moul, lon, crow, cur, dom, spic, rio, minis, wed, stan, bic, kabo, chir, mand, kenne, court, maul, buck, scar, row, cat, anto, tiss, bil, jav, pra, sitt, qu, scul, acu, lao, marin, whel, pher, ten, lac, obl, vag, fet, yel, meg, lough, bub, clou, gira, blo, stu, hin, dle, chic, pel, tru, den, fair, colli, ful, tou, mill, arti, hic, clam, hul, rand, sno, stal, colo, hor, cooper, ble, poin, bug, fal, spl, jou, ping, smel, tag, son, ich, satur, cr, collar, gim, chap, broo, bee, wri, cli, hal, di, pear, chom, gent, brun, villi, gli, spen, bod, stru, too, semin, torn, swe, dum, camer, horn, mbo, main, lis, dn, igu, just, bey, tot, scallo, craw, victori, enti, carri, tid, slan, hab, past, taun, paste, clin, bw, tul, teas, grou, bl, cali, krat, pag, caul, thaw, aur, vit, kil, kell, desp, plum, tab, stol, coll, baz, dau, jel, itt, bren, fav, chil, fern, twin, musc, ech, fit, wq, phili, bm, lob, dil, amp, capit, fat, ign, meli, ming, strat, gly, spla, gag, coel, wali, infl, carol, app, mitt, pine, lay, ht, drum, dim, ando, sad, vig, spoo, scru, vir, said, jame, sni, hydro, epi, sten, trun, dele, sill, hey, bt, fy, slo, litt, ise, stap, pli, smoo, brow, balo, rais, flo, guil, ern, wil, thel, tali, pot, like, alt, dd, iz, shel, strick, ror, smash, wind, cutt, dow, mono, thin, bot, langu, club, beu, pend, poly, sie, iv, dem, hur, list, git, scri, chen, uru, twer, dul, staf, graci, dir, place, lor, allo, beh, van, salu, atl, lit, sever, bud, guer, zig, stin, liv, mart, dit, aff, still, stag, vel, hn, sale, thir, phal, shat, wol, fol, fine, emp, cle, limb, lau, sna, thur, ail, quan, wai, hil, sut, rhine, jen, add, ote, brac, ick, who, stom, shine, fou, nil, mati, alla, kut, cic, yin, trin, stein, det, ghi, cait, trol, fel, cano, britt, patri, corner, pau, lid, butter, stoo, chol, hay, scho, ding, clo, nord, mud, ship, miri, chau, fif, sit, shim, twee, pper, gren, wom, along, bus, dac, scan, lind, vill, him, wait, gul, mus, camp, shr, ske, jung, azu, montag, scu, gir, tann, gou, tro, string, fic, suit, soli, math, schu, clut, diet, god, haw, equ, blan, colle, span, tour, wine, kno, avi, vil, cour, swa, magin, vine, mali, group, des, christ, plu, del, ambro, scat, ril, colla, rubi, vand, shor, mist, quin, his, cani, bach, cow, gno, sall, tram, corn, tape, form, spu, ratt, raz, asy, shutt, slu, nur, beau, buff, kni, brah, gui, christi, cau, sru, thy, spor, sci, hass, thro, ght, asper, kop, miro, brat, trac, gori, mach, mind, flor, stri, ging, wy, mich, lori, lot, tier, grin, fix, agi, cran, allu, roc, zoo, laun, scal, lom, cari, jig, gaz, scur, cell, jor, seas, bour, stor, lik, somer, chill, glou, stam, bir, asho, lamin, iri, omon, brock, gro, ben, ld, lea, glad, lax, gali, ador, shing, tren, wyn, pir, kit, tand, kel, scoo, sav, schi, goo, smu, chapp, caf, cot, cad, suz, bern, uss, cole, skar, clar, flan, unit, olo, kip, spru, mack, swif, duc, oz, quit, cav, vani, grat, ux, ffi, hall, peri, fai, elu, vu, clu, chal, yi, beg, ves, shee, trum, bast, jour, shap, stati, kir, pall, stig, hd, bott, pg, oti, cul, dai, fili, yt, fest, tis, ques, nik, penn, tiv, sigh, lock, wen, seme, chas, rhin, labe, mour, sid, vent, sop, shol, apat, cob, fitt, fill, tall, dio, willi, gee, noo, pit, rox, turn, mush, billi, mish, deep, tend, sche, ish, nati, pou, tani, agar, ichi, well, adi, scor, sug, spot, ind, stir, tomo, sen, vast, pav, hud, xen, mot, sprink, tore, suf, aju, was, brit, aun, wir, sud, mut, scro, litter, frei, dumb, esk, wau, sag, filip, leon, stran, wad, rust, bis, raf, gur, hann, swar, phe, twit, dand, luci, wid, kin, tj, wra \\\midrule
531 & holl \\\midrule
532 & performance, perform, conducts, performs, performances, delivers, performers, performed, presenting, applying, performing, providing, practising, delivering, perform, rehearsing, performer, representing, conducting, committing, deliver \\\midrule
533 & gle \\\midrule
534 & h, hr, ht, hhh \\\midrule
535 & jungle \\\midrule
536 & gr, gor, gri, gram \\\midrule
537 & brothers, sisters, sibling, cousin, bros, siblings, brother, brother, sister \\\midrule
538 & oud, crabs \\\midrule
539 & com, comm, comi \\\midrule
540 & tanning \\\midrule
541 & mellow, glowing, funky, dank, comfy, delicate, gloss, smooth, chubby, styli, tearful, bubbly, curly, bohemian, phat, soothing, cuddly, shiny, upscale, luxury, spacey, bouncy, picturesque, clever, lively, dreamy, enchanting, fancy, indie, tranquil, custom, exotic, earthy, decorative, spooky, trendy, smoky, jolly, cozy, curvy, spiced, artistic, textured, unusual, sparkling, erotic, cency, regal, famous, crisp, ornate, colourful, smokey, skinny, flavored, faux, desirable, tuous, slender, vibrant, scrumptious, sizzling, puffy, sexiest, mysterious, rustic, foxy, shady, gourmet, astic, novelty, sparkle, ghostly, edgy, mingle, eclectic, matching, leafy, diy, classy, rowdy, crafty, flavorful, ominous, glows, cosmetic, silky, romantic, exquisite, squishy, iconic, jazz, strous, dapper, sassy, juicy, sexy, styling, sleek, oldschool, collectible, fierce, cheerful, fashionable, playful, glitter, steamy, stylish, creamy, sparkly, moody, gory, posh, fuzzy, futuristic, twinkle, dusty, peaceful, naughty, casual, quaint, joyous, joyful, starry, hairy, sleepy, serene, nostalgic, feline, scent, lush, blush, whimsical, wealthy, smooth, hipster, glamorous, topless, glam, artsy, crunchy, smiley, chunky, scenic, suede, lacy, chic, luxurious, fiery, delicacy, quirky, sketchy, gritty, rockstar, kawaii, colorful, silicone, flattering, airy, sizzle, flavoured, cosmic, plush, lavish, snazzy, matte, jazzy, moist, sophisticated, beauties, divine, mystical, chewy, sensual, elegant, curious, idyllic, luscious, expensive, sloppy, sturdy, festive, acial, pleasing, lovable, groovy, metallic, soulful, breezy, frosty, itchy, photogenic, sporty, spacious, upbeat \\\midrule
542 & each, all, select, both, all, rest, alls, everybody, everyone, everything, total, everywhere, every \\\midrule
543 & ph, thr \\\midrule
544 & ci \\\midrule
545 & memor, accomplishments, successful, succeed, realization, achievements, reagan, success, accomplishment, accompli, accolades, accomplish, realizing, successfully \\\midrule
546 & float, flies, flew, flown, flying, fly, fly, flight, flights \\\midrule
547 & graffiti, mural \\\midrule
548 & attempting, attempt, attempted, tries, attempts, tried, trying, try \\\midrule
549 & buggy \\\midrule
550 & tables, counter, menu, counters, tabletop, table, buffet, menus, register, cabinet, table \\\midrule
551 & tr, st, spar, sk, sty, str, saint, whit, sty, fir, sp, must, lc, st, sta, wish, sr, street, smi, street, first, spri, stun, tl \\\midrule
552 & mlb, nba, wwe, nfl, nhl \\\midrule
553 & volkswag, vw, chevy, lambo, opel, honda, dodge, ferrari, bugatti, bmw, mazda, infiniti, pokemon, mercedes, maserati, nissan, gmc, hyundai, lamborgh, volkswagen, toyota, audi, benz, chevrolet, acura, porsche, suzuki, sega, lamborghini, fiat, volvo, adidas, scion \\\midrule
554 & distr, distracted, distract \\\midrule
555 & fla, fr, fl \\\midrule
556 & shaking, shake, shakes, shook, shaken, shake \\\midrule
557 & frying, fry, fries \\\midrule
558 & shocks, surprise, surprises, shocking, shocked, surprising, unexpected, stunned, scared, upset, surprised, shock, delighted, amazed \\\midrule
559 & dead, dying, dead \\\midrule
560 & though, however, although, tho, doe \\\midrule
561 & rotating, revolving, rotation \\\midrule
562 & transformer, transformers \\\midrule
563 & handmade, making, makers, made, written, made, make, homemade, make, maker, makes, makin, write, wrote \\\midrule
564 & leaf, many, know, veer, holy, atro, medic, uke, calam, fanc, prick, cope, hk, popsic, prod, tux, ext, spel, chead, miz, squat, zoom, rag, melo, adren, moroc, pedi, terri, fox, gym, sway, swat, tender, begg, egy, pizz, mosch, veterin, jewel, pow, egyp, fang, goldeng, ruff, grun, rik, pean, hydra, pedic, baske, pope, heck, oj, albat, taran, chine, spn, bench, giam, thermost, spee, ited, comman, worm, eyel, uten, griff, swag, lulla, plun, michi, blon, goss, vul, coles, veg, ebon, psy, soil, gymna, corp, candle, rear, wav, mocking, glit, mountaine, collo, ggy, spider, pocket, drun, data, slam, patron, oly, www, demol, itch, degra, cry, poun, exor, tern, childre, sciss, scare, mmm, kick, splin, ura, thai, megap, titi, kash, kitt, carto, pk, ancho, matsu, pupp, carpen, peril, pose, petal, whist, writ, econ, ete, meet, pedal, swee, stad, perfu, myster, pode, canv, oman, keen, fidd, neur, masc, tight, natu, sugar, marvel, bulldo, bino, boun, dump, loop, tank, meth, flex, sexi, bond, tant, nois, plic, narr, obe, cori, velve, swer, chag, sque, droo, fashion, dang, motor, shru, tyran, loud, roun, sling, ghost, steff, stick, podi, crun, jaw, knuck, sany, aci, drow, irl, trape, flyn, button, papar, cathedr, cyto, dres, meand, click, ghou, carab, advent, twi, defl, floo, wren, chee, neg, newsc, uber, hamp, scram, nether, moto, plex, hitch, allot, vod, krun, arsen, roller, cave, kry, ultram, cough, jalap, bandic, lette, cbc, squir, dulu, gang, pleas, hash, graf, appa, offro, politi, octa, fell, sanje, ssy, slee, stopp, santac, augh, desol, scrap, sole, shack, vaul, polic, ross, shut, treas, dino, chie, cod, metal, feather, ying, squee, butt, spray, unt, neuro, glaci, audit, abr, bust, trous, letter, yaw, breath, leis, tote, tigh, dread, sini, dism, escal, vom, ghet, acl, scand, stumb, sautÃ©, handicapp, volley, gib, hollow, hear, sizz, hake, amid, paras, hammer, wiz, gett, ruck, wins, freed, masse, trap, bore, spaw, whir, pepper, bann, thick, cree, zyn, saul, shrin, carls, myri, hock, anten, ung, turt, nose, dinosa, level, cater, aller, newsp, kram, shre, whirl, peek, spit, type, jume, ragha, dolph, cathe, grocer, dip, spas, cambo, bathro, machin, fior, collap, pie, vacu, horri, dodge, nutr, why, flur, eat, phy, smir, vex, muham, paedi, cymb, sedi, neck, illu, eleph, drey, dimp, push, candel, soun, rhy, noi, oxi, sandwich, plant, cooking, zucker, legal, eart, batter, brai, fed, laven, deo, cellu, slap, snar, yum, footb, baller, summon, snee, icic, price, pepp, cool, macin, stric, aph, urin, rap, vogue, tomat, aquari, powe, judi, suicide, globe, shil, logo, toxic, kus, arbor, moisturi, loss, meadow, neve, gay, breakfa, event, wreck, paci, prab, jap, mode, harb, robb, epic, tribe, giz, breast, alcat, hypo, drain, tink, cub, meer, round, aero, deodor, biscu, crew, page, hallo, ack, thermo, barber, atta, calyp, saras, toma, hig, patti, vh, holi, bally, shift, zip, mccor, lulu, auti, pixel, athle, babys, schan, craft, jugg, newly, wro, temper, croo, grid, moi, upl, kine, oxy, hub, toy, cobble, bedro, arm, kung, spoon, molo, hust, stance, doom, bier, smur, fig, ripp, koso, solst, scow, pup, step, fierc, doll, parach, conj, piano, mcfar, foun, snoop, jail, peac, theat, stab, tick, camel, pump, grow, barric, ballon, esa, kool, delic, ambul, mutil, hispan, brook, pes, carra, aor, cumber, bloo, brick, dude, gap, flatt, sly, tug, merce, veriz, snat, iss, volk, cray, anem, tanz, spher, cheap, chast, omer, spiel, msn, gossi, mosqu, whal, sput, trash, futuri, madd, porsch, pyro, helicop, manne, hippo, anger, portu, simm, steep, astr, mpu, schem, forsy, hail, peep, clow, prison, tennis, howto, davin, samo, weight, galac, spread, dwar, stain, caffe, icu, liqu, copper, napp, orang, punc, jets, anchor, waz, skim, carbon, lunch, anch, topp, cil, dirt, tube, pod, empty, pum, random, waist, fake, ecker, gallo, clay, swal, swan, mobi, sweat, crock, harsh, atar, grav, catap, sso, grapp, stewar, kaleido, cheek, eras, lobb, coast, chalk, poli, tinker, seaf, heav, rott, cki, pale, kangar, fright, yol, stadi, lepre, homer, cruis, salmon, bungal, djo, cany, anal, stark, inn, rip, gob, onic, glas, aban, xia, temp, chand, pony, decor, ille, lumber, craz, pede, quarter, blit, maje, mood, fing, merr, wet, acro, tax, splat, umi, jec, baff, ribe, hoar, thes, draw, moore, pierc, meso, seed, feroci, spir, kev, bubb, potam, beast, rp, volcan, cudd, zom, thra, ragh, rhino, chori, archa, trampol, juic, soap, risk, spark, dram, behin, match, pendu, upper, hoi, trust, cuis, fantasy, fric, armad, heli, lever, kyu, sson, parme, casc, evapor, hurric, octo, marsh, firen, pix, hipp, vant, cincin, pour, calm, jiha, drau, chiev, seal, pong, eclip, swing, testic, mumb, gest, cats, paddle, quizz, anxi, ayurve, russi, conn, sker, clas, dash, player, ply, dome, magn, quick, Ð², rubber, semic, foss, monarch, pimp, robot, bachel, mosquit, chatt, pew, skel, takeme, hypno, dust, master, betra, eci, curi, bass, jaf, pann, alban, blanc, manic, hatch, ceram, mercen, neat, glee, bloss, khali, capu, gear, kidnapp, tter, kore, buzz, taxi, posit, saber, loy, arch, bail, alumin, ether, rune, bark, sauer, berser, tool, crab, glass, sink, cycl, nutri, priest, skull, sudden, ido, comic, leave, parag, flav, labou, neph, guj, dizz, cinnam, mao, ket, mccar, wrink, broc, awk, aerop, fry, casu, vix, alth, toll, boomer, astro, poe, colon, macro, pert, agon, aster, pne, lamb, groun, flame, shipp, knick, aerob, female, awak, mouse, hap, finn, vap, dais, silen, sax, quay, hc, barrac, belt, puzz, stret, pair, narco, lick, mob, shuff, zapp, morph, cryp, cigar, inciner, lux, skid, emper, donat, scotti, nec, gain, shy, eso, fris, prun, mache, dish, cart, cannon, vest, auc, veter, scorpi, goal, mcgra, aux, titan, sting, leep, glar, percu, flint, drug, viro, drag, plough, aard, aure, brack, peach, wob, anom, skil, atle, catt, albu, count, dyn, leak, alpha, angry, feat, thum, daun, marion, peel, pist, guit, cov, fairi, tow, talent \\\midrule
565 & hover, hover \\\midrule
566 & model, models, modelling, modeling, model, modeled \\\midrule
567 & snt, nt \\\midrule
568 & keeping, staying, stop, keep, kept, brake, stay, handle, stays, handles, stay, stop, remain, keeps, stopped, stops, stayed, stopping \\\midrule
569 & sold, trade, offers, trading, auction, sells, fitting, sale, sell, offering, sellers, offer, sales, selling, issuing, offered, dealing, donating, eving, seller, traded \\\midrule
570 & snowboarding, snowboard, skateboard, skateboarding \\\midrule
571 & ked, king, queen, kin, kings, king \\\midrule
572 & liverpool, cine, cinema, credits, cinematic, cinemas \\\midrule
573 & clippers, playstation, ops, ps, xbox, ping, naps, pes, mps, ps \\\midrule
574 & statues, statu, sculptures, statue, monuments \\\midrule
575 & record, recorded, records, recording, recordings \\\midrule
576 & wrest, wrestle \\\midrule
577 & unfortunate, disappointment, painful, ashamed, disgusting, disappointed, unfortunately, disgusted, intrigued, disrespectful, saddened, heartbroken \\\midrule
578 & show, show, displays, showing, shows, demonstrating, sporting, shown, displayed, showed, displaying \\\midrule
579 & screaming, cry, crying, cries, screamed, scream, screams \\\midrule
580 & t, t, f, tt, kel \\\midrule
581 & tic, tica, tic, tics \\\midrule
582 & spon \\\midrule
583 & phon \\\midrule
584 & simul, simulation, simulated \\\midrule
585 & buddies, mate, ranger, friend, buddy, mates, friends, teammate, pals, buds, pal, teammates \\\midrule
586 & sparrow \\\midrule
587 & pirate, viking, pirates \\\midrule
588 & chur \\\midrule
589 & require, seeks, needing, need, demands, appropriate, needs, requiring, required, requirement, necessity, requires, missing, needed, necessary \\\midrule
590 & upside \\\midrule
591 & tent \\\midrule
592 & fan, fa, rsa, fan, fans, fake, replica, fairs, trades, coke, pga, era, fair, fifa \\\midrule
593 & ves, ve, ple \\\midrule
594 & english, vietnamese, french, dutch, spanish, english, italian, japanese, russian, swiss, chinese, russians, german, swedish \\\midrule
595 & charac, inti, intre, factor, humor, communic, proce, deliver, synchron, visu, comfor, straigh, numer, feature, surroun, hyster, surve, sens, expe, inser, relent, avail, convers, descrip, rejuven, eventu, fashi, omni, promp, testi, demonstr, argu, acceler, region, ortho, destruc, attach, cultiv, addic, incre, gover, govin, figu, advoc, develop, manipu, conduc, move, grote, recipi, descri, vali, interro, beha, forgi, anec, reminis, presu, transi, advance, meaning, destin, local, correspon, together, inquis, enthusi, facilit, displa, resur, replac, depar, educ, admir, disru, ilit, erup, dilig, unidenti, obstruc, dial, lumin, inten, litur, transcend, engine, acqu, exhib, incorpor, moder, exerc, opha, comer, discre, sensu, resemb, progre, explan, semb, denti, compens, rejo, dep, disapp, psycho, trouble, circuit, acci, vladi, amate, contro, partic, predat, exam, penetr, repri, discipl, clever, virtu, crystalli, gimm, impre, demo, aless, conve, accom, moment, affe, emul, renais, excav, instin, confe, execu, present, brief, paro, conco, repor, correc, outw, vehic, fanta, condol, verti, incu, renov, hast, impe, migr, defe, ante, cont, suspec, comp, overwhel, inc, uto, prop, transm, enqui, deton, retri, credit, ejec, revolu, mobili, reinfor, hallucin, aud, corpor, explain, deliber, questi, metaph, mistre, exper, cruel, common, inver, negoti, ticul, selec, expect, adap, struc, amphi, duplic, distor, pamph, contamin, harmon, disco, social, deci, adju, sportsc, stereo, ambi, complex, leng, aphra, collec, elabor, inner, revol, coun, manipul, presi, handle, course, establi, gradu, anno, applau, activ, moving, nutrition, frigh, acou, glimp, servic, delight, reflec, commer, pass, recipe, intermitt, indic, provoc, diagno, threat, revers, rehear, protag, altern, sexu, contempl, miser, construc, uncondition, excit, contin, control, expl, discu, appeti, intere, convin, custom, excur, conce, disc, configu, replic, profe, furi, desig, exagger, recl, presiden, happen, domestic, motive, suggesti, objec, euchar, formu, persu, experi, intro, represent, appo, imper, ascen, haras, disper, navig, effe, spoke, assas, particul, condu, modu, critic, aint, interven, fraud, coer, eloqu, process, unite, congre, creati, chron, dissol, eque, respir, submer, perpetu, expla, scrip, intoler, disappro, elector, jeal, attend, conveni, juxta, ingredi, compe, nouri, reflex, infan, envel, compet, youtu, cosme, bombar, suspen, attrac, imperson, camoufla, compul, inci, comb, sacrific, choreo, enqu, acce, accompan, promis, appar, debun, protect, equi, mediac, distingui, prostitu, dispar, automobi, opor, precipit, auditi, illumin, indiffe, theore, question, materi, congr, dignit, bure, unfor, solic, interpre, criti, exce, disgu, benef, terrori, forwar, physio, seem, border, extingui, arbitr, compu, weap, entertain, arrang, empha, concentr, crit, trage, exhau, inqu, infiltr, fellow, anthro, classi, energi, srilan, defend, prag, perce, direc, evalu, panor, dedic, embelli, worshi, assaul, midd, partici, compri, nucle, practi, infor, enthr, err, occa, interrup, beati, footh, anatom, accur, chronic, document, circum, embr, cushi, exten, curren, popul, respec, apologi, appe, manag, flexi, clari, eleg, oper, reboun, stimul, mathemat, ethnic, modi, electri, sym, interpret, lincol, deduc, exhi, fluctu, eleng, accor, disinfe, accent, role, margin, suppo, organ, handic, consul, enjo, positi, inju, phra, attribu, specul, maneu, emin, through, enlar, financi, customiz, refr, depos, commerci, intersec, extre, encoun, diffu, uter, contra, justi, certi, begin, ornam, toile, dispo, func, obli, categori, occu, solidi, orchestr, initi, contr, obstru, susp, depic, expi, atten, artist, dissec, hour, intru, prac, occup, mirac, abbrevi, secu, frankfur, invo, answ, consi, monit, organi, signi, regular, ambu, compla, champion, publ, sobri, parame, possi, upro, suppre, enh, confron, obsole, motion, astron, culmin, conclu, receip, landsc, prat, adventur, prece, exfoli, intercep, additi, prefer, dispat, supremac, vibr, deplo, applic, trilo, extravag, oppre, compart, incredi, capac, conte, decan, copy, quali, cospla, equip, informat, calcul, divi, access, festi, technic, impro, catalo, convic, flaun, hygi, aflo, limous, competiti, codi, occur, adver, acc, trav, near, dispen, pregn, soci, parano, appli, engra, meteor, appell, digni, summari, logi, paragra, instru, physi, outer, restra, transp, absor, hesit, omic, conven, compli, caric, melan, confi, vici, responsi, belong, prepar, absolu, combin, paraly, inspec, timel, injec, pronoun, diffe, pilo, memb, journ, avoi, stabili, innov, summ, proto, complic, inhal, briti, portra, annivers, hypothe, dece, candi, contain, subscri, medit, dif, practic, author, mult, desper, theori, orig, ritu, funer, improvis, mimic, eviden, sophistic, extraordin, vincen, environment, divin, prob, situ, decre, succe, conden, vocal, contest, trajec, note, reson, polym, preserv, adventure, fashioni, evacu, tremend, confu, proc, aband, transport, bangla, candid, dire, scienti, appro, congress, trium, distur, mainst, affirm, comprehen, consu, propag, conspir, confor, defen, opla, dismant, guid, into, shoul, desc, search, consol, alig, controversi, substan, invent, thresh, caver, opini, distri, compar, disa, announ, critici, luxu, competit, motiv, analo, predic, emplo, foreclo, constru, intern, manife, asser, repet, descend, syste, campa, consecu, genoci, bizar, natur, digit, astoni, alum, presen, immer, symboli, metast, ico, aesthe, integr, discrimin, marke, paralle, demean, simil, descen, coordin, apolo, vigor, imag, absol, trou, punctu, percent, oci, busine, incl, suspici, effec, disin, aeron, victi, obsc, profici, persecu, artif, courty, conse, pover, ridic, charis, apocaly, produc, recep, dramati, sabot, pollu, touri, sponsor, prohib, chauffe, encoura, apor, autom, imple, protec, conju, foreig, aeronau, identi, purpose, diversi, conten, chrono, counc, nostal, nothing, oura, congreg, archae, simpli, arche, inste, nomin, homo, formul, precau, disintegr, accu, concer, carre, casser, intimid, succes, multip, antag, liken, contribu, admini, civil \\\midrule
596 & taliban, catwoman, paintball, manta, aryan, godzilla, rubio, brees, yellowstone, thatcher, septic, gemini, streep, lotto, vodafone, bambi, sumo, labyrinth, thunderbird, pixar, katniss, buddhist, submarine, sephora, chipmun, mannequin, ferris, dola, oktoberfest, retriever, buffett, dressage, harvard, toddlers, starfish, gibbs, tux, biden, gnome, palms, ritos, wolverine, keanu, depp, ufos, volta, kermit, usaid, stonehenge, cleopatra, hindi, illary, legos, linkin, montessori, gangnam, mayweather, yosemite, hyatt, kohl, justices, alpac, kruger, sphinx, terrier, ozzy, swan, oahu, milford, ellini, toto, tropic, pvc, gatsby, albino, benghazi, mayday, orchid, vigne, auburn, twain, silicon, wolff, corgi, khaki, imac, sable, cowell, pyramids, splatoon, utopia, mustang, mcfarlane, enos, nike, oprah, comet, gogh, muppets, hendrix, byu, sachs, korn, tarzan, gotham, goku, ajith, caterpillar, bluejays, gators, ebola, theri, raqqa, acea, cougar, antarctic, bauer, eros, lannister, sriracha, meryl, raven, putin, simba, starcraft, kobe, pitbull, bullock, mermaids, teaparty, norris, stant, pharaoh, cosby, violet, mccormick, tekken, metallica, addams, tutu, rouge, barack, cheetah, zuma, giraffe, plankton, gladiators, census, magnum, ukip, spielberg, rainforest, munster, timberlake, crimea, cayenne, whisky, stork, yoshi, dota, scorpio, dinosaurs, amarine, kombat, mccartney, greco, saltwater, spongebob, colonial, neon, tician, skyrim, aladdin, windmill, mlin, stingray, chimp, sony, beagle, mington, hathaway, tuxedo, cupid, buccane, sherlock, indigo, bieber, bobcat, minaj, dolby, mulligan, scuba, kurds, mormon, versa, pixie, pewdiepie, motorola, sade, dupont, clooney, hulk, glaciers, potassium, blender, nickelodeon, chess, cramer, cnbc, avril, pompey, saber, alpaca, ronaldo, sheeran, blazers, alligator, scrabble, loon, monopoly, filet, shiva, javelin, bluray, goliath, wicklow, dipper, briggs, bamboo, boomer, nemo, cedar, stormtrooper, unicorns, ballet, sperm, raccoon, nikon, gamecube, skeletons, everglades, blond, campos, tahoe, trex, burgundy, blonde, padres, beret, lakers, knicks, bacca, barrymore, freud, goldberg, pepsi, birdman, forkids, wahlberg, ghetto, dorado, malala, razer, ballerina, latex, husky, bowser, surya, koala, alpine, crimson, celtics, ferns, rihanna, abrams, calico, ayurveda, miku, rajinikanth, ubuntu, macfarlane, zumba, coyote, carp, atari, firefox, witcher, jain, dhoni, adolf, agave, iggy, eminem, disneyworld, colosse, marlins, jellyfish, linux, flamingo, hercules, banjo, chanel, kangaroo, norse, domino, cannes, olaf, fargo, churchill, chakra, adata, thunderbirds, azalea, zeppelin, polka, lenin, coyotes, labrador, garfield, cascades, dolly, orcas, genie, cology, barbie, fairytale, hippo, cajun, kinder, jackman, trident, cherokee, malibu, emu, kahn, unicorn, rousey, naf, mohawk, nixon, blackfish, loki, capri, cadillac, muppet, gaga, mandu, griffith, hamlet, reggae, enzymes, crowe, steelers, darth, deadpool, cern, ghostbusters, frankenstein, pluto, vegans, mayan, volcanoes, hebdo, llama, grizzly, mccain, rubin, zebra, madonna, sume, chrome, orca, elmo, glacial, sloth, skunk, sharapova, molina, netanyahu, iceberg, volcanic, fossils, buddha, tiki, dune, tedx, merkel, mellon, skywalker, reddish, venom, pikachu, cobra, johansson, bengali, rudolph, outback, otter, badminton, brunette, collagen, magenta, orangu, optimus, maxi, macklemore, kaku, antigua, homer, bundy, helix, snowden, steampunk, congo, riesling, tyga, whiskey, puma, prada, ember, ymca, schwarzenegger, leopards, guinea, coldplay, panda, palin, robo, bumblebee, elk, octopus, rolex, colon, mishra, hula, leno, toberfest, cholera, polo, tuscan, baylor, sinha, gumbo, coral, supermoon, doge, zuckerberg, baghdad, ffes, brero, zambia, mandela, durga, tamine, napoleon, possum, hedges, colbert, sundance, browning, terriers, amish, terracotta, tibet, everest, kfc, crocs, bronte, looney, monoxide, hanson, yoda, phillies, gameboy, bison, elites, neurons, dalmati, kites, gopher, camouflage, tidal, tesla, netflix, dancehall, argyle, haider, punjabi, messi, gothic, vatican, daytona, galloway, chrysler, boko, limbo, falcon, viper, foxx, sunflowers, flappy, ferguson, leblanc, turk, beyonce, hiddleston, einstein, hawkeye, creole, macau, nadal, gallons, mullet, poppies, nokia, hearthstone, mosquitoes, gator, kite, bridesmaids, rainbows, pajama, typewriter, fender, douglass, bernardino, chucky, bulldog, westlake, mmings, sabre, ingrad, monsanto, kapil, pox, aristotle, arches, twister, wiiu, treehouse, lunar, calcium, moonshine, zimmer, jeb, bulldogs, snoopy, cardinals, gandhi, diwali, monet, yachts, incense, gibbons, buccaneers, dicaprio, opry, merle, orphans, vulture, dulce, bucharest, fern, grette, hemp, buddhism, mccann, triton, koch, vmware, rooney, peterson, plato, tropics, nutcracker, dinosaur, badger, mantis, poppins, sharpie, bongo, algae, polar, hdmi, scorpions, bacteria, lullaby, unborn, chaplin, oracle, viruses, clegg, spock, diaz, lava, rogen, wiener, bosch, conan, kovich, donetsk, chewbacca, scorpion, mley, weasel, hemsworth, amigos, suarez, tibetan, bluebird, snowman, stallion, snooker, longhorns, farage, beyoncÃ©, lebron, heimer, sith, helium, quaker, discus, morrisons, leopard, yoona, celtic, turin, brics, macbook, nister, roblox, dredge, emerald, donkeys, dodgeball, mosquito, wrestlemania, goro, poodle, kanth, crombie, lolita, soros, vegan, epcot, ophobia, collie, werewolf, famine, nero, simpsons, shetland, rudolf, saurus \\\midrule
597 & color, colored, colour, color, colours, coloured, colors \\\midrule
598 & assist, support, supports, assistance, help, supported, helps, assisting, helping, helped, supporting, help, assists, assisted \\\midrule
599 & vie \\\midrule
600 & tu, ou, um, glu, uk, mu, u, us, uc, un, nu, ug, oun, ud, ut, usa, anu, uu, uri \\\midrule
601 & roof, hallway, ounge, room, ground, flooring, roofing, walls, floor, legs, leg, wall, ground, lounge, floors, carpets, roof, rooftop, ceiling, roofs, carpet, rooms, wall, floor, room \\\midrule
602 & preten, pretending, pretend \\\midrule
603 & floyd \\\midrule
604 & whis \\\midrule
605 & hits, hit, hit, hitting, singles, click, tap, hitter \\\midrule
606 & us, me, `, him, ive, she, they, he, ich, we, you, i, u, ], it, im \\\midrule
607 & chop, chopped, chop, chops, chopping \\\midrule
608 & wi \\\midrule
609 & rin \\\midrule
610 & ape \\\midrule
611 & discussions, examiner, examined, examining, discover, examine, discussing, interpreting, understand, disagree, symposium, applaud, argue, debate, consider, unfold, investigates, agreeing, debating, explore, arguing, suggest, tackles, pondering, contemplating, discussion, examines, conclusions, confront, considering, discussed, propose, discuss, weighs, questioning, argues, debates, discusses, communicate, considers, investigate, explores, exploring, unpacking, ponder, argued, evaluating, discovering, evaluate, argument, arguments, explored \\\midrule
612 & pay, pay, worry, payment, paying, paid, salary, earn, spend, pays \\\midrule
613 & quickly, fast, fast, quick \\\midrule
614 & test, tests, testing, test, tested \\\midrule
615 & final, last, founding, last, parting, next, past, earlier, previous, lasts, remaining, final, yesterday \\\midrule
616 & wo, war \\\midrule
617 & solo, solo \\\midrule
618 & lily, ruby, lilly, lily, rose, pearl, rose, roses, rosa \\\midrule
619 & tam \\\midrule
620 & twitter, facebook, instagram \\\midrule
621 & punch, punching, punched, punches \\\midrule
622 & band, bandana \\\midrule
623 & turquoise \\\midrule
624 & pos, ph, pp, pc, p, ppa, mp, \$, pa, pt, ip, ped, pper, pim, py, per, pen, p, price, dp, pm, vp, rp, mph, ppers, po, sp, pers, comm, pping, ppi, ap, pk, ppy, ppp, pc \\\midrule
625 & im, jn, sm, kn, mam, sn, m, n, mr, hl, ml, mm, ym, mn, mx, mb, ms \\\midrule
626 & megan, ryan, ryan, ashley \\\midrule
627 & ry, by, ys, y, fy, cy, ay, ty, ey, oy, ary, ory, ney, y, ly, ny, ny, vy, ay, sey, yo, asy, sby, ddy, ony, ily, wy, ays, bby, eny, ys, illy \\\midrule
628 & tasting \\\midrule
629 & dug, dig, digging, digs \\\midrule
630 & som \\\midrule
631 & wax, flour, wax, waxing \\\midrule
632 & avocado, avocados, zucchini \\\midrule
633 & skates, skate, skate, skaters, skater \\\midrule
634 & scrolls, scroll \\\midrule
635 & sizes, length, size, sized, sizing \\\midrule
636 & pointing, pointed \\\midrule
637 & pitt \\\midrule
638 & trick, over, wor, dark, out, ever, under, ove, death \\\midrule
639 & ye, ge, ge, gue \\\midrule
640 & rent, rental, rentals, renting \\\midrule
641 & serial, emo, series, seri \\\midrule
642 & sailing, sail, sails, sail \\\midrule
643 & je \\\midrule
644 & volleyball, handball, volley \\\midrule
645 & multiple, multic, dual, multi, multi \\\midrule
646 & pal \\\midrule
647 & polish, victorian, polishing, portugal, turkish, danish, poland \\\midrule
648 & opener, open, open, opening, opened, premiere, opens, openings \\\midrule
649 & latin \\\midrule
650 & outlining, outlines, outline \\\midrule
651 & google, google, amazon \\\midrule
652 & lopez \\\midrule
653 & itu \\\midrule
654 & anti, electro, micro, inter, inter, trans, tran, counter \\\midrule
655 & col, scol \\\midrule
656 & dubs, dub, dub \\\midrule
657 & compliment, compliments \\\midrule
658 & casts, acting, artiste, heroine, actress, artist, casting, actors, actor, villain, cast, celeb, cast, actresses, writer, artists, celebs, celebrity, casted \\\midrule
659 & ard, ards \\\midrule
660 & christian, julia, melo, adele, ritchie, christy, mario, duncan, joanne, sara, newman, thor, bradford, crystal, greta, flynn, danielle, reilly, mason, quentin, cooper, debra, morgan, nicholson, rahul, willard, lauren, collins, elvis, kent, hannibal, britney, isabella, tabby, mathews, solomon, ayesha, michele, victoria, jennings, wesley, jane, robinson, daisy, oswald, johnson, erin, truman, kendrick, irah, sierra, colton, cole, kylie, bowers, arnold, spencer, thomson, kanye, blair, hammond, benjamin, ellen, rhett, macdonald, juliette, mcdonald, sarah, ramsay, morty, sheryl, gunnar, claus, brennan, leo, jenny, barrett, garcia, carey, sullivan, randolph, alfonso, santos, elton, juliet, katie, mcil, marley, mariah, abdul, claudia, mary, paulo, skye, lancaster, sinclair, alessandro, hilary, warner, monica, cody, canterbury, harper, gabrielle, ramsey, samantha, marian, diana, sonia, lester, carols, jupiter, cameron, lamar, dawson, dora, lizzy, ariana, vaughn, fallon, abraham, rhonda, francis, whitney, kennedy, jennifer, olivia, maggie, costa, watson, margot, roxy, kate, davis, lisa, wyatt, emanuel, quinn, meghan, adams, scarlett, brooke, carlin, matthews, cyrus, julian, romeo, stuart, lewis, elliott, scarlet, yates, deandre, harriet, mila, pooja, betty, kumar, wills, hawkins, osbourne, nicolas, christie, brittany, jefferson, ventura, lana, oliver, carson, stacy, elizabeth, atie, savannah, penny, sylvester, alejandro, guernsey, murphy, irvine, pearson, mcqueen, clara, miranda, stefani, vanessa, hale, zachary, akshi, jana, hailey, alexander, bryant, carolyn, tyson, connolly, nikki, tracy, roland, steph, susan, gage, emile, melissa, carol, luna, holly, joan, jade, jonah, janice, nichols, angelina, zac, bonnie, lolo, patton, jackie, leslie, nicholas, maria, patricia, christine, kerry, muhammad, sharon, michelle, laura, juli, illian, louise, abbas, ally, osborne, elly, kelly, francisco, becca, dolan, mitchell, pope, adel, benedict, amr, didier, shelton, penelope, gayle, harvey, bridget, flora, etta, eoin, benson, martha, cheryl, rivera, cass, stanley, sandra, sawyer, sami, carly, suresh, minnie, ryder, nicole, taylor, angie, jordan, linus, stella, brittany, waldo, harmon, madison, oscar, jett, presley, nadia, regan, nolan, diane, nicki, lennon, noah, norton, leonardo, obrien, sofia, khalifa, parker, carrie, alice, maguire, cristiano, lovett, vivek, martinez, skylar, lola, klein, louis, susie, finn, elliot, drian, lauren, moses, luigi, marino, hopkins, brigitte, ruth, zhang, carmen, lucy, everett, jackson, lene, sutherland, marco, jessica, winston, jenner, audrey, margaret, phillips, ashton, willow, abigail, griffin, charisma, roosevelt, annie, leah, rene, tatiana, agatha, jessie, andreas, selena, atlas, hazel, chloe, keaton, bea, sandy, katy, molly, michelle, johanna, shay, jolie, lindsay, judah, thornton, royce, lois, phelps, zelda, evans, astor, riley, winnie, dominic, sally, bruno, aurora, diego, carter, halle, baroness, clarkson, mcguire, toria, hannah, kapoor, douglas, lincoln, baldwin, dexter, apollo, dakota, kathy, holly, pedro, tracey, luis, wendell, kingsley, eliot, brody, anushka, calvin, miley, witter, clarke, vladimir, adriana, elmer, windsor, geneva, chrissy, bryce, nelly, alberto, chapman, amanda, alexa, abel, levine, trinity, elsa, cate, schneider, dorothy, otis, gabriel, stephanie, blake, drake, phine, harrison, marin, harlow, jacobson, shelby, katrina, esteban, bethesda, celine, wilson, alicia, rosemary, sweeney, rosie, pratt, laney, johan, parry, michel, williams \\\midrule
661 & jack, jacks, jacking, jack \\\midrule
662 & cyber, hack, hacks, hacked, hack, hacker, hackers, hacking \\\midrule
663 & documenting, documents, documentation, document, documented \\\midrule
664 & seg \\\midrule
665 & pickup, picked, pick, chooses, choices, pick, choose, picking, picks, choice \\\midrule
666 & usc, fighton, lsu \\\midrule
667 & capture, captures, captured, capturing \\\midrule
668 & file, folder, file, filed, filing, files \\\midrule
669 & tw, hash \\\midrule
670 & theatre, shakespeare, theatres, literature, midwives, theatrical, theater, realm, theater, festivals \\\midrule
671 & cowboys, cowboy, cowgirl \\\midrule
672 & chants, chant, wiggins, chanting \\\midrule
673 & gestures, gesture \\\midrule
674 & \ \\\midrule
675 & retro, antique, classic, historic, vintage \\\midrule
676 & fo, sou, fau, shu, fur, fu \\\midrule
677 & cauliflower, broccoli \\\midrule
678 & charging, chargers, charger, charges, charge, charged \\\midrule
679 & coating, vest, coats, weather, coat, coated \\\midrule
680 & chili, chilli, chilli \\\midrule
681 & et \\\midrule
682 & relax, relaxing, relaxed, relaxation \\\midrule
683 & line, lip, lin, liners, lining, wire, inline, eline, lineup, liner, lined, pline, line, lines \\\midrule
684 & ann, anne, anna, anne, ann \\\midrule
685 & haired, hair, hairs, hairstyles, hair, haircut, hairstyle \\\midrule
686 & bath, bathing, bath \\\midrule
687 & martian \\\midrule
688 & ast \\\midrule
689 & kat, kat \\\midrule
690 & across, behind, above, overlooking, against, over, throughout, dominates, towards \\\midrule
691 & mis, miss, miss, misses, missed \\\midrule
692 & stir \\\midrule
693 & wakes, wake, woken, woke, wake, waking \\\midrule
694 & chair, candidate, inventor, aide, stylist, translator, assistants, assistant, journalist, organizer, general, commander, director, caretaker, detective, owner, processor, agent, author, specialist, manger, presidents, producer, inspector, president, lawyers, minister, detectives, chiefs, coach, mister, founders, educator, officers, ruler, officials, instructor, dictator, coaches, pastor, associate, leader, collector, constable, principals, executive, broadcaster, chancellor, counsel, animator, creator, representative, chief, leaders, rabbi, owners, campaigner, professor, innovator, managers, coordinator, spokesman, agents, deputy, manager, commanders, investigator, consultant, principal, editor, commissioner, operator, capt, captain, partner, correspondent, directors, counselor, premier, creators, members, official, colleague, designer, attorney, psychologist, ambassador, veteran, officer, promoter, coach, founder, ceo, chairman, mayor, ologist, diplomat, marshal, adviser, therapist, cinematographer, captains, secretary, choreographer, advisors, executives, admiral, filmmaker, spokesperson, ceos, member, comrade, controller, lawyer \\\midrule
695 & uni \\\midrule
696 & plat, plates, plate, mantle, platter, plate, tray \\\midrule
697 & ists, ist, alists, ism, dism, isi, isms, ist, onists, deshi, jitsu, ird, sist, istic, sted, sect, stic, stra, arist, logist, mounts, alism, stree, tist, alist, stics, tionist, dist \\\midrule
698 & tom, don, paul, dick, johnny, ron, jean, tom, dwayne, victor, doug, sean, dan, kim, alex, don, sheldon, martin, roger, brad, anthony, benny, david, perry, juan, jeremy, woody, bolton, walt, albert, justin, matthew, todd, carl, garry, harry, derrick, dwight, darryl, nathan, mick, micky, phil, andy, nick, reggie, billy, bernie, timmy, matt, scott, gerard, daryl, jake, josh, jim, gary, barry, fred, stewart, jeff, roy, vincent, phil, marshall, jim, tony, ricky, pete, frank, dave, nicky, jesse, bryan, jonny, evan, tino, toby, amy, wade, chad, carlton, ronald, neil, william, steven, fred, kenny, darrell, john, joh, gordon, richard, charles, teddy, dirk, ross, freddie, dean, wayne, rory, christopher, clark, claude, matt, hank, philip, tim, adam, salman, robin, alvin, herman, ben, howard, rich, glen, alan, aaron, clive, jon, jose, russell, simon, george, marc, clint, rick, roddy, tommy, rick, dennis, manny, arthur, jean, mitch, ron, craig, victor, derek, daniel, corey, louie, keith, luke, mickey, sam, malcolm, wendy, hal, marty, bill, allen, damon, butch, teddy, marty, gabe, terry, vern, vince, grant, james, todd, kelvin, ralph, stephen, jerry, shane, larry, neal, paddy, greg, leonard, thomas, johnnie, sonny, gerry, jay, alec, mikey, mack, barry, neil, jason, tyler, brian, robbie, trey, eric, steve, stevie, eddy, scotty, jamie, troy, kevin, nick, patty, andrew, robin, zach, rodney, rod, rex, jimmy, philippe, walter, jimi, joe, hugh, joseph, darren, brock, phill, eric, seth, adam, bernard, warren, gerald, shawn, bill, donald, judy, grant, mathew \\\midrule
699 & sid \\\midrule
700 & freddy \\\midrule
701 & sting, tting, tted \\\midrule
702 & electrical, electronic, electric, electronica \\\midrule
703 & donald, obama, clinton, obam, trump, trumps \\\midrule
704 & rating, rated, ratings, ranking \\\midrule
705 & 6, 1, 7, 8, 9, 3, 2, 5, 0, 4 \\\midrule
706 & patch, patches \\\midrule
707 & structure, form, balance, shape, forms, formations, formed, shaped, structures, forming, shapes, formation \\\midrule
708 & ple, pl \\\midrule
709 & sh, sh, eth, shi, ash, shi \\\midrule
710 & mechanic, plumber, mechanics, mechanical, cyclists, cyclist, mechan \\\midrule
711 & catch, caught, steals, catching, catches \\\midrule
712 & rian, tton \\\midrule
713 & redhead \\\midrule
714 & pharmaceutical, manufacture, printing, automotive, aluminium, manufacturing, production, aerospace, agriculture, printed, manufacturers, industrial, industri, manufac, print, manufactured, economic, agricultural, textile \\\midrule
715 & anim, animated \\\midrule
716 & kong \\\midrule
717 & kerala, portuguese, malayalam, telugu, kannada \\\midrule
718 & champion, champions, champ, championship, championships \\\midrule
719 & iron, ironman, irons, iron, ironing \\\midrule
720 & cartoon, cartoon, toons, cartoons, cartoonist \\\midrule
721 & excer, excerpt \\\midrule
722 & hole, circles, hell, tholes, repeats, shuffle, holes, circle, atters \\\midrule
723 & mike, bob, micheal, chris, michael, bob, mike \\\midrule
724 & load, loads, loading, loaded \\\midrule
725 & dig \\\midrule
726 & complex, squared, square, alphabet, square, sq, squares, sq, cubic \\\midrule
727 & strategy, plotting, plot, proposal, plann, planning, plans, plan, plots, ideas, strategies, policy, planned, policies \\\midrule
728 & chatting, chat, threads, chats, chatted \\\midrule
729 & scra, scrap \\\midrule
730 & food, food, meal, meals, foods \\\midrule
731 & hosts, host, hostess, hosted, hosting \\\midrule
732 & dise \\\midrule
733 & grilling, grill, grille, grills \\\midrule
734 & elli \\\midrule
735 & read, ite, reb, rein, vou, une, medi, prest, cri, are, rapp, sor, energ, aren, rec, scam, isra, rai, deta, reven, sec, vec, ferr, dre, rever, mee, dist, bei, asse, nor, rela, hei, reli, real, abil, ibi, nex, suc, electr, cruci, fini, choo, meme, evi, scre, recei, ffe, vive, reen, tear, elec, reale, lear, param, liber, rei, aqui, boo, gre, pre, kre, erc, wea, demon, tre, rest, vari, ire, entr, exc, scien, tsi, fre, stre, exer, fun, rele, fore, fas, spra, prote, reci, tori, thor, shad, wre, cere, bre, reas, spr, alter, entre, disp, perio, repe, defin, rt, nes, solu, fear, diss, fron, fen, resi, cele, brea, ffer, tec, isu, dis, re, sear, mem, fam, revi, ferre, rel, geor, publi, agre, ide, visi, refu, geo, pei, nov, fac, mess, celi, ones, elev, force, seren, ren, offic, escu, spa, stere, pren, fati, projec, reno, tere, veri, kne, spro, where, fab, aber, radic, vege, besto, ros, dent, sri, assi, de, cess, dest, infe, tex, bran, cit, excell, reall, resc, fra, arc, unic, rep, reve, rev, inv, dec, rak, avar, extrac, exp, enor, trade, arre, act, rhe, radi, edu, vivi, ema, thre, rese, ope, movi, emb, exe, retro, res, rw, wei, aler, thero, desi, def, part, milit, change, esc, sre, debu, frac, serv, here, morri, persi, grac, regi, freef, enter, reco, elo, vers, nev, mir, eman, exi, rebel, newe, aver, restaur, reck, extr, rub, feren, transpor, wer, kare, ave, tain, regre, ces, ate, bene, refe, kee, spear, sme, reh, eer, hea, dei, trek, thou, diam, arac, has, dee, bree, deser, rema, endo, ree, edic, turi, store, islam, reta, ace, rl, twe, apr, inde, resu \\\midrule
736 & sub, sub \\\midrule
737 & mid, mid, middle \\\midrule
738 & wit, ty, dry, dra, chit, asi, loo, fin, pee, tri, ki, nig, ti, indi, try, tsh, pig, koo, tian, lat, tee \\\midrule
739 & bles, able, ble, mable, ered, bility, durable, ability, sible, ables, vable, lable, rable \\\midrule
740 & vi, vic, vin, viv \\\midrule
741 & stadium, council, malls, island, planet, crescent, towns, mahal, wilderness, gates, kingdoms, quarters, lane, ballroom, union, motorway, quarry, empire, marketplace, museum, location, circus, crown, city, outpost, countdown, parliament, triangle, pharmacy, mall, stables, villa, resorts, airways, memorial, dairy, subway, racecourse, booths, arena, shops, parkway, inlet, stores, club, chapel, outlet, store, country, coastal, motel, heights, northside, camp, manor, mosque, dome, zone, homeland, cafe, boutique, oasis, playground, caves, towers, villages, warehouse, abbey, shop, riverside, coastline, harbor, festival, docks, pocket, coliseum, tower, terminal, hotel, township, circuit, markets, waterfront, summit, canteen, gate, metro, roadside, ouse, monument, rapids, island, rink, village, countryside, broadway, armory, halls, cove, arenas, league, fountain, sville, route, aisle, winery, overlook, steakhouse, shop, empires, revolution, patrol, bridges, salvation, ville, fort, campsite, harbour, corner, factory, gallery, arcade, cottages, anchor, branch, dock, sworth, nowhere, downtown, campground, booth, clubhouse, marathon, shipyard, mill, peninsula, stations, shelter, chambers, basin, tavern, market, castles, newtown, garage, castle, ashore, lagoon, cave, camps, suburb, gardens, quarter, bazaar, zoo, estates, hotels, motors, colony, plantation, museums, ports, bazar, highways, canal, estate, corners, habitat, leagues, port, neighborhood, path, arsenal, kingdom, area, academy, bay, ballpark, borders, district, ave, zones, dominion, uptown, shack, corridor, prison, town, mart, thames, carnival, mills, courthouse, hometown, tombs, city, lakeside, graveyard, lanes, town, wonderland, parlour, republic, cottage, isle, ranch, cemetery, bookstore, airport, seaside, province, stown, forums, drome, marina, opera, mansion, expo, islands, inn, reservation, midtown, galleries, cities, supermarket, thouse, norte, fest, depot, plaza, junction, parlor, pub, forum, coast, pavilion, casino, commons, ceme, shoreline, parade, pastures, lighthouse, meadows \\\midrule
742 & come, comes, came, coming, come \\\midrule
743 & seated \\\midrule
744 & channel, network, networking, influence, connections, hub, geographic, channel, conne, connecting, connect, channels, communications, connected, communities, community, networks, connec, connection \\\midrule
745 & region, vampire, valley, speedway, valley, raceway, temples, temple, delta, lakes, mountains, valleys, glacier, canyon, desert, highlands, monastery, prairie, weaver, river, canals, dunes, walden, cathedral \\\midrule
746 & uga, uk, teh, fi, gar, gh, ati, har, int, dai, ari, pas, ku, aki, op, adi, pi, ti, naw, bi, fu, ji, un, ul, ut, yu, hou, gal, aw, lat, thi, you, ig, ang, si, tai, thr, ot, agh, sir, tus, pak, ju, rai, ind, thia, sai, sa, au, ya, af, ung, hai, ai, dit, aii, ake, atta, ic, ish, waz, issa, lau, pur, kar, ft, wo, gon, tr, ont, ci, sk, ouf, ue, fo, tha, hel, wi, burg, eli, ye, bu, vi, ei, achi, tw, ri, li, zn, una, uni, hari, bah, ba, zai, chu, ood, ah, thou, kus, ab, itti, oli, ini, athi, um, gu, yal, hu, iri, yang, lah, da, tor, ota, wh, ool, tn, aa, abe, ef, uo, oya, ag, kl, kh, pathi, wie, fd, asi, phy, tf, eh, shu, eu, ow, ud, aga, ili, oon, tah, fus, hei, aus, ahu, fah, att, oth, tu \\\midrule
747 & greenery, green, green, greens \\\midrule
748 & mic \\\midrule
749 & eagle, eagles \\\midrule
750 & selfie, eclipse, elfie, tattoos, tattoo, selfies \\\midrule
751 & pas, vis \\\midrule
752 & nat, nat \\\midrule
753 & bane \\\midrule
754 & ste, sto \\\midrule
755 & nail, nails, nail \\\midrule
756 & but \\\midrule
757 & googled, goog \\\midrule
758 & stats, score, scoring, result, scores, results, outcome, scored, scoreboard \\\midrule
759 & fishing, fish, fishes, fish \\\midrule
760 & vlog \\\midrule
761 & alibaba \\\midrule
762 & wel, wh, wis \\\midrule
763 & claimed, claim, claiming, claims \\\midrule
764 & adventurer, rapping, drivers, chainsaw, guitar, keyboard, projector, cleric, pianist, binder, barista, waitress, rappers, paramedics, telescope, bmx, skier, server, tutor, hairdresser, caster, quarterback, diagram, yorker, trainer, olympian, motorcycle, screwdriver, steering, flyers, piper, adapter, composer, archer, thrower, screenplay, dslr, bowling, drones, parachute, defender, diner, archers, nurse, iders, astronauts, bikers, divers, driver, shifter, fundraiser, fashionista, cello, streamer, iliary, pharmacist, rocket, bartender, kickboxing, saxophon, umpire, carpenter, golfer, reporter, rollercoaster, turbines, synthesizer, conductor, medics, qb, singer, fishermen, puppet, windshield, frisbee, rockers, blocker, concert, chopper, sprinter, rapper, racket, medalist, sheriff, rocker, priests, pitcher, guitarist, violinist, pitchers, motorbike, goalie, astronomer, player, hottie, trainers, drone, streamers, coaster, goalkeeper, rector, reporters, bass, indycar, comedian, drums, diver, synth, dubstep, astronaut, trumpet, waiter, fangirl, launcher, singers, motorcycles, drummers, saxophone, smoker, blower, forklift, mathematician, physio, comedians, biker, jockey, kicker, lifter, keyboards, piano, courier, youtuber, chefs, smokers, recorder, racers, flute, carrier, sniper, spinner, goaltender, batsman, clarinet, logger, tumbler, soloist, guitar, turntable, punter, kilt, accordion, songwriter, dentist, catcher, paramedic, casters, drummer, printer, stoner, pundit, harp, percussion, bowler, caller, handler, glider, airtel, airplanes, tanker, servers, magician, announcer, loader, cpu, defenseman, medic \\\midrule
765 & spark, sparks, sparkles \\\midrule
766 & male \\\midrule
767 & farmer, farms, farm, farming, farm, farmers \\\midrule
768 & imaging, ill, ids, arch, ill, id, id, dren, drug, ral, oid, oids \\\midrule
769 & ufc \\\midrule
770 & outfits, outfit \\\midrule
771 & spi \\\midrule
772 & look, looking, searching, looks, looked, lookin, glance \\\midrule
773 & applications, apps, app, application \\\midrule
774 & ant \\\midrule
775 & grown, grew, grow, grows, growing \\\midrule
776 & cn \\\midrule
777 & blind, blind, blindness, blinds \\\midrule
778 & there, ven, en, eng, end, ek, ner, fran, yn, or, ene, tn, eni \\\midrule
779 & ame \\\midrule
780 & acne, face, toes, faced, mouth, skin, facial, voice, brow, lips, ear, forehead, tooth, cheek, teeth, cheeks, brows, noses, ears, eyebrows, neck, faces, eyes, toe, eyed, tone, breast, throat, tooth, mouth, skin, mouths, tears, jaw, facing, face, eyebrow, eye, nerve, nose, voice, tongue, scars, skins, necks, waist, scalp, eye, knee \\\midrule
781 & care, care \\\midrule
782 & ho, ha \\\midrule
783 & reader, viewing, reads, speech, feed, readers, feeds, singing, coding, feeding, playing, reading, counting, sharing, translate, sorting, readings, writing, texting, briefing, receiving, feed, voting, planting, read, translating \\\midrule
784 & h \\\midrule
785 & rushing, cycling, jog, runners, run, running, runs, jogging, ran, runnin, runner \\\midrule
786 & may, ca, sma, mad, dad, ma, nad, mai, meg, map, mad \\\midrule
787 & buffy \\\midrule
788 & stat, state, state, national, states, sate \\\midrule
789 & rob, robert, rob \\\midrule
790 & cheesy, cheese \\\midrule
791 & ails, ders, dc, ds, ds \\\midrule
792 & snap, snapped, snapchat, snap, snaps, snapping \\\midrule
793 & character, characters, character \\\midrule
794 & ro, ton, ori, cor, oc, os, pe, ore, chro, to, no, con, on, o, of, pom, po, od, ano, bo, ob, acon, ah, oo, ov, sco, iso, yo, op, osc, tc, ero, moo, ok, sof, oe, ole, omo, onto, aco, amo, alo, apo, ome, cos, ong, ow \\\midrule
795 & orchestra, group, sections, choir, bands, section, band, chains, chorus, chain, groups \\\midrule
796 & beats, then, than, least, except \\\midrule
797 & whi \\\midrule
798 & cha, br \\\midrule
799 & horse, cart, railway, boating, horses, canoe, boat, wagon, lorry, horse, motor, bike, yacht, train, planes, camper, plane, pots, ambulance, helicopter, trains, locomotive, boats, boat, truck, tanks, carriage, rail, tents, train, airplane, engine, ships, truck, pot, containers, horseback, carts, container, trucks, aircraft, bikes, tractor, engines, railroad, vessel, tractors, wagons, ship, vessels \\\midrule
800 & windows, windo, window \\\midrule
801 & hop, jump, jumps, bounce, hopping, jump, jumping, jumper, jumpers, jumped \\\midrule
802 & hu \\\midrule
803 & leave, leaving, leaves, leaf, foliage, leav, leafs \\\midrule
804 & tric \\\midrule
805 & request, requesting, requests, suggestions, requested \\\midrule
806 & nar \\\midrule
807 & tay, shan, sha, shav \\\midrule
808 & bri \\\midrule
809 & ver, vers \\\midrule
810 & ith \\\midrule
811 & california, ga, ca, cas \\\midrule
812 & out, upp, away, sup, up, together, outs, ups, dup \\\midrule
813 & shak, bay, ji, agu, say, pon, kap, bau, jab, lam, na, cas, aqu, grand, om, lak, tem, rail, pam, jac, yam, pan, cp, mas, mon, pat, ham, wag, kame, abou, bam, bag, ku, flam, mak, maro, ath, cam, mar, cun, nom, kam, lass, vr, bk, chan, am, jun, mani, avent, asa, ram, yong, nay, ang, cham, ja, dan, smar, shar, kor, zu, hon, tang, nag, zam, yom, kom, anth, abu, abe, lim, any, sa, yu, mv, aim, chak, kla, ami, salam, sura, sam, jam, kay, megam, mang, ao, tak, hart, sab, mom, kha, amaz, samu, acap, ake, shaw, mass, rang, hg, shal, gat, bon, amer, jan, mau, shin, amar, nan, tumb, cab, zar, sham, ais, pand, camar, anam, tan, bac, vas, vam, bagu, mc, ank, mari, nav, chann, way, arri, sem, apar, isi, arn, wam, pran, phan, sant, milk, kag, anc, mul, rash, chim, hum, alay, tun, ani, daw, ach, jag, nak, mash, aram, pah, kh, wan, yan, nap, kau, sap, bang, tz, kab, sum \\\midrule
814 & spec \\\midrule
815 & cannon, gun, weapons, knife, pistol, sword, guns, firearm, gun, weapon, weapon, sword, arms, rifle, cannons, trigger, gunner, cartridge \\\midrule
816 & bows, bow, bow \\\midrule
817 & reached, reach, breach, reaching, reaches, breaches, scaling, achieve, achieved \\\midrule
818 & sewing, loaf, bakes, baked, woodworking, baking, drying, bake, bakery \\\midrule
819 & releasing, launches, released, publishes, release, unveiled, launch, releases, debuts, launched, launching \\\midrule
820 & noodle, noodles, ramen, pasta \\\midrule
821 & =, > \\\midrule
822 & mermaid, mer, ban \\\midrule
823 & ski, skis, ski \\\midrule
824 & peop, mudder \\\midrule
825 & gu, gone, gon, goes, goin, going, go, go, goo, went \\\midrule
826 & win \\\midrule
827 & bout, involved, about, surrounding, around, wit, abt, regarding, about, concerning \\\midrule
828 & ward, bart, wards \\\midrule
829 & hyper, hyper \\\midrule
830 & ie \\\midrule
831 & mag \\\midrule
832 & marching, march, marches \\\midrule
833 & mics, mic, microphone \\\midrule
834 & v, v, var, av, vol, ev, va \\\midrule
835 & cking, cks, ck, ck, cked \\\midrule
836 & incompetent, tional, psychological, articulate, wearable, enclosed, factual, ethnic, disciplinary, rical, northeastern, infinite, edible, airborne, quantum, martial, influential, critical, static, imperial, volatile, renaissance, verbally, nonstop, aggressive, governmental, stationary, superior, rectangular, aluminum, confined, emotionally, deliberate, molecular, opathic, panoramic, makeshift, legendary, translucent, statistical, parallel, umatic, upright, spiritual, versatile, scholastic, dynamic, periodic, sideways, acclaimed, succulent, alternative, privileged, electron, alternate, binary, friction, universal, inappropriate, comedic, explicit, televised, protective, irical, evergreen, sustainable, baseline, intercontinental, metabolic, symbolic, centric, daytime, metropolitan, renewable, catastrophic, acoustic, extreme, handheld, cultivated, downward, dangerous, ancient, philosophical, confederate, complicated, heavyweight, aromatic, territorial, senting, reactive, landmark, recreational, geometric, atable, underwater, inverted, favorable, runaway, motivational, animate, developmental, artificial, urban, defensive, compatible, isolated, beneficial, tribal, humanities, affordable, residential, singular, balanced, lucent, predictive, nourished, populated, unconscious, magnitude, forensic, illuminated, constructive, impromptu, captive, icular, underdog, felony, premium, antioxidants, dominant, horizontal, logical, hydrating, negative, robotic, elaborate, overboard, sensory, mythical, gical, meaningless, structural, unconventional, verbal, internal, visible, intellect, charismatic, supernatural, nighttime, advanced, biographical, stical, visually, affectionate, pedestrian, spatial, itative, contrasting, lethal, natural, mathematical, practical, invasive, pelvic, monumental, misunderstood, unmanned, transgender, profitable, radiant, medieval, shirtless, orthopedic, homosexual, traumatic, enriched, lightweight, realistic, partial, introductory, intricate, racially, circulating, collegiate, cellular, skilled, specific, secondary, ometric, bodily, divergent, heated, harmless, victorious, interstate, tional, barefoot, alcoholic, imaginative, ballistic, social, terrestrial, fictional, scopic, intimate, surgical, precision, planetary, intellectual, rugged, macro, reproductive, poisonous, veterinary, environmentally, irrational, passionate, convenient, elevated, saturated, underlying, continental, vegetarian, seamless, disruptive, militant, repeating, temporary, hybrid, hazardous, atomic, responsive, transparent, destructive, rhythmic, explosive, tual, inflatable, unarmed, orthodox, despicable, neutral, healthier, interactive, unnamed, modern, creative, economical, appreciative, noxious, remote, integrated, neural, offensive, symphonic, responsible, abstract, patterned, pediatric, clockwise, geographical, efficient, undercover, concrete, radical, extremist, longtime, controversial, biblical, positive, reckless, diagnostic, invisible, vertical, bionic, cluster, emergency, oppressed, strategic, foreground, thorough, indigenous, gruesome, nutritious, historical, contemporary, angular, noticeable, architectural, elastic, productive, interstellar, paramount, suburban, personalized, fraudulent, inclined, atmospheric, conscious, customizable, median, analogue, virtual, comprehensive, manual, limitless, demonic, breakthrough, stainless, expressive, abundant, charitable, unidentified, traditional, nuclear, amphibious, genital, regional, aerial, synthetic, hydraulic, neurological, patory, tactical, competitive, ultimate, sentimental, specialized, ceremonial, baroque, independent, primary, classical, portable, peripheral, paranormal, problematic, organic, circular, intelligent, vitamin, particular, excessive, emotional, flexible, stimulating, spontaneous, prominent, astronomical, metrical, kinetic, energetic, apocalyptic, homosexuality, compound, controlled, distinct, cordless, reasonable, muscular, genetically, provocative, digital, unpopular, topical, conventional, miraculous, anonymous, devotional, disposable, medical, psychic, instrumental, realism, gravitational, autistic, dimensional, athletic, deadly, prosthetic, aquatic, hostile, fermented, orchestral, nutritional, analog, informal, embedded, generic, prehistoric, arial, adjustable, physical, herbal, fundamental, expansive, adventurous, accurate, biological, commanding, feminine, skeletal, testosterone, oversized, recycled, dramatic, mortal, reformed, oriented, mediocre, fluorescent, acquainted, ological, external, racial, revolutionary, hydrogen, millennial, tropical, perpetual, abusive, resistant, humorous, reluctant, alistic, encyclopedia, eccentric, modular, multipurpose, comfortable, axial, private, electro, sarcastic, sacred, ateral \\\midrule
837 & flick \\\midrule
838 & scen, scene, scenes \\\midrule
839 & done, do, did, doing, does \\\midrule
840 & pus \\\midrule
841 & unit, machine, hardware, system, conditioning, machines, operations, processing, robot, systems, machinery, apparatus, equipment, robots, units, dispenser \\\midrule
842 & ric, ri, pri, bruce, rid, ry \\\midrule
843 & point, magnetic, center, pts, centers, hough, points, centre, center, pointer \\\midrule
844 & nano, micro, nanotechnology \\\midrule
845 & myths, rumor, rumour, rumours, odds, leak, rumors, leaks \\\midrule
846 & sent, sending, send, sends \\\midrule
847 & upgrade, gardening, survival, upgrades, repaired, repairs, improvement, damage, rebuild, remodeling, maintenance, repairing, renovation, remodel, remodel, repair, renovations, makeover, rebuilding, restoration, inspections, reconstruction, improvements, archaeology \\\midrule
848 & gar, gel, dar \\\midrule
849 & lessons, lesson, wisdom \\\midrule
850 & bump, bump, bumping, bumps, bumped \\\midrule
851 & compact, compac \\\midrule
852 & present, gifting, presents, gifts, gift, gift \\\midrule
853 & filling, fills, fill, filled \\\midrule
854 & bet \\\midrule
855 & diag \\\midrule
856 & wheeling, wheels, wheel, wheel, wheeler, foot, ycle \\\midrule
857 & decade, year, month, season, episode, months, seasons, years, decades, season, period, episodes, seasonal \\\midrule
858 & sle, sled, sleigh \\\midrule
859 & sal \\\midrule
860 & southern, south, southern, grand, northeast, southeastern, southeast, horizon, south \\\midrule
861 & aveng, avengers \\\midrule
862 & businesses, services, profits, restaurants, charity, manufacturer, firm, provider, marketing, commerce, contractors, growers, software, companies, industry, investing, solutions, corporation, resources, suppliers, clients, partnerships, employment, healthcare, brokers, business, business, sector, corp, contracts, traders, partnership, product, partners, client, employer, corps, investment, consumer, nonprofit, contract, brands, profit, assets, revenue, startup, revenues, company, entrepreneur, startups, designers, airline, industries, entrepreneurs, franchise, corporations, enterprise, workforce, insurance, charities, biz, financial, products, capital, ventures, consumers, inc, economy, finance, developers, corporate, producers, investor, broker, businessman, contractor, investors, employers, agency, writers, investments, agencies, procurement \\\midrule
863 & philli \\\midrule
864 & set, setup, sets, setting, set, sett \\\midrule
865 & diff \\\midrule
866 & thanksgiving, christma, cruise, holliday, holiday, vacation, xmas, vacation, vacations, fantasy, resort, anniversary, hols, holidays, caravan, christmas \\\midrule
867 & woo, woo, whoo \\\midrule
868 & race, racec, race \\\midrule
869 & pray, praying, prays, prayer \\\midrule
870 & steal, enjoy, sneaking, bring, takes, taking, bringing, brings, take, take, brought, took, taken \\\midrule
871 & whole, whole, entire \\\midrule
872 & lucifer, devils, demon, evil, satan, devil \\\midrule
873 & laying, lays, lying, laid, lay \\\midrule
874 & stretching, stretch, stretched, stretches \\\midrule
875 & princess, duchess, princes, princesses, prince, cinderella \\\midrule
876 & packed, full, full, extended \\\midrule
877 & twenty, hundred, nine, thirty, eigh, dozen, three, two, ww, nine, fifteen, forty, twent, twenti, iv, sixteen, four, eight, eighteen, seven, century, zero, billion, eleven, million, ninety, fives, ii, seven, iii, fortune, ten, five, four, five, twelve, vii, six, sixty, fifty \\\midrule
878 & walmart \\\midrule
879 & blouse, ouses, consciousness, lotion, blazer \\\midrule
880 & patrick \\\midrule
881 & hot, hotter, spicy, heat, heating, sticky, cold, hot, chilly, warm \\\midrule
882 & rots, parrot \\\midrule
883 & tees, sweaters, shirt, bottle, comic, laptop, sweater, hoodies, sticker, tshirt, hoodie, jerseys, tshirts, tee, jersey, shir, stickers, shirt, sweatshirt, towel, towels, bottles, shirts \\\midrule
884 & second, third, minutes, seconds, minute, first \\\midrule
885 & clips, clip, clip \\\midrule
886 & opp, pr \\\midrule
887 & fossil, shell, shell, shelling, shells \\\midrule
888 & download, publication, downloadable, downloaded, downloads, uploading, downloading \\\midrule
889 & spots, spaces, places, space, spac, place, spot, space \\\midrule
890 & ber, aster, oper, rel, zer, sanders, sever, tanner, ffler, keepers, erman, angers, wer, keeper, acker, roberts, mand, rer, kier, asters, ler, ender, sley, moore, gers, ery, rell, erson, eck, ellers, erd, cutter, ff, akers, kov, palmer, hines, dier, apper, smith, eger, mer, berg, ware, fee, leman, turner, aver, walker, mey, yor, hanger, kley, vet, ggins, porters, bourne, stein, zel, ner, sher, itter, brien, ers, aser, ingles, ent, butler, aker, dery, eer, hardy, mper, bert, yer, ger, tier, wel, itor, fowler, lator, ager, nett, ander, enders, mers, meter, mant, ener, fer, baker, fier, reeves, sman, eler, berry, feld, lers, ret, meyers, dder, omer, lar, iller, eller, cey, er, meier, zers, gies, iser, neill, enes, rance, mber, zier, thier, ize, gher, hopper, holder, rogers, mcgee, ittle, rey, iney, teer, yser, mery, ier, iler, heer, rover, agers, gress, inger, cer, aler, decker, borne, mbers, hier, der, bery, ller, dee, wess, berger, dler, yers, bers, anner, garner, ffer, ners, gardner, aller, berman, arer, vert, sson, ggers, beater, ister, ader, tener, iter, lder, barnes, lier, ream, meer, timer, cker, zr, taker \\\midrule
891 & moose \\\midrule
892 & il, il, ils, phillip \\\midrule
893 & break, broke, breaking, breaks, break \\\midrule
894 & receiver, installment, option, returning, returned, returns, return, receivers, addition, arrival, comeback, debut \\\midrule
895 & sonic \\\midrule
896 & dbz, dragonball, batman \\\midrule
897 & comple \\\midrule
898 & mr, m, metre, ms, mo, med, mm, meters, mk, km, sm \\\midrule
899 & perspective, pov \\\midrule
900 & breaker, breakers \\\midrule
901 & dic, meat \\\midrule
902 & mccon \\\midrule
903 & tj, j, ja, jj, j, jc, aj \\\midrule
904 & ling, li, eli, ili, ly \\\midrule
905 & chase, chasing, scanning, chaser, chasers, diaries, chases, chased \\\midrule
906 & cut, cutting, cut, cuts \\\midrule
907 & tin, tins, tens \\\midrule
908 & gam, game, videogame, gamer, gaming, game, games, gamers \\\midrule
909 & wa, ware \\\midrule
910 & ex, sex, ex, exp \\\midrule
911 & jeep \\\midrule
912 & letterman \\\midrule
913 & zombies, zombie \\\midrule
914 & chall, challenges, challenging, competition, challenge, challenged \\\midrule
915 & pressed, press, presses, press, pres, pressing \\\midrule
916 & tonite, nite, tonight \\\midrule
917 & feel, feeling, feels, feelings, felt \\\midrule
918 & max, max \\\midrule
919 & layer, layered, layers \\\midrule
920 & buil, builder, build, builds, building, builders, building, built, buildings \\\midrule
921 & whe \\\midrule
922 & carries, holding, holds, carried, hold, carry, carry, held, carrying \\\midrule
923 & explo, dev, development, developer \\\midrule
924 & details, intelligence, confidence, inform, info, info, data, information, informative, educational \\\midrule
925 & ami, deen \\\midrule
926 & beauti, beauty \\\midrule
927 & sequ \\\midrule
928 & mini, mini, miniature \\\midrule
929 & crash, crashing, crashes, wreck, crashed, accident \\\midrule
930 & sri \\\midrule
931 & yellow, golden, rainbow, yellow, beige \\\midrule
932 & pla \\\midrule
933 & bb, bb \\\midrule
934 & titanic \\\midrule
935 & types, sort, typing, typed, sorts, type, kinds \\\midrule
936 & og \\\midrule
937 & stra \\\midrule
938 & cy \\\midrule
939 & focuses, focused, focus, refresh, focusing \\\midrule
940 & retreat, damages, serve, sample, serves, strate, prise, bolster, arriving, overflow, possess, assess, sneak, unites, control, settle, securing, consult, unleash, hurry, recovering, initial, enroll, adapting, commit, solve, borrow, direct, pause, prepping, adjusting, dispatch, recovers, suffers, access, adapt, preserve, insert, trace, restore, disposal, observe, protects, replace, scramble, compose, submit, attend, arrive, protecting, recover, subscribe, surround, approached, grasp, disguise, waited, recovery, remove, sprinkle, collide, arrives, preventing, reunite, arrange, compete, escape, decline, enters, waiting, approaches, unlock, portray, urgent, prepare, exchange, precise, indulge, prepares, adjacent, tends, sacrifice, repeat, awakens, overcome, cept, differ, apply, additional, descend, separate, predict, excess, sync, bother, erase, mourn, approve, overnight, awaits, avail, coordinate, reverse, pursue, enter, participate, prevent, abandon, separates, obtain, extract, competes, brance, rethink, adjust, replacement, avoid, stumble, satisfy, benefit, refer, fetch, geared, conquer, exchanging, achieves, detect, defend, remainder, execute, proceed, salute, brace, acquire, gearing, spread, manage, merge, donate, align, awaiting, inspire, tend, escorted, prior, operate, conduct, undergo, calculate, emerge, hydrate, entered, heal, survive, attention, immerse, cater, customize, awaited, recite, impress, managing, observing, operates, withstand, prompt, pregame, protect, accompany, inspect, pursuing, kickstart, await, prevents, resist, invade, prove, summon, locate, itate, absorb, collect, collaborate, emerges, accelerate, preparing, defending, standby, resolve, ignite, seeking, complement, bypass, awaken, deploying, advance, enrich, traverse, emerging, presale, activate, destroy, navigate, secured, compelled, occur, vening, release, entertain, anticipate, respects, paused, ready, awake, resume, attach, threaten, departure, dominate, secure, occupy, disrupt, regulate, relate, elect, facilitate, assessing \\\midrule
941 & velocity, epilepsy, qualifier, tribute, receptor, contender, duel, chaos, escort, automobile, trophy, sedly, finale, thumbnail, capsule, ignition, implant, auto, takeoff, bluetooth, borderlands, defence, portal, audition, infinity, courtroom, fantasia, generator, wireless, pixels, convertible, upstream, cutout, censor, watcher, tempo, airforce, standoff, cctv, index, flashlight, gamestop, suspense, concussion, predator, liberation, magnets, bootleg, intermission, boardgame, steamer, footpath, grime, gauntlet, thriller, ensemble, widget, stamina, offroad, constellation, gamma, overlay, skillet, relay, touchdown, lasers, symphony, doppler, closeup, safari, siren, matrix, supermodel, commando, frontal, freestyle, endeavor, anime, meditation, interchange, ballad, autos, medley, smartwatch, medallion, scrapbook, monologue, injection, smackdown, flyover, combo, compass, ovation, asteroid, extras, gadget, nascar, boyband, formula, actment, jackpot, autoshow, sensors, contour, coupe, panorama, asana, fringe, firework, defense, catalogue, recital, freeway, mover, joyride, autographs, maestro, apocalypse, gladiator, cascade, lifeboat, alloy, grenade, meltdown, sensor, checkers, prank, jurassic, prix, hamster, collision, auto, confetti, pictorial, chariot, collapse, valence, crossover, accelerator, mmorpg, fragrance, escorts, tollywood, antibody, fiesta, assassin, pistons, dashboard, immersion, artifact, dropbox, sportscar, tailgate, narrator, rebellion, broadband, underworld, fireworks, seizure, xfactor, radar, showdown, encryption, unison, scifi, titanium, lapse, pursuit, polymer, cityscape, rotary, android, gearbox, artery, revenge, nology, polaris, terminals, accent, checkpoint, cardio, stealth, vaccine, gridiron, fielder, dakar, semifinal, novella, foxsports, excavation, vortex, meantime, enary, subtitles, infusion, glitch, scrimmage, twitch, webcast, livestock, multiplayer, domain, ligament, eruption, satellite, epiphany, remover, parasite, voltage, solstice, trance, enigma, saloon, corpse, landrover, struction, inary, reflex, facade, wordpress, composites, motorsport, blockbuster, transmitter, animations, avatar, quake, vengeance, cursor, duet, reunion, equinox, explosions, expedition, valet, supra, fairway, voyage, password, roundup, asphalt, supercar, mulator, partition, acceleration, sequel, autograph, brutality, monarchy, havoc, quota, rampage, vitamins, americana, emblem, oxygen, choral, esports, rematch, verge, revolver, lightroom, endurance, overpass, csgo, gameplay, breakout, postage, neutron, torrent, sidekick, downstream, militia, diment, observer, convoy, rave, ipment, terminator, roundtable, montage, fireball, microscope, zenith, archery, vanity, torque, ticon, posse, vigil, orama, sphere, ssional, tarmac, module, mosaic, orail, inception, warcraft, paypal, novice, stride, clone, scanner, pageant, droid, improv, entertainer, ketball, browser, climax, toolbox, utility, traction, mimic, demolition, twilight, propeller, enduro, explosives, gunshot, slider, astronomy, billboards, backstreet, fiance, artillery, primer, seascape, breakaway, jazeera, kidnap, expanse, nament, powerpoint, infection, explorer, entourage, handshake, adrenaline, amphitheater, souvenir, battlefront, physique, bluegrass, descent, molecule, trove, nemesis, raptor, reactor, columns, polaroid, ophone, altitude, armored, timelapse, shuttle, strial, spaceship, sightseeing, outbreak, rollover, motocross, seeker, mammal, command, mileage, battalion, skyline, rundown, magnet, melee, combustion, galactic, gtav, spacecraft, illuminate, simulator, remedy, ecg, sportscenter, doomsday, meteor, vantage, midfield, procession, homage, kimmel, rodeo, knockout, meridian, finity, aroma, vertigo, warfare, mobiles, implants, lemans, trauma, horsepower, assassination, proxy, companion, leaflet, siege, forensics, webseries, frontier, troupe, disturbance, stampede, vandalism, navigation, hangar, streetcar, hazmat, vapor, genesis, tarot, singularity, marquee, minion, probe, vector, tripod, firmware, maxim, buzzer, satellites, raptors \\\midrule
942 & parties, palace, party, partying, picnic, invasion \\\midrule
943 & shaggy \\\midrule
944 & kayaking, skiing, hikes, snorkeling, hikers, biking, hiking, trekking, kayak, hiked, hike, hiker \\\midrule
945 & universe, galaxy, samsung, galaxies \\\midrule
946 & underwear, lingerie \\\midrule
947 & movies, book, anime, films, taping, film, filming, tape, albums, tapes, filmmakers, filmed, movie, dvd, movie, album, books, documentary, film, booklet, taped, book, dvds \\\midrule
948 & stic, sti \\\midrule
949 & ans, shers, vans, arians, tians, ics, wns, icians, icans, vian, ician, lins, ians \\\midrule
950 & por, tar \\\midrule
951 & boarding, board, boards, boarder, board, boarded, boar \\\midrule
952 & cleared, clear, calm, clarity, clearing, clears, clear \\\midrule
953 & fitted, installing, installed, install, installs, install, installation \\\midrule
954 & thought, thoughts, thinks, think, thinking \\\midrule
955 & ocean, ocean, wind, sea, water, lake, oceans, water, salt, tea, salt, river, sea \\\midrule
956 & ip, si, ik, ibm, i, ii, bi, thi, iw, io, ncaa, ai, ib \\\midrule
957 & cause, caused, causes, because \\\midrule
958 & gn \\\midrule
959 & creeper, creepy, scary, terrifying, creep, creep \\\midrule
960 & shoots, shot, shoot, shoot, spray, headshot, shootout, shooter, shooting, lamb, shots, shootings, shot, shooters, gunman, shotgun \\\midrule
961 & stro \\\midrule
962 & bicy, bicycle, bicycles \\\midrule
963 & sweetheart, dream, pain, giggle, passion, smiles, fear, happ, breath, minds, blessed, shout, grace, laughs, spirit, proud, bravery, relief, comfort, heartbreak, desire, soul, awe, ecstasy, envy, prosper, beauty, embrace, senses, emotion, shine, grin, harmony, lucky, breeze, manners, giggles, merry, heart, grace, spite, chance, soul, dreams, romance, blessings, royalty, moods, riches, delight, flair, miracle, agony, praise, blessing, laugh, moonlight, flames, happy, sexual, joy, glory, sweeter, fame, glee, heartbeat, silence, happiest, trust, hallelujah, fun, joy, rejoice, gratitude, sweet, treasure, emotions, favor, hello, hype, worship, glory, charms, holy, excited, laughter, respect, honesty, satisfaction, curse, wonder, courage, laugh, pleased, pains, happy, desires, hunger, magic, mercy, smile, crush, inspiration, luck, affection, treat, laughed, paradise, hello, laughing, happiness, smiled, honor, wonders, spice, talent, addiction, goody, kindness, amore, fever, heart, jealous, faith, spirits, mood, friendship, smiling, heck, applause, regret, amusement, pleasures, destiny, pride, unity, honour, charm, excitement, bliss, fitness, goodie, treasures, marry, patience, obsession, forgiveness, approval, dreaming, jealousy, freedom, warmth, greatness, peace, energy, pleasure, thrill, healing \\\midrule
964 & zo \\\midrule
965 & mma \\\midrule
966 & jerusalem, paris, milan, copenhagen, moines, indy, newyork, philly, nyc, barcelona, austin, mumbai, melbourne, brooklyn, singapore, cincinnati, oslo, delhi, denver, vegas, aviv, glasgow, penn, johannesburg, beijing, midwest, stlouis, philadelphia, knoxville, berlin, tampa, charleston, athens, atlanta, angeles, pittsburgh, nairobi, manchester, pennsylvania, valencia, sanfrancisco, miami, moscow, brussels, nashville, charlotte, tokyo, chicago, sacramento, indiana, oakland, indianapolis, budapest, delaware, dubai, dhabi, bangalore, toronto, boston, seattle, washington, sheffield, orlando, sydney, phoenix, dallas, london, milwaukee, york, springfield, baltimore, frankfurt, seoul, houston \\\midrule
967 & inj \\\midrule
968 & vision, mission, visions, vision \\\midrule
969 & drills, drill, drilling \\\midrule
970 & song, anthem, sang, hymn, song, songs \\\midrule
971 & lou, mo, smo, plan, lotus \\\midrule
972 & forward, forwards \\\midrule
973 & awhile, while, meanwhile, whilst \\\midrule
974 & makeup, makeup, cosmetics \\\midrule
975 & tunic \\\midrule
976 & wraps, wrap, wrapped, wrapping \\\midrule
977 & tight, close, close, closest, closer \\\midrule
978 & folding, foldable \\\midrule
979 & zy, rez, z, zi, zi, z, zzy, afro, zz, zer, zz, zzzz, zie, tz, zzi \\\midrule
980 & quitting, quit \\\midrule
981 & pics, pic, pic, pictures, pho, pictured, slideshow, photos, photo, img, image, images, imagery, photoshop, photo, photographers, visual, picture, photoshoot, stills, photographer, picture, photography, posters, foto, portrait, poster, photogra \\\midrule
982 & pun, qui \\\midrule
983 & blending, blend, blends, blended \\\midrule
984 & acrob \\\midrule
985 & tigers, tiger, tiger \\\midrule
986 & skirts, skirt, gown, gowns \\\midrule
987 & comment, comments, comment, commentary, commentator, commented, commenting \\\midrule
988 & teal, pink, purple, peach, orange, red, maroon, pink \\\midrule
989 & bowls, cups, bowl, cup, bowl \\\midrule
990 & home, home, houses, residence, hom, property, house, house, homes, domestic \\\midrule
991 & civic \\\midrule
992 & hours, time, adventure, timed, time, hrs, timing, times, moment, moments, imes \\\midrule
993 & teen, teenage, teens, teenagers, teenager, teen \\\midrule
994 & plug, plugs, plugged \\\midrule
995 & gwen \\\midrule
996 & marks, peter, mark, marking, marked, peter \\\midrule
997 & handed, gave, giving, gives, handing, give, given, give \\\midrule
998 & export, exports, import, exporting, imports \\\midrule
999 & conver \\\midrule
1000 & ded, dering, ding \\\midrule
1001 & side, side, sides \\\midrule
1002 & ini, ici, cin, men, min, sin, amin, oni, ingu, ain, in, jin, non, len, imit, quad, beat, pain, mit, nam, tin, inf, ino, ima, indu, ink, mont, ins, nin \\\midrule
1003 & aquarium, sofa, couch, sectional \\\midrule
1004 & goose, uck, crab, ducks, geese, duck, duck \\\midrule
1005 & has, thank, have, hasn, had, have, having \\\midrule
1006 & bored, stuck, miserable, exited, terrified, tripping, depressing, confused, traumati, exhausted, optimistic, worried, distress, sorrow, desperate, stress, grumpy, concerned, nerves, angst, sighs, infuri, restless, stressful, turmoil, skeptical, screwed, confusing, distressed, nightmares, tempting, harassed, fatigue, disturbed, uncomfortable, stressing, vomit, irrit, despair, hopeless, melancholy, tempted, frightened, worrying, frustrated, headache, dreadful, annoyed, scares, satisfied, angry, panic, intimidating, unhappy, offended, freaked, anxious, helpless, sigh, stranded, sad, comforts, cruelty, lonely, overweight, devastated, ptsd, suffering, worries, concerns, stress, urgency, refuse, obese, relieved, confusion, overwhelmed, discomfort, darkness, trapped, annoy, furious, depression, frustrating, gloomy, hungry, cringe, nervous, concern, depressed, disturb, confuse, nightmare, unlucky, troubled, stressed, anxiety, tired, unhealthy, ignorant, pathetic, struggled \\\midrule
1007 & spiral \\\midrule
1008 & bli \\\midrule
1009 & buffalo, buffalo \\\midrule
1010 & tit, atin \\\midrule
1011 & ea \\\midrule
1012 & ical, onic, ational, ction, ity, lect, tation, alize, sions, ous, dent, ption, fication, tives, ilation, ments, lage, mation, itude, cular, versary, mony, ment, iment, ance, ances, ment, vent, sion, scence, atures, atic, ency, sion, logy, sation, itive, ization, sity, cism, eness, ness, tions, ord, orial, vement, pathy, ature, tery, eries, phic, ination, stime, ation, tion, tones, gency, uous, liness, tial, matics, ative, vity, ulation, oric, tical, chment, lation, atives, tations, ety, cest, emission, ations, stion, logy, ancy, ssion, tivity, iness, ator, fications, mption, tionary, tion, sement, tive, lators, sive, itions, acy, alization, ious, ators, arly, genic, zation, sque, cture, logies, ctions, gement, ence, ation, tures, tish, ities, ience, nation, acies, icity, cation, atory, ality, dential, ition, itation, dition, ousness, ture, monia, veness, xion, manship, dence, itic, ories, rence, cion, ity, ssions, itudes, ssion, dity, tness, stration, shment, ements, omic, ions, ctive, ology, lessness, entary, ement, nesses, atio, vention, itious, inity, fulness \\\midrule
1013 & raising, raise, raised, raises \\\midrule
1014 & military, warriors, army, armies, navy \\\midrule
1015 & em, bone, emma \\\midrule
1016 & ber, beli, ker, bull \\\midrule
1017 & with, to, at, for, using, w, via, by, @, in, from, of, off, on, upon, along, [, onto, from, into \\\midrule
1018 & harley, mming, mmer, mmer, morris \\\midrule
1019 & mi, edm, gran, zyk, sims, cbn, mod, puri, font, gta, bil, oto, neuro, oman, lt, md, hi, pani, cns, bibi, som, rt, omy, furry, onal, vio, mods, mani, pj, vr, mire, hd, pri, min, nam, rus, amd, ob, cor, yuan, omi, mtv, psp, cci, mmo, wb, hue, forma, rj, bis, neu, nian, vips, mii, rss, inf, mile, nim, mea, fuji, pho, maha, lr, wny, indi, dii, rom, jid, sim, ris, minal, avi, jt, asus, ipc, umi, inian, nato, hilton, mint, aney, omni, gur, mbps, iwd, mod, kd, mms, wv, uti, imo, eme, bom, iny, dios, jun, omas, mi, nos, rion, tali, itary, sr, mundo, hg, lz, ib, apr, mcfly, acom, iche, mie, fm \\\midrule
1020 & bend, bending, bent \\\midrule
1021 & dgers, anders, dge, dging, dges, ennes \\\midrule
1022 & belly, tails, ponytail, tail, venture, hitch, tail, chair \\\midrule
1023 & angela, angel \\\midrule
\bottomrule
\end{tblr}

==> tables.tex <==
\textbf{``Hubness problem''. } 
The longstanding “hubness problem”~\cite{DBLP:journals/jmlr/RadovanovicNI10} in which a small number of database embeddings become the nearest neighbours of many queries, can negatively affect the performance of retrieval models. 
Recently, QBNorm~\cite{DBLP:conf/cvpr/BogolinCJLA22} a simple but effective method, has been proposed to address this problem. 
We incorporate QBNorm as a post-processing step in our experiments on MSR-VTT.
We find that QBNorm is able to consistently improve the performance of \ours, indicating that \ours still suffers from the ``hubness problem''.
In the future, it would be beneficial if aligned space can be able to alleviate the effect of “hubness problem” in multi-modal retrieval.
\begin{table*}[t!]
\centering
\caption{Ablation study on Hubness problem.}
\label{tab: temporal encoder and qbnorm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|ccccc|ccccc}
\toprule
\multirow{2}{*}{Model}                     & \multirow{2}{*}{QBNorm} & \multicolumn{5}{c|}{Text to Video Retrieval} & \multicolumn{5}{c}{Video to Text Retrieval} \\
                                           &                         & R@1    & R@5    & R@10   & MdR   & MnR   & R@1    & R@5    & R@10   & MdR   & MnR   \\
                                           \midrule
\multirow{2}{*}{Ours-MeanP (ViT-B/32)}     &                         & 46.8   & 74.8   & 82.6   & 2.0    & 14.1    & 45.6   & 73.2   & 82.4   & 2.0    & 9.5     \\
                                           & \Checkmark            & 47.0   & 73.9   & 81.8   & 2.0    & 14.5    & 45.7   & 72.3   & 82.0   & 2.0    & 9.6     \\
                                           \midrule
\multirow{2}{*}{Ours-seqTransf (ViT-B/32)} &                         & 48.7   & 73.9   & 82.7   & 2.0    & 13.5    & 46.6   & 73.4   & 82.0   & 2.0    & 9.2     \\
                                           & \Checkmark            & 49.1   & 73.9   & 82.8   & 2.0    & 13.5    & 46.9   & 73.8   & 82.1   & 2.0    & 9.3     \\
                                           \midrule
\multirow{2}{*}{Ours-MeanP (ViT-B/16)}     &                         &  47.1&75.0 &84.4&2.0&12.2&45.7&74.9&84.8&2.0&9.5 \\
                                           & \Checkmark    &47.3&74.9&84.0&2.0&12.8&46.0&75.1&84.1     &2.0&9.5\\\midrule
\multirow{2}{*}{Ours-seqTransf (ViT-B/16)} &                         & 49.8   & 75.1   & 83.0   & 2.0    & 12.2    & 46.6   & 75.2   & 83.7   & 2.0    & 9.0     \\
                                           & \Checkmark            & 49.8   & 75.1   & 83.9   & 2.0    & 12.2    & 47.3   & 76.0   & 84.3   & 2.0    & 8.9    \\
                                           \bottomrule
\end{tabular}%
}
\end{table*}
\begin{table*}[]
\centering
\caption{}
\label{tab:ablation codebook full}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cc|ccccc|ccccc}
\toprule
\multirow{2}{*}{Model}                     & \multirow{2}{*}{Codebook Size} & \multirow{2}{*}{QBNorm} & \multicolumn{5}{c}{Text to Video Retrieval} & \multicolumn{5}{c}{Video to Text Retrieval} \\
                                           &                                &                         & R@1    & R@5    & R@10   & MedR   & MeanR   & R@1    & R@5    & R@10   & MedR   & MeanR   \\\midrule
\multirow{8}{*}{Ours-seqTransf (ViT-B/32)} & 512                            &                         & 48.5   & 73.0   & \textbf{83.4}   & 2.0    & 12.9    & 46.4   & 72.8   & 82.6   & 2.0    & 9.0     \\
                                           & 512                            & \Checkmark            & \underline{48.7}   & 73.0   & \textbf{83.4}   & 2.0    & 12.9    & 46.4   & 72.8   & 82.6   & 2.0    & 9.0     \\
                                           & 1024             &              &   \underline{48.7}   & \textbf{73.9}   & 82.7   & 2.0    & 13.5    & 46.6   & \underline{73.4}   & 82.0   & 2.0    & 9.2     \\
                                           & 1024                           & \Checkmark            &   \textbf{49.1}   & \textbf{73.9}   & 82.8   & 2.0    & 13.5    & 46.9   & \textbf{73.8}   & 82.1   & 2.0    & 9.3     \\
                                           & 2048                           &                         & 47.9   & \textbf{73.9}   & 82.8   & 2.0    & 13.5    & 46.5   & 72.7   & 82.6   & 2.0    & 9.2     \\
                                           & 2048                           & \Checkmark            & 48.3   & \textbf{73.9}   & 82.8   & 2.0    & 13.5    & 47.0   & 72.7   & 82.6   & 2.0    & 9.1     \\
                                           & 4096                           &                         & 47.6   & \underline{73.6}   & 82.8   & 2.0    & 13.6    & 46.5   & \underline{73.4}   & \underline{82.8}   & 2.0    & 9.3     \\
                                           & 4096                           & \Checkmark            & 47.6   & \underline{73.6}   & \underline{82.9}   & 2.0    & 13.6    & 46.8   & \underline{73.4}   & \textbf{82.9}   & 2.0    & 9.3  \\\bottomrule  
\end{tabular}%
}
\end{table*}



\begin{table*}[]
\centering
\caption{Ablation study of $\alpha$ and $\beta$ on MSR-VTT.}
\label{tab:my-table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccc}
\toprule
                          &          &         & \multicolumn{4}{c}{Text to Video Retrieval}                      &                   & \multicolumn{4}{c}{Video to Text Retrieval}                      &                   \\
                          & $\alpha$ & $\beta$ & R@1$\uparrow$ & R@5$\uparrow$ & R@10$\uparrow$ & MnR$\downarrow$ & MeanR$\downarrow$ & R@1$\uparrow$ & R@5$\uparrow$ & R@10$\uparrow$ & MnR$\downarrow$ & MeanR$\downarrow$ \\
                          \midrule
Ours-seqTransf (ViT-B/32) & 0        & 0       & 48.0          & 72.9          & 82.4           & 2.0             & 13.1              & 45.4          & 73.2          & 82.1           & 2.0             & 9.1               \\
                          & 0.01     & 0       & 48.1          & 73.9          & 82.4           & 2.0             & 13.0              & 46.0          & 73.6          & 82.5           & 2.0             & 8.9               \\
                          & 0.02     & 0       & 48.0          & 73.5          & 82.7           & 2.0             & 13.4              & 47.1          & 74.2          & 82.9           & 2.0             & 9.1               \\
                          & 0.05     & 0       & 48.6          & 73.6          & 82.6           & 2.0             & 13.4              & 45.5          & 73.9          & 82.4           & 2.0             & 9.2               \\
                          & 0.1      & 0       &     48.8          &    73.0           &    82.4            & 2.0             &             13.3      &      45.9         &         74.2      &       82.3         & 2.0             &             9.1      \\
                          & 0        & 0.01    & 47.4          & 73.5          & 82.7           & 2.0             & 13.5              & 46.8          & 73.2          & 82.2           & 2.0             & 9.2               \\
                          & 0        & 0.02    & 48.6          & 72.4          & 83.5           & 2.0             & 13.6              & 46.2          & 73.2          & 83.3           & 2.0             & 9.1               \\
                          & 0        & 0.05    & 46.8          & 72.4          & 83.3           & 2.0             & 13.3              & 46.2          & 73.4          & 83.6           & 2.0             & 8.7               \\
                          & 0        & 0.1     & 48.1          & 73.2          & 83.0           & 2.0             & 13.4              & 46.5          & 73.3          & 81.9           & 2.0             & 8.9               \\
                          & 0.01     & 0.01    & 47.6          & 74.0          & 82.7           & 2.0             & 13.8              & 46.7          & 82.2          & 73.5           & 2.0             & 9.5               \\
                          & 0.01     & 0.02    & 48.5          & 74.1          & 83.6           & 2.0             & 13.5              & 47.0          & 73.2          & 82.9           & 2.0             & 9.1               \\
                          & 0.01     & 0.05    & 47.4          & 72.5          & 83.1           & 2.0             & 13.9              & 45.6          & 74.7          & 82.2           & 2.0             & 9.2               \\
                          & 0.01     & 0.1     & 47.4          & 73.2          & 82.6           & 2.0             & 13.4              & 46.2          & 73.4          & 82.6           & 2.0             & 8.7               \\
                          & 0.02     & 0.01    & 49.1          & 73.9          & 82.8           & 2.0             & 13.5              & 46.9          & 73.8          & 82.1           & 2.0             & 9.3               \\
                          & 0.02     & 0.02    & 48.5          & 73.8          & 83.2           & 2.0             & 14.0              & 46.3          & 73.1          & 82.1           & 2.0             & 9.4               \\
                          & 0.02     & 0.05    & 47.6          & 72.7          & 82.4           & 2.0             & 14.0              & 45.8          & 74.0          & 82.2           & 2.0             & 9.2               \\
                          & 0.02     & 0.1     & 47.7          & 72.3          & 82.9           & 2.0             & 13.4              & 45.3          & 73.6          & 83.3           & 2.0             & 9.0               \\
                          & 0.05     & 0.01    & 48.1          & 73.6          & 83.1           & 2.0             & 13.2              & 46.3          & 72.9          & 82.7           & 2.0             & 9.1               \\
                          & 0.05     & 0.02    & 48.5          & 74.3          & 83.5           & 2.0             & 13.8              & 46.2          & 73.8          & 82.2           & 2.0             & 9.2               \\
                          & 0.05     & 0.05    & 47.9          & 72.2          & 83.0           & 2.0             & 13.7              & 46.5          & 74.3          & 82.4           & 2.0             & 9.0               \\
                          & 0.05     & 0.1     & 47.3          & 73.2          & 83.4           & 2.0             & 12.9              & 45.2          & 75.0          & 83.1           & 2.0             & 9.1               \\
                          & 0.1      & 0.01    & 47.9          & 74.2          & 82.3           & 2.0             & 13.3              & 46.3          & 73.4          & 82.5           & 2.0             & 9.1               \\
                          & 0.1      & 0.02    & 48.2          & 73.9          & 83.8           & 2.0             & 13.5              & 46.4          & 73.1          & 82.4           & 2.0             & 9.3               \\
                          & 0.1      & 0.05    & 47.7          & 73.2          & 83.5           & 2.0             & 13.4              & 45.5          & 74.1          & 82.8           & 2.0             & 9.0               \\
                          & 0.1      & 0.1     & 46.9          & 73.3          & 82.9           & 2.0             & 13.4              & 46.0          & 73.8          & 82.5           & 2.0             & 9.0    \\
                          \bottomrule
\end{tabular}%
}
\end{table*}





\begin{table*}[]
\centering
\caption{Ablation study of different similarities on MSR-VTT.}
\label{tab:ablation study similarity full}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cc|cc|ccccc|cccccc}
\toprule
                          & \multicolumn{2}{c|}{Separated Spaces} & \multicolumn{2}{c|}{Aligned Codebook Space} & \multicolumn{5}{c|}{Text to Video Retrieval}                                          & \multicolumn{5}{c}{Video to Text Retrieval}                                                                                     \\
                          & Sentence-Video    & Sentence-Frame   & Sentence-Video       & Sentence-Frame      & R@1$\uparrow$ & R@5$\uparrow$ & R@10$\uparrow$ & MnR$\downarrow$ & MeanR$\downarrow$ & R@1$\uparrow$ & R@5$\uparrow$ & R@10$\uparrow$ & MnR$\downarrow$ & MeanR $\downarrow$ \\\midrule
\multirow{12}{*}{Ours-seqTransf (ViT-B/32)} & \Checkmark      &                  &                      &                                          & 42.8          & 72.0          & 82.3           & 2.0             & 15.0              & 41.9          & 71.1          & 81.5           & 2.0             & 11.1                                                             \\
                          &                   & \Checkmark     &                      &                     &  44.4          & 71.8          & 81.8           & 2.0             & 14.5              & 44.1          & 71.8          & 81.7           & 2.0             & 10.4                                                       \\
                          & \Checkmark      & \Checkmark     &                      &                     & 44.0          & 71.3          & 80.9           & 2.0             & 14.8              & 43.6          & 69.5          & 80.1           & 2.0             & 10.4                                                         \\
                          & \Checkmark      &                  & \Checkmark     &    & 43.3          & 70.5          & 81.4           & 2.0             & 15.6              & 42.5          & 71.0          & 80.9           & 2.0             & 11.9                                         \\
                          & \Checkmark      &                  &                      & \Checkmark        & 42.9          & 72.3          & 81.6           & 2.0             & 15.2              & 42.0          & 70.9          & 81.1           & 2.0             & 11.0                                                         \\
                          &                   & \Checkmark     & \Checkmark         &                     & 43.8          & 72.1          & 82.3           & 2.0             & 14.7              & 41.5          & 70.6          & 80.3           & 2.0             & 9.8                                                          \\
                          &                   & \Checkmark     &                      & \Checkmark        & 44.8          & 72.1          & 81.7           & 2.0             & 15.9              & 41.7          & 70.2          & 79.6           & 2.0             & 10.8                                                          \\
                          &                   &                  & \Checkmark         & \Checkmark        & 14.0          & 36.7          & 50.5           & 13.0            & 57.4              & 9.8           & 31.1          & 46.3           & 13.0            & 57.4                                                         \\
                          & \Checkmark      & \Checkmark     & \Checkmark         &                     & 47.4          & 73.3          & 82.4           & 2.0             & 12.9              & 46.4          & 73.0          & 82.2           & 2.0             & 8.9                                                          \\
                          & \Checkmark      & \Checkmark     &                      & \Checkmark        & 47.4          & 73.6          & 82.5           & 2.0             & 13.2              & 47.3          & 72.3          & 81.7           & 2.0             & 8.9                                                          \\
                          & \Checkmark      & \Checkmark     & \Checkmark         & \Checkmark        &      49.1   & 73.9   & 82.8   & 2.0    & 13.5    & 46.9   & 73.8   & 82.1   & 2.0    & 9.3         \\
                          \bottomrule
\end{tabular}%
}
\end{table*}



\begin{table*}[ht!]
\centering
\caption{Video-Text retrieval results on MSR-VTT. * represents data copied from Align\&Tell. Best results are marked in \textbf{bold}, second best results are \underline{underlined}.}
\label{tab:msr-vtt-full}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccc}
\toprule
\rowcolor{gray!30}             & \multicolumn{5}{c}{Text to Video Retrieval}                                        & \multicolumn{5}{c}{Video to Text Retrieval}                                        \\
\rowcolor{gray!30}             & R@1$\uparrow$ & R@5$\uparrow$ & R@10$\uparrow$ & MdR$\downarrow$ & MnR$\downarrow$ & R@1$\uparrow$ & R@5$\uparrow$ & R@10$\uparrow$ & MdR$\downarrow$ & MnR$\downarrow$ \\
\midrule
CLIP                           & 31.2          & 53.7          & 64.2           & 4.0               & -               & 27.2          & 51.7          & 62.6           & 5.0               & -               \\
CLIP4Clip-meanP (ViT-B/32)     & 43.1          & 70.4          & 80.8           & 2.0               & 16.2            & -             & -             & -              & -               & -               \\
CenterCLIP-meanP (ViT-B/32)    & \underline{44.2}          & 71.6          & \underline{82.1}           & 2.0               & 15.1            & \underline{42.8}          & \underline{71.7}          & \textbf{82.2}           & 2.0               & \underline{10.9}            \\
\midrule
DiscreteCodebook-meanP (ViT-B/32)    & 43.4          & \underline{72.3}          & 81.2           & -               & \underline{14.8}            & 42.5          & 71.2          & 81.1           & -               & 12.0            \\
\rowcolor{gray!30}\ours-MeanP (ViT-B/32)          & \textbf{47.0}          & \textbf{73.9}          & \underline{81.8}           & 2.0             & \textbf{14.5}            & \textbf{45.7}          & \textbf{72.3}          & \underline{82.0}           & 2.0             & \textbf{9.6}             \\
\bottomrule
CLIP4Clip-seqTransf (ViT-B/32) & 44.5          & 71.4          & 81.6           & 2.0               & 15.3            & -             & -             & -              & -               & -               \\
TS2-Net-seqTransf (ViT-B/32)   & 47.0          & \textbf{74.5}          & \underline{83.8}           & 2.0             & 13.0            & 45.3          & 74.1          & 83.7           & 2.0             & \underline{9.2}             \\
Align\&Tell (ViT-B/32)         & 45.2          & 73.0          & 82.9           & 2.0             & -               & 43.4          & 70.9          & 81.8           & 2.0             & -               \\
X-CLIP-seqTransf (ViT-B/32)    & 46.1          & \underline{74.3}          & 83.1           & 2.0             & 13.2            & 46.8          & 73.3          & \underline{84.0}           & 2.0             & \textbf{9.1}             \\
CAMoE (ViT-B/32)               & \underline{47.3}          & 74.2          & \textbf{84.5}           & 2.0             & 11.9            & \textbf{49.1}          & \textbf{74.3}          & \textbf{84.3}           & 2.0             & 9.9             \\
CLIP2TV (ViT-B/32)             & 45.6          & 71.1          & 80.8           & 2.0             & 15.0            & 43.9          & 70.9          & 82.2           & 2.0             & 12.0            \\
CLIP2Video (ViT-B/32)          & 45.6          & 72.6          & 81.7           & 2.0             & 14.6            & 43.5          & 72.3          & 82.1           & 2.0             & 10.2            \\
VCM (ViT-B/32)                 & 43.8          & 71.0          & 80.9           & 2.0             & 14.3            & 45.1          & 72.3          & 82.3           & 2.0             & 10.7            \\
X-Pool (ViT-B/32)    & 46.9          & 72.8          & 82.2           & 2.0               & 14.3            & -             & -             & -              & -               & -               \\
\midrule
\rowcolor{gray!30}\ours-seqTransf (ViT-B/32)      & \textbf{49.1}   & 73.9   & 82.8   & 2.0    & 13.5    & \underline{46.9}   & \underline{73.8}   & 82.1   & 2.0    & 9.3             \\
\bottomrule
CLIP4Clip-seqTransf (ViT-B/16) & 45.8*         & 74.3*         & 84.1*          & 2.0*              & -               & 43.2*         & 71.3*         & 82.0*          & 2.0*              & -               \\
Align\&Tell (ViT-B/16)         & 47.4          & 74.3          & 84.1           & 2.0             & -               & 45.3          & 73.5          & 83.7           & 2.0             & -               \\
CenterCLIP-meanP (ViT-B/16)    & 48.4          & 73.8          & 82.0           & 2.0               & 13.8            & \underline{47.7}          & 75.0          & 83.3           & 2.0               & 10.2            \\
CLIP2TV (ViT-B/16)             & 49.3          & 74.7          & 83.6           & 2.0             & \underline{13.5}            & 46.9          & 75.0          & \textbf{85.1}           & 2.0             & 10.0            \\
HiSE-seqTransf (ViT-B/16)      & 45.0          & 72.7          & 81.3           & 2.0             & -               & 46.6          & 73.3          & 82.3           & 2.0             & -               \\
TS2-Net-seqTransf (ViT-B/16)   & \underline{49.4}          & \underline{75.6}          & \textbf{85.3}           & 2.0             & \underline{13.5}            & 46.6          & 75.9          & \underline{84.9}           & 2.0             & \underline{8.9}             \\
X-CLIP-seqTransf (ViT-B/16)    & 49.3          & \textbf{75.8}          & \underline{84.8}           & 2.0             & \textbf{12.2}            & \textbf{48.9}          & \textbf{76.8}          & 84.5           & 2.0             & \textbf{8.1}             \\
\midrule
\rowcolor{gray!30}\ours-seqTransf (ViT-B/16)      & \textbf{49.8}          & 75.1          & 83.9           & 2.0             & \textbf{12.2}            & 47.3          & \underline{76.0}          & 84.3           & 2.0             & \underline{8.9}            \\
\bottomrule
\end{tabular}%
}
\end{table*}


\begin{table*}[]
\centering
\caption{MSVD}
\label{tab: msvd ablation}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccccccc}
                               & \multicolumn{5}{c}{Text to Video Retrieval}                                        & \multicolumn{5}{c}{Video to Text Retrieval}                                        \\
                               & R@1$\uparrow$ & R@5$\uparrow$ & R@10$\uparrow$ & MdR$\downarrow$ & MnR$\downarrow$ & R@1$\uparrow$ & R@5$\uparrow$ & R@10$\uparrow$ & MdR$\downarrow$ & MnR$\downarrow$ \\
CLIP                           & 37.0          & 64.1          & 73.8           & 3.0             & -               & 59.9          & 85.2          & 90.7           & 1.0             & -               \\
CLIP4Clip-MeanP (ViT-B/32)     & 46.2          & 76.1          & 84.6           & 2.0             & 10.0            & 56.6          & 79.7          & 92.6           & 1.0             & 7.6             \\
CLIP4Clip-seqTransf (ViT-B/32) & 45.2          & 75.5          & 84.3           & 2.0             & 10.3            & 62.0          & 87.3          & 92.6           & 1.0             & 4.3             \\
CLIP4Clip-seqTransf (ViT-B/16) & 47.2          & 77.7          &                & 2.0             & 9.1             & 63.2          & 87.2          &                &                 & 4.2             \\
X-CLIP (ViT-B/32)              & 47.1          & 77.8          & -              & -               & 9.5             & 60.9          & 87.8          & -              & -               & 4.7             \\
X-CLIP (ViT-B/16)              & 50.4          & 80.6          & -              & -               & 8.4             & 66.8          & 90.4          & -              & -               & 4.2             \\
CLIP2VIDEO                     & 47.0          & 76.8          & 85.9           & 2.0             & 9.6             & 58.7          & 85.6          & 91.6           & 1.0             & 4.3             \\
HiSE                           & 45.9          & 76.2          & 84.6           & 2.0             & -               & 66.3          & 90.7          & 95.2           & 1.0             & -               \\
X-Pool                         & 47.2          & 77.4          & 86.0           & 2.0             & 9.3             & -             & -             & -              & -               & -               \\
\ours                          & 47.3          & 78.8          & 85.7           & 2.0             & 9.3             &               &               &                &                 &                 \\
\ours                          & 50.1          & 80.2          & 87.5           & 2.0             & 8.5             &               &               &                &                 &                
\end{tabular}%
}
\end{table*}

\begin{table*}[]
\centering
\caption{ActivityNet}
\label{tab: actnet ablation}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccc}
                               & \multicolumn{5}{c}{Text to Video Retrieval}                                        & \multicolumn{5}{c}{Video to Text Retrieval}                                        \\
                               & R@1$\uparrow$ & R@5$\uparrow$ & R@10$\uparrow$ & MdR$\downarrow$ & MnR$\downarrow$ & R@1$\uparrow$ & R@5$\uparrow$ & R@10$\uparrow$ & MdR$\downarrow$ & MnR$\downarrow$ \\
CLIP4Clip-MeanP (ViT-B/32)     & 40.5          & 72.4          &                & 2.0             & 7.4             & 42.5          & 74.1          & 85.8           & 2.0             & 6.6             \\
CLIP4Clip-seqTransf (ViT-B/32) & 40.5          & 72.4          &                & 2.0             & 7.5             & 41.4          & 73.7          & 85.3           & 2.0             & 6.7             \\
CLIP4Clip-seqTransf (ViT-B/16) & 44.5          & 75.2          &                & 2.0             & 6.4             & 44.1          & 75.2          &                & 2.0             & 6.4             \\
Align\&Tell (ViT-B/32)         & 42.6          & 73.8          & -              & 2.0             & -               & 43.5          & 73.6          & -              & 2.0             & -               \\
Align\&Tell (ViT-B/16)         & 44.9          & 75.4          & -              & 2.0             & -               & 45.1          & 76.3          & -              & 2.0             & -               \\
X-CLIP (ViT-B/32)              & 44.3          & 74.1          & -              & -               & 7.9             & 43.9          & 73.9          & -              & -               & 7.6             \\
X-CLIP (ViT-B/16)              & 46.2          & 75.5          & -              & -               & 6.8             & 46.4          & 75.9          & -              & -               & 6.4             \\
TS2-Net                        & 41.0          & 73.6          & 84.5           & 2.0             & 8.4             & -             & -             & -              & -               & -               \\
VCM                            & 40.8          & 72.8          & -              & 2.0             & 7.3             & 42.6          & 74.9          & 86.2           & 2.0             & 6.4             \\

\ours                          & 45.0          & 75.5          & 85.7           & 2.0             & 6.3             & 44.5          & 75.6          & 86.9           & 2.0             & 6.0             \\
\ours                          &               &               &                &                 &                 &               &               &                &                 &                
\end{tabular}%
}
\end{table*}
